Linear Map of $D$-Algebra

Module is effective representation of ring in Abelian group. Linear map of module over commutative ring is morphism of corresponding representation. This definition is the main subject of the book. To consider this definition from more general point of view I started the book from consideration of Cartesian product of representations. Polymorphism of representations is a map of Cartesian product of representations which is a morphism of representations with respect to each separate independent variable. Reduced morphism of representations allows us to simplify the study of morphisms of representations. However a representation has to satisfy specific requirements for existence of reduced polymomorphism of representations. It is possible that Abelian group is only $\Omega$-algebra, such that representation in this algebra admits polymorphism of representations. However, today, this statement has not been proved. Multiplicative $\Omega$-group is $\Omega$-algebra in which product is defined. The definition of tensor product of representations of Abelian multiplicative $\Omega$-group is based on properties of reduced polymorphism of representations of Abelian multiplicative $\Omega$-group. Since an algebra is a module in which the product is defined, then we can use this theory to study linear map of algebra. For instance, we can study the set of linear transformations of $D$-algebra $A$ as representation of algebra $A\otimes A$ in algebra $A$.

==> Algebra.Linear.Map.Russian.tex <==
%auto-ignore
\input{Algebra.Linear.Map.Eq}

\chapter{Линейное отображение алгебры}
\label{chapter: Linear Map of Algebra}

\section{Линейное отображение алгебры}
\label{Section: Linear Map of Algebra}

\begin{definition}
\label{definition: linear map from A1 to A2, algebra}
Пусть $A_1$ и
$A_2$ - алгебры над кольцом $D$.
Линейное отображение
$D$\hyph модуля $A_1$
в $D$\hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
$D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
Обозначим
\ShowEq{set linear maps, module}
множество линейных отображений
$D$\Hyph алгебры
$A_1$
в $D$\Hyph алгебру
$A_2$.
\qed
\end{definition}

\begin{definition}
\label{definition: polylinear map of algebras}
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph алгебры.
Полилинейное отображение
\ShowEq{polylinear map of algebras}
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$,
Мы будем называть отображение
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph алгебру
$S$.
Обозначим
\ShowEq{set polylinear maps An}
множество $n$\hyph линейных отображений
$D$\Hyph алгебры $A$ ($A_1=...=A_n=A$)
в $D$\Hyph алгебру
$S$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: tensor product of D-algebras is D-algebra}
Тензорное произведение
$\Tensor A$
$D$\Hyph алгебр
$A_1$, ..., $A_n$
является $D$\Hyph алгеброй.
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: algebra over ring}
и теореме
\ref{theorem: there exists tensor product of modules},
тензорное произведение
$\Tensor A$
$D$\Hyph алгебр
$A_1$, ..., $A_n$
является $D$\Hyph модулем.

Рассмотрим отображение
\ShowEq{xA1n*xA1n->oxA1n}
определённое равенством
\ShowEq{xA1n*xA1n->oxA1n=}
Для заданных значений переменных
$b_1$, ..., $b_n$,
отображение
\EqRef{xA1n*xA1n->oxA1n}
полилинейно по переменным
$a_1$, ..., $a_n$.
Согласно теореме
\ref{theorem: tensor product and polylinear map},
существует линейное отображение
\ShowEq{b:oxA1n->oxA1n}
определённое равенством
\ShowEq{b:oxA1n->oxA1n=}
Так как произвольный тензор
\ShowEq{a in oxA1n}
можно представить в виде суммы тензоров вида
$\Tensor a$,
то для заданного тензора
\ShowEq{a in oxA1n}
отображение
\EqRef{b:oxA1n->oxA1n}
является полилинейным отображением переменных $b_1$, ..., $b_n$.
Согласно теореме
\ref{theorem: tensor product and polylinear map},
существует линейное отображение
\ShowEq{a:oxA1n->oxA1n}
определённое равенством
\ShowEq{a:oxA1n->oxA1n=}
Следовательно, равенство
\EqRef{a:oxA1n->oxA1n=}
определяет билинейное отображение
\ShowEq{oxA1n*oxA1n->oxA1n}
Билинейное отображение
\EqRef{oxA1n*oxA1n->oxA1n}
определяет произведение в $D$\Hyph модуле
$\Tensor A$.
\end{proof}

В случае
тензорного произведения $D$\Hyph алгебр
$A_1$, $A_2$
мы будем рассматривать произведение,
определённое равенством
\ShowEq{A12 2->A12 =}

\begin{theorem}
Пусть $\Basis e_i$ - базис алгебры $A_i$ над кольцом $D$.
Пусть $B_{i\cdot}{}^{\gi j}_{\gi{kl}}$ -
структурные константы алгебры $A_i$ относительно базиса $\Basis e_i$.
Структурные константы тензорного произведение $\Tensor A$
относительно базиса $\TensorBasis i$ имеют вид
\ShowEq{structural constants tensor algebra}
\end{theorem}
\begin{proof}
Непосредственное перемножение тензоров
$\TensorBasis i$ имеет вид
\ShowEq{structural constants tensor algebra, proof, 1}
Согласно определению структурных констант
\ShowEq{structural constants tensor algebra, proof, 2}
Равенство
\EqRef{structural constants tensor algebra}
следует из сравнения
\EqRef{structural constants tensor algebra, proof, 1},
\EqRef{structural constants tensor algebra, proof, 2}.

Из цепочки равенств
\ShowEq{structural constants tensor algebra, proof, 3}
следует, что определение произведения
\EqRef{structural constants tensor algebra, proof, 2}
со структурными константами
\EqRef{structural constants tensor algebra}
согласовано с определением произведения
\EqRef{a:oxA1n->oxA1n=}.
\end{proof}

\begin{theorem}
Для тензоров $a$, $b\in\Tensor A$
стандартные компоненты произведения удовлетворяют равенству
\ShowEq{standard components of product, tensor product}
\end{theorem}
\begin{proof}
Согласно определению
\ShowEq{standard components of product, tensor product, 1}
В тоже время
\ShowEq{standard components of product, tensor product, 2}
Равенство
\EqRef{standard components of product, tensor product}
следует из равенств
\EqRef{standard components of product, tensor product, 1},
\EqRef{standard components of product, tensor product, 2}.
\end{proof}

\begin{theorem}
Если алгебра $A_i$, $i=1$, ..., $n$, ассоциативна,
то тензорное произведение $\Tensor A$ - ассоциативная алгебра.
\end{theorem}
\begin{proof}
Поскольку
\ShowEq{tensor product, associative algebra, 1}
то
\ShowEq{tensor product, associative algebra, 2}
\end{proof}

\begin{theorem}
\label{theorem: tensor product and product in algebra}
Пусть $A$ -
алгебра над коммутативным кольцом $D$.
Существует линейное отображение
\ShowEq{tensor product and product in algebra}
\end{theorem}
\begin{proof}
Теорема является следствием определения
\ref{definition: algebra over ring}
и теоремы
\ref{theorem: tensor product and polylinear map}.
\end{proof}

\begin{theorem}
\label{theorem: linear map times constant, algebra}
Пусть отображение
\EqParm{f:A->B}{f=f,A=12}
является линейным отображением $D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
Тогда отображения
\ShowEq{linear map times constant, algebra}
определённые равенствами
\ShowEq{linear map times constant, 0, algebra}
также являются линейными.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{linear map times constant, 1, algebra}
\end{proof}

\Section{Алгебра \texorpdfstring{$\mathcal L(D;A\rightarrow A)$}{L(D;A->A)}}

\begin{theorem}
\label{theorem: product of linear map, algebra}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Пусть $f$ - линейное отображение из $D$\Hyph алгебры $A$ в $D$\Hyph алгебру $B$.
Пусть $g$ - линейное отображение из $D$\Hyph алгебры $B$ в $D$\Hyph алгебру $C$.
Отображение $g\circ f$, определённое диаграммой
\ShowEq{product of linear map, algebra}
является линейным отображением из $D$\Hyph алгебры $A$ в $D$\Hyph алгебру $C$.
\end{theorem}
\begin{proof}
Доказательство теоремы следует из цепочек равенств
\ShowEq{product of linear map, algebra, 1}
\end{proof}

\begin{theorem}
\label{theorem: product of linear map, algebra, f}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Пусть $f$ - линейное отображение из $D$\Hyph алгебры $A$ в $D$\Hyph алгебру $B$.
Отображение $f$ порождает линейное отображение
\ShowEq{product of linear map, algebra, f}
\ShowEq{product of linear map, algebra, f diagram}
\end{theorem}
\begin{proof}
Доказательство теоремы следует из цепочек равенств\,\footnote{Мы пользуемся
следующими определениями операций над отображениями
\ShowEq{operations over linear map}
}
\ShowEq{product of linear map, algebra, f1}
\end{proof}

\begin{theorem}
\label{theorem: product of linear map, algebra, g}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Пусть $g$ - линейное отображение из $D$\Hyph алгебры $B$ в $D$\Hyph алгебру $C$.
Отображение $g$ порождает линейное отображение
\ShowEq{product of linear map, algebra, g}
\ShowEq{product of linear map, algebra, g diagram}
\end{theorem}
\begin{proof}
Доказательство теоремы следует из цепочек равенств\,\footnote{Мы пользуемся
следующими определениями операций над отображениями
\ShowEq{operations over linear map}
}
\ShowEq{product of linear map, algebra, g1}
\end{proof}

\begin{theorem}
\label{theorem: product of linear map, algebra, gf}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Отображение
\ShowEq{product of linear map, algebra, gf}
является билинейным отображением.
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\ref{theorem: product of linear map, algebra, f},
\ref{theorem: product of linear map, algebra, g}.
\end{proof}

\begin{theorem}
\label{theorem: module L(A;A) is algebra}
Пусть $A$ - алгебра над коммутативным кольцом $D$.
$D$\Hyph модуль
\EqParm{L(A;B)}{A=A,=c}
оснащённый произведением
\ShowEq{module L(A;A) is algebra}
\ShowEq{product of linear map, algebra 1}
является алгеброй над $D$.
\end{theorem}
\begin{proof}
Теорема является следствием определения
\ref{definition: algebra over ring}
и теоремы
\ref{theorem: product of linear map, algebra, gf}.
\end{proof}

\section{Линейное отображение в ассоциативную алгебру}

\begin{theorem}
\label{theorem: bilinear map A LA}
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения
\EqParm{f in L(A->B)}{A=12,=z}
отображение
\ShowEq{bilinear map A LA}
является билинейным отображением.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{bilinear map A LA, 1}
\end{proof}

\begin{theorem}
\label{theorem: linear map AA LAA}
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения
\EqParm{f in L(A->B)}{A=12,=z}
существует линейное отображение
\ShowEq{linear map AA LAA}
определённое равенством
\ShowEq{linear map AA LAA, 1}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теорем
\ref{theorem: tensor product and polylinear map},
\ref{theorem: bilinear map A LA}.
\end{proof}

\begin{theorem}
\label{theorem: algebra A2 representation in LA}
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Определим произведение в алгебре $\ATwo$
согласно правилу
\ShowEq{product in algebra AA}
Линейное отображение
\ShowEq{representation A2 in LA}
определённое равенством
\ShowEq{representation A2 in LA, 1}
является представлением\,\footnote{Определение представления
$\Omega$\Hyph алгебры дано в определении
\xRef{0912.3315}{definition: left-side representation of algebra}.
}
алгебры $\ATwo$
в модуле
\EqParm{L(A;B)}{A=12,=.}
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: linear map times constant, algebra},
отображение \EqRef{representation A2 in LA, 1}
является преобразованием модуля
\EqParm{L(A;B)}{A=12,=.}
Для данного тензора $c\in \ATwo$
преобразование $h(c)$ является линейным преобразованием
модуля
\EqParm{L(A;B)}{A=12,=c}
так как
\ShowEq{representation A2 in LA, 2}
Согласно теореме
\ref{theorem: linear map AA LAA},
отображение \EqRef{representation A2 in LA, 1}
является линейным отображением.

Пусть
\ShowEq{algebra A2 representation in LA, 1}
Согласно теореме
\ref{theorem: linear map AA LAA}
\ShowEq{algebra A2 representation in LA, 2}
Следовательно, согласно теореме
\ref{theorem: linear map AA LAA}
\ShowEq{algebra A2 representation in LA, 3}
Поскольку произведение в алгебре $A_2$ ассоциативно, то
\ShowEq{algebra A2 representation in LA, 4}
Следовательно, если мы определим произведение в алгебре $\ATwo$
согласно равенству
\EqRef{product in algebra AA},
то отображение \EqRef{representation A2 in LA}
является морфизмом алгебр.
Согласно определению
\xRef{0912.3315}{definition: left-side representation of algebra},
отображение \EqRef{representation A2 in LA, 1}
является представлением алгебры $\ATwo$
в модуле
\EqParm{L(A;B)}{A=12,=.}
\end{proof}

\begin{theorem}
\label{theorem: representation of algebra A2 in LA}
Рассмотрим $D$\Hyph алгебру $A$.
Определим произведение в алгебре $A\otimes A$
согласно правилу
\EqRef{product in algebra AA}.
Представление
\ShowEq{representation AA in LA}
алгебры $A\otimes A$ в модуле
\EqParm{L(A;B)}{A=A,=c}
определённое равенством
\ShowEq{representation AA in LA, 1}
позволяет отождествить тензор
\ShowEq{product in algebra AA 1}
с отображением
\ShowEq{product in algebra AA 2}, где
\ShowEq{product in algebra AA 3}
- тождественное отображение.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: linear map AA LAA},
отображение
\EqParm{f in L(A->B)}{A=A,=z}
и тензор $d\in A\otimes A$
порождают отображение
\ShowEq{tensor and map in A, algebra}
Если мы положим $f=\delta$, $d=a\otimes b$,
то равенство \EqRef{tensor and map in A, algebra}
приобретает вид
\ShowEq{tensor and map in A, 1, algebra}
Если мы положим
\ShowEq{tensor and map in A, 2, algebra}
то сравнение равенств
\EqRef{tensor and map in A, 1, algebra} и
\EqRef{tensor and map in A, 2, algebra}
даёт основание отождествить действие тензора
$a\otimes b$ с
преобразованием $(a\otimes b)\circ\delta$.
\end{proof}

Из теоремы \ref{theorem: representation of algebra A2 in LA}
следует, что отображение
\EqRef{representation A2 in LA, 1}
можно рассматривать как произведение отображений
$a\otimes b$ и $f$.
Тензор $a\in \ATwo$
\AddIndex{невырожден}{nonsingular tensor},
если существует
тензор $b\in \ATwo$ такой, что $a\circ b=1\otimes 1$.

\begin{definition}
\begin{sloppypar}
Рассмотрим\,\footnote{Определение дано по
аналогии с определением
\xRef{0912.3315}{definition: orbit of left-side representation of group}.
} представление алгебры $\ATwo$
в модуле
\EqParm{L(A;B)}{A=12,=.}
\AddIndex{Орбитой линейного отображения}{orbit of linear map}
\EqParm{f in L(A->B)}{A=12,=z}
называется множество
\ShowEq{orbit of linear map}
\qed
\end{sloppypar}
\end{definition}

\ShowTheorem{h generated by f, associative algebra}
\begin{proof}
Произвольный тензор $a\in\ATwo$ можно представить в виде
\ShowEq{h generated by f 1, associative algebra}
Согласно теореме \ref{theorem: algebra A2 representation in LA},
отображение \EqRef{representation A2 in LA, 1}
линейно.
Это доказывает утверждение теоремы.
\end{proof}

\begin{theorem}
\label{theorem: orbit of linear map}
Пусть $A_2$ - алгебра с единицей $e$.
Пусть
\ShowEq{orbit of linear map, 02}
- невырожденный тензор.
Орбиты линейных отображений
\EqParm{f in L(A->B)}{A=12,=z}
и \ShowEq{orbit of linear map, 01}
совпадают
\ShowEq{orbit of linear map, f = g}
\end{theorem}
\begin{proof}
Если
\ShowEq{orbit of linear map, 1}
то существует
\ShowEq{orbit of linear map, 2}
такое, что
\ShowEq{orbit of linear map, 3}
Тогда
\ShowEq{orbit of linear map, 4}
Следовательно,
\ShowEq{orbit of linear map, 5}
\ShowEq{orbit of linear map, g in f}

Так как $a$ - невырожденный тензор, то
\ShowEq{orbit of linear map, 6}
Если
\ShowEq{orbit of linear map, 5}
то существует
\ShowEq{orbit of linear map, 2}
такое, что
\ShowEq{orbit of linear map, 7}
Из равенств
\EqRef{orbit of linear map, 6},
\EqRef{orbit of linear map, 7},
следует, что
\ShowEq{orbit of linear map, 8}
Следовательно,
\ShowEq{orbit of linear map, 1}
\ShowEq{orbit of linear map, f in g}

\EqRef{orbit of linear map, f = g}
следует из равенств
\EqRef{orbit of linear map, g in f},
\EqRef{orbit of linear map, f in g}.
\end{proof}

Из теоремы
\ref{theorem: orbit of linear map} также следует, что, если
\ShowEq{orbit of linear map, 01}
и \ShowEq{orbit of linear map, 02}
- вырожденный тензор, то
отношение
\EqRef{orbit of linear map, g in f} верно.
Однако основной результат теоремы
\ref{theorem: orbit of linear map}
состоит в том, что представления алгебры
$\ATwo$ в модуле
\EqParm{L(A;B)}{A=12,=z}
порождает отношение эквивалентности в модуле
\EqParm{L(A;B)}{A=12,=.}
Если удачно выбрать представители каждого класса эквивалентности,
то полученное множество будет множеством образующих
рассматриваемого представления.\,\footnote{Множество образующих
представления определено в определении
\xRef{0912.3315}{definition: generating set of representation}.
}

\Section{Линейное отображение в свободную
конечно мерную ассоциативную алгебру}

\ShowTheorem{standard representation of map A1 A2, associative algebra}
\ShowEq{proof: standard representation of map A1 A2, associative algebra}

\ShowTheorem{conjugation transformation}
\ShowEq{proof: conjugation transformation}

\ShowTheorem{representation of composition of linear maps}
\ShowEq{proof: representation of composition of linear maps}

\ShowTheorem{representation of composition of linear maps A->A}
\ShowEq{proof: representation of composition of linear maps A->A}

\ShowTheorem{coordinates of map A1 A2, algebra}
\ShowEq{proof: coordinates of map A1 A2, algebra}

\begin{theorem}
\label{theorem: linear map over ring, matrix}
Пусть $D$ является полем.
Пусть $\Basis e_1$ - базис свободной конечно мерной
$D$\Hyph алгебры $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть $C_{2\cdot}{}_{\gi{kl}}^{\gi p}$ - структурные константы алгебры $A_2$.
Рассмотрим матрицу
\ShowEq{linear map over ring, matrix}
строки которой пронумерованы индексом
\ShowEq{linear map over ring, row of matrix}
и столбцы пронумерованы индексом
\ShowEq{linear map over ring, column of matrix}.
Если
матрица $\mathcal B$ невырождена,
то для заданных координат линейного преобразования
\ShowEq{linear map over ring, left side}
и для отображения
\ShowEq{linear map over ring, f=1},
система линейных уравнений
\EqRef{coordinates of map A1 A2, 2, associative algebra}
относительно стандартных компонент этого преобразования
$g^{\gi{kr}}$ имеет единственное
решение.

Если
матрица $\mathcal B$ вырождена,
то условием существования решения
системы линейных уравнений
\EqRef{coordinates of map A1 A2, 2, associative algebra}
является равенство
\ShowEq{linear map over ring, determinant=0, 1}
В этом случае система линейных уравнений
\EqRef{coordinates of map A1 A2, 2, associative algebra}
имеет бесконечно много решений и существует линейная
зависимость между величинами $g_{\gim}^{\gik}$.
\end{theorem}
\begin{proof}
Утверждение теоремы
является следствием
теории линейных уравнений над полем.
\end{proof}

\begin{theorem}
\label{theorem: linear map over ring, determinant=0}
Пусть $A$ - свободная конечно мерная ассоциативная алгебра
над полем $D$.
Пусть $\Basis e$ - базис алгебры $A$ над полем $D$.
Пусть $C_{\gi{kl}}^{\gi p}$
- структурные константы алгебры $A$.
Пусть матрица \EqRef{linear map over ring, matrix} вырождена.
Пусть линейное отображение
\EqParm{f in L(A->B)}{A=A,=z}
невырождено.
Если координаты линейных преобразований $f$ и $g$
удовлетворяют равенству
\ShowEq{linear map over ring, determinant=0, 2}
то система линейных уравнений
\ShowEq{coordinates of map A}
имеет бесконечно много решений.
\end{theorem}
\begin{proof}
Согласно равенству
\EqRef{linear map over ring, determinant=0, 2}
и теореме
\ref{theorem: linear map over ring, matrix},
система линейных уравнений
\ShowEq{coordinates of map A1 A2, 4f}
имеет бесконечно много решений,
соответствующих линейному отображению
\ShowEq{coordinates of map A1 A2, 5f}
Согласно равенству
\EqRef{linear map over ring, determinant=0, 2}
и теореме
\ref{theorem: linear map over ring, matrix},
система линейных уравнений
\ShowEq{coordinates of map A1 A2, 4g}
имеет бесконечно много решений,
соответствующих линейному отображению
\ShowEq{coordinates of map A1 A2, 5g}
Отображения $f$ и $g$ порождены отображением $\delta$.
Согласно теореме
\ref{theorem: orbit of linear map},
отображение $f$ порождает отображение $g$.
Это доказывает утверждение теоремы.
\end{proof}

\begin{theorem}
\label{theorem: linear map in L(A,A), associative algebra}
Пусть $A$ - свободная конечно мерная ассоциативная алгебра
над полем $D$.
Представление алгебры $A\otimes A$ в алгебре
\EqParm{L(A;B)}{A=A,=z}
имеет конечный \AddIndex{базис}{basis of algebra L(A,A)} $\Basis I$.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\EqParm{f in L(A->B)}{A=A,=z}
имеет вид
\ShowEq{f in L(A,A), 1, associative algebra}
\LabelItem{f in L(A,A), 1, associative algebra}
\item
Его стандартное представление имеет вид
\ShowEq{f in L(A,A), 2, associative algebra}
\LabelItem{f in L(A,A), 2, associative algebra}
\end{enumerate}
\end{theorem}
\begin{proof}
Из теоремы \ref{theorem: linear map over ring, determinant=0}
следует, что если матрица $\mathcal B$ вырождена
и отображение $f$ удовлетворяет равенству
\ShowEq{linear map over ring, determinant=0, 3}
то отображение $f$ порождает то же самое множество отображений,
что порождено отображением $\delta$.
Следовательно, для того, чтобы построить базис представления
алгебры $A\otimes A$ в модуле
\EqParm{L(A;B)}{A=A,=c}
мы должны выполнить следующее построение.

Множество решений системы уравнений
\EqRef{coordinates of map A}
порождает свободный подмодуль $\mathcal L$ модуля
\EqParm{L(A;B)}{A=A,=.}
Мы строим базис $(\Vector h_1, ..., \Vector h_k)$ подмодуля $\mathcal L$.
Затем дополняем этот базис линейно независимыми векторами
$\Vector h_{k+1}$, ..., $\Vector h_m$, которые не принадлежат
подмодулю $\mathcal L$, таким образом, что множество векторов
$\Vector h_1$, ..., $\Vector h_m$
является базисом модуля
\EqParm{L(A;B)}{A=A,=.}
Множество орбит $(A\otimes A)\circ\delta$,
$(A\otimes A)\circ\Vector h_{k+1}$, ..., $(A\otimes A)\circ\Vector h_m$
порождает модуль
\EqParm{L(A;B)}{A=A,=.}
Поскольку множество орбит конечно, мы можем выбрать орбиты так, чтобы
они не пересекались. Для каждой орбиты мы можем выбрать
представитель, порождающий эту орбиту.
\end{proof}

\begin{example}
Для поля комплексных чисел алгебра $\mathcal L(R;C\rightarrow C)$ имеет базис
\ShowEq{basis L(C,C)}
Для алгебры кватернионов алгебра $\mathcal L(R;H\rightarrow H)$ имеет базис
\ShowEq{basis L(H,H)}
\qed
\end{example}

\section{Линейное отображение в неассоциативную алгебру}
\label{Section: Linear Map into Nonassociative Algebra}

Так как произведение неассоциативно, мы можем предположить,
что действие $a$, $b\in A$ на отображение $f$ может быть
представленно либо в виде $a(fb)$, либо в виде $(af)b$.
Однако это предположение приводит нас к довольно сложной
структуре линейного отображения.
Чтобы лучше представить насколько сложна структура линейного
отображения, мы начнём с рассмотрения левого и правого сдвигов
в неассоциативной алгебре.

\begin{theorem}
Пусть
\ShowEq{left shift algebra}
отображение левого сдвига.
Тогда
\ShowEq{left shift algebra, 1}
где мы определили линейное отображение
\ShowEq{left shift algebra, 2}
\end{theorem}
\begin{proof}
Из равенств
\EqRef{associator of algebra},
\EqRef{left shift algebra}
следует
\ShowEq{left shift algebra, 3}
Равенство \EqRef{left shift algebra, 1}
следует из равенства \EqRef{left shift algebra, 3}.
\end{proof}
%\ShowEq{left shift algebra, 2a}

\begin{theorem}
Пусть
\ShowEq{right shift algebra}
отображение правого сдвига.
Тогда
\ShowEq{right shift algebra, 1}
где мы определили линейное отображение
\ShowEq{right shift algebra, 2}
\end{theorem}
\begin{proof}
Из равенств
\EqRef{associator of algebra},
\EqRef{right shift algebra}
следует
\ShowEq{right shift algebra, 3}
Равенство \EqRef{right shift algebra, 1}
следует из равенства \EqRef{right shift algebra, 3}.
\end{proof}

Пусть
\ShowEq{f over A}
линейное отображение алгебры $A$.
Согласно теореме \ref{theorem: linear map times constant, algebra},
отображение
\ShowEq{g over A}
также линейное отображение.
Однако неочевидно, можем ли мы записать отображение $g$ в виде
суммы слагаемых вида $(ax)b$ и $a(xb)$.

Если $A$ - свободная конечно мерная алгебра, то мы можем предположить,
что линейное отображение имеет стандартное представление в виде\,\footnote{Выбор
произволен. Мы можем рассмотреть стандартное представление в виде
\ShowEq{linear map, standard representation, nonassociative algebra, 1}
Тогда равенство
\EqRef{coordinates of map A1 A2, 2, nonassociative algebra}
имеет вид
\ShowEq{coordinates of map A1 A2, 21, nonassociative algebra}
Я выбрал выражение
\EqRef{linear map, standard representation, nonassociative algebra}
так как порядок сомножителей соответствует порядку, выбранному в теореме
\ref{theorem: linear map in L(A,A), associative algebra}.}
\ShowEq{linear map, standard representation, nonassociative algebra}
В этом случае мы можем применить
теорему \ref{theorem: linear map in L(A,A), associative algebra}
для отображений в неассоциативную алгебру.

\begin{theorem}
\label{theorem: coordinates of map A1 A2, nonassociative algebra}
Пусть $\Basis e_1$ - базис свободной конечно мерной
$D$\Hyph алгебры $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной неассоциативной
$D$\Hyph алгебры $A_2$.
Пусть $C_{2\cdot}{}_{\gi{kl}}^{\gi p}$ - структурные константы алгебры $A_2$.
Пусть отображение
\ShowEq{standard representation of map A1 A2, 1, nonassociative algebra}
порождённое отображением
\EqParm{f in L(A->B)}{A=12,=z}
посредством тензора $a\in\ATwo$, имеет стандартное представление
\ShowEq{standard representation of map A1 A2, 2, nonassociative algebra}
Координаты отображения
\EqRef{standard representation of map A1 A2, 1, nonassociative algebra}
и его стандартные компоненты
связаны равенством
\ShowEq{coordinates of map A1 A2, 2, nonassociative algebra}
\end{theorem}
\begin{proof}
Относительно базисов
$\Basis e_1$ и $\Basis e_2$, линейные отображения $f$ и $g$ имеют вид
\ShowEq{coordinates of maps f g, nonassociative algebra}
Из равенств
\EqRef{coordinates of map f, nonassociative algebra},
\EqRef{coordinates of map g, nonassociative algebra},
\EqRef{standard representation of map A1 A2, 2, nonassociative algebra}
следует
\ShowEq{coordinates of map A1 A2, 3, nonassociative algebra}
Так как векторы $\Vector e_{2\cdot\gik}$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\EqRef{coordinates of map A1 A2, 2, nonassociative algebra}
следует из равенства
\EqRef{coordinates of map A1 A2, 3, nonassociative algebra}.
\end{proof}

\begin{theorem}
\label{theorem: linear map in L(A,A), nonassociative algebra}
Пусть $A$ - свободная конечно мерная неассоциативная алгебра
над кольцом $D$.
Представление алгебры $A\otimes A$ в алгебре
\EqParm{L(A;B)}{A=A,=z}
имеет конечный базис $\Basis I$.
\begin{enumerate}
\item \label{f in L(A,A), 1, nonassociative algebra}
Линейное отображение
\EqParm{f in L(A->B)}{A=A,=z}
имеет вид
\ShowEq{f in L(A,A), 1, nonassociative algebra}
\item \label{f in L(A,A), 2, nonassociative algebra}
Его стандартное представление имеет вид
\ShowEq{f in L(A,A), 2, nonassociative algebra}
\end{enumerate}
\end{theorem}
\begin{proof}
Рассмотрим матрицу
\EqRef{linear map over ring, matrix}.
Если
матрица $\mathcal B$ невырождена,
то для заданных координат линейного преобразования
\ShowEq{linear map over ring, left side}
и для отображения
\ShowEq{linear map over ring, f=1},
система линейных уравнений
\EqRef{coordinates of map A1 A2, 2, nonassociative algebra}
относительно стандартных компонент этого преобразования
$g^{\gi{kr}}$ имеет единственное
решение.
Если
матрица $\mathcal B$ вырождена,
то согласно теореме
\ref{theorem: linear map in L(A,A), associative algebra}
существует конечный базис $\Basis I$,
порождающий множество линейных отображений.
\end{proof}

В отличие от случая ассоциативной алгебры
множество генераторов $I$ в теореме
\ref{theorem: linear map in L(A,A), nonassociative algebra}
не является минимальным.
Из равенства \EqRef{left shift algebra, 1}
следует, что неверно равенство
\EqRef{orbit of linear map, 4}.
Следовательно, орбиты отображений
$I_k$ не порождают отношения эквивалентности в алгебре $L(A;A)$.
Так как мы рассматриваем только отображения вида $(aI_k)b$, то
возможно, что при $k\ne l$ отображение $I_k$ порождает отображение $I_l$,
если рассмотреть все возможные операции в алгебре $A$.
Поэтому множество образующих $I_k$ неассоциативной алгебры $A$
не играет такой критической роли как отображение сопряжения в
поле комплексных чисел.
Ответ на вопрос насколько важно отображение $I_k$ в
неассоциативной алгебре требует дополнительного исследования.

\section{Полилинейное отображение в ассоциативную алгебру}

\begin{theorem}
\label{theorem: polylinear map A 1n A}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Пусть
\ShowEq{set of maps, L(A;A)}
\ShowEq{set of elements A}
Для заданной перестановки $\sigma$ $n$ переменных
отображение
\ShowEq{n linear map A LA}
является $n$\hyph линейным отображением в алгебру $A$.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{polylinear map A 1n A, 1}
\end{proof}

В равенстве \EqRef{n linear map A LA},
также как и в других выражениях полилинейного отображения,
принято соглашение, что отображение $f_i$ имеет своим аргументом переменную $x_i$.

\begin{theorem}
\label{theorem: polylinear map A LA}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Для заданного семейства отображений
\ShowEq{set of maps, L(A;A)}
отображение
\ShowEq{n+1 linear map A LA}
определённое равенством
\ShowEq{n+1 linear map A LA 1}
является $n+1$\hyph линейным отображением в $D$\Hyph модуль $\LAAnA$.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{n+1 linear map A LA, 1}
\end{proof}

\begin{theorem}
\label{theorem: linear map An LAAnA}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Для заданного семейства отображений
\ShowEq{set of maps, L(A;A)}
существует линейное отображение
\ShowEq{linear map An LAAnA}
определённое равенством
\ShowEq{linear map An LAAnA, 1}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теорем
\ref{theorem: tensor product and polylinear map},
\ref{theorem: polylinear map A LA}.
\end{proof}

\begin{theorem}
\label{theorem: polylinear map A LA, 1}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Для заданного тензора
\ShowEq{tensor over A} и заданной перестановки $\sigma\in S_n$
отображение
\ShowEq{n linear map LA LA}
определённое равенством
\ShowEq{n linear map LA LA 1}
является $n$\hyph линейным отображением в $D$\Hyph модуль $\LAAnA$.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{representation An in LAAnA, 3}
\end{proof}

\begin{theorem}
\label{theorem: linear map LA LA, 1}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Для заданного тензора
\ShowEq{tensor over A} и заданной перестановки $\sigma\in S_n$
существует линейное отображение
\ShowEq{linear map LA LA}
определённое равенством
\ShowEq{linear map LA LA, 1}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теорем
\ref{theorem: tensor product and polylinear map},
\ref{theorem: polylinear map A LA, 1}.
\end{proof}

\begin{theorem}
\label{theorem: polylinear map, algebra}
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Полилинейное отображение
\ShowEq{polylinear map, algebra}
порождённое отображениями
\ShowEq{I1n in L(A;A)},
имеет вид
\ShowEq{polylinear map, algebra, canonical morphism}
где $\sigma_s$ - перестановка множества переменных
\ShowEq{transposition of set of variables, algebra}
\end{theorem}
\begin{proof}
Мы докажем утверждение индукцией по $n$.

При $n=1$ доказываемое утверждение является следствием утверждения
\RefItem{f in L(A,A), 1, associative algebra}.
При этом мы можем отождествить\,\footnote{В представлении
\EqRef{polylinear map, algebra, canonical morphism}
мы будем пользоваться следующими правилами.
\begin{itemize}
\item Если область значений какого-либо индекса - это множество,
состоящее из одного элемента, мы будем опускать соответствующий
индекс.
\item Если $n=1$, то $\sigma_s$ - тождественное преобразование.
Это преобразование можно не указывать в выражении.
\end{itemize}}
\ShowEq{polylinear map, associative algebra, 1, canonical morphism}

Допустим, что утверждение теоремы справедливо при $n=k-1$.
Тогда отображение
\EqRef{polylinear map, algebra}
можно представить в виде
\ShowEq{polylinear map, induction on n, 1, associative algebra}
Согласно предположению индукции полилинейное отображение
$h$ имеет вид
\ShowEq{polylinear map, induction on n, 2, associative algebra}
Согласно построению $h=g\circ a_k$.
Следовательно, выражения $h_{t\cdot p}$
являются функциями $a_k$.
Поскольку $g\circ a_k$ - линейная функция $a_k$,
то только одно выражение $h_{t\cdot p}$
является линейной функцией переменной $a_k$, и остальные выражения
$h_{t\cdot q}$
не зависят от $a_k$.

Не нарушая общности, положим $p=0$.
Согласно равенству
\EqRef{h generated by f, associative algebra}
для заданного $t$
\ShowEq{polylinear map, induction on n, 3, associative algebra}
Положим $s=tr$ и определим перестановку $\sigma_s$ согласно правилу
\ShowEq{polylinear map, induction on n, 4, associative algebra}
Положим
\ShowEq{polylinear map, induction on n, 5, associative algebra}
Мы доказали шаг индукции.
\end{proof}

\begin{definition}
\begin{sloppypar}
Выражение
\ShowEq{component of polylinear map, associative algebra}
в равенстве \EqRef{polylinear map, algebra, canonical morphism}
называется
\AddIndex{компонентой полилинейного отображения}
{component of polylinear map} $f$.
\qed
\end{sloppypar}
\end{definition}

\begin{theorem}
\label{theorem: representation module An in LAAnA}
Рассмотрим $D$\Hyph алгебру $A$.
Линейное отображение
\ShowEq{representation An in LAnA}
определённое равенством
\ShowEq{representation An in LAnA, 1}
является представлением\,\footnote{Определение представления
$\Omega$\Hyph алгебры дано в определении
\xRef{0912.3315}{definition: left-side representation of algebra}.
}
алгебры
\ShowEq{representation An in LAnA, 2}
в $D$\Hyph модуле $\LAnA$.
\end{theorem}
\begin{proof}
Согласно теоремам
\ref{theorem: linear map in L(A,A), associative algebra},
\ref{theorem: polylinear map, algebra},
$n$\hyph линейное отображение можно представить в виде суммы слагаемых
\EqRef{n linear map A LA},
где $f_i$, $i=1$, ..., $n$, генераторы представления
\EqRef{representation A2 in LA}.
Запишем слагаемое $s$ выражения
\EqRef{polylinear map, algebra, canonical morphism}
в виде
\ShowEq{n linear map A LA, 1}
где
\ShowEq{n linear map A LA, 2}
Положим в равенстве
\EqRef{n linear map A LA, 1}
\ShowEq{n linear map A LA, 3}
Следовательно, согласно теореме
\ref{theorem: linear map An LAAnA},
отображение \EqRef{representation An in LAnA, 1}
является преобразованием модуля $\LAnA$.
Для данного тензора $c\in \AOn$
и заданной перестановки $\sigma\in S_n$,
преобразование $h(c,\sigma)$ является линейным преобразованием
модуля $\LAnA$
согласно теореме \ref{theorem: linear map LA LA, 1}.
Согласно теореме
\ref{theorem: linear map An LAAnA},
отображение \EqRef{representation An in LAnA, 1}
является линейным отображением.
\ifx\texFuture\Defined
Пусть
\ShowEq{algebra An representation in LAnA, 1}
Согласно теореме
\ref{theorem: linear map LA LA, 1}
\ShowEq{algebra An representation in LAnA, 2}
Следовательно, согласно теореме
\ref{theorem: linear map LA LA, 1}
\ShowEq{algebra An representation in LAnA, 3}
Поскольку произведение в алгебре $A$ ассоциативно, то
\ShowEq{algebra An representation in LAnA, 4}
Следовательно, если мы определим произведение в алгебре $\AOn$
согласно равенству
\EqRef{product in algebra An},
то отображение \EqRef{representation An in LAnA, 1}
является морфизмом алгебр.
\fi
Согласно определению
\xRef{0912.3315}{definition: left-side representation of algebra},
отображение \EqRef{representation An in LAnA, 1}
является представлением алгебры
\ShowEq{representation An in LAnA, 2}
в модуле $\LAnA$.
\end{proof}

\begin{theorem}
\label{theorem: representation of algebra An in LAnA}
Рассмотрим $D$\Hyph алгебру $A$.
Представление
\ShowEq{representation An in LAnA}
алгебры $\AOn$
в модуле $\LAnA$,
определённое равенством
\EqRef{representation An in LAnA, 1}
позволяет отождествить тензор
\ShowEq{product in algebra An 1}
и перестановку $\sigma\in S^n$
с отображением
\ShowEq{product in algebra An 2} где
\ShowEq{product in algebra AA 3}
- тождественное отображение.
\end{theorem}
\begin{proof}
Если в равенстве \EqRef{linear map An LAAnA, 1}
мы положим $f_i=\delta$,
\ShowEq{n tensor and map in A, 3, algebra},
то равенство \EqRef{linear map An LAAnA, 1}
приобретает вид
\ShowEq{n tensor and map in A, 1, algebra}
Если мы положим
\ShowEq{n tensor and map in A, 2, algebra}
то сравнение равенств
\EqRef{n tensor and map in A, 1, algebra} и
\EqRef{n tensor and map in A, 2, algebra}
даёт основание отождествить действие тензора
\ShowEq{n tensor and map in A, 3, algebra}
и перестановки $\sigma\in S^n$
с отображением \EqRef{product in algebra An 2}.
\end{proof}

Вместо записи $(a_0\otimes...a_n,\sigma)$ мы также будем пользоваться
записью
\[
a_0\otimes_{\sigma(1)}...\otimes_{\sigma(n)}a_n
\]
если мы хотим явно указать какой аргумент становится на соответствующее место.
Например, следующие выражения эквивалентны
\ShowEq{example of tensor notation}

\section{Полилинейное отображение в свободную
конечно мерную ассоциативную алгебру}

\begin{theorem}
\label{theorem:  polylinear map, finite dimensional associative algebra}
Пусть $A$ - свободная конечно мерная ассоциативная алгебра
над кольцом $D$.
Пусть $\Basis I$ - базис алгебры
\EqParm{L(A;B)}{A=A,=.}
Пусть $\Basis e$ - базис алгебры $A$ над кольцом $D$.
\AddIndex{Стандартное представление полилинейного отображения}
{polylinear map, standard representation} в ассоциативную алгебру
имеет вид
\ShowEq{standard component of polylinear map}
\ShowEq{polylinear map, associative algebra, standard representation}
Индекс $t$ нумерует всевозможные перестановки
$\sigma_t$ множества переменных
\VarSet.
Выражение
$\ShowSymbol{standard component of polylinear map}{}$
в равенстве \EqRef{polylinear map, associative algebra, standard representation}
называется \AddIndex{стандартной компонентой полилинейного отображения}
{standard component of polylinear map} $f$.
\end{theorem}
\begin{proof}
Мы изменим индекс $s$ в равенстве
\EqRef{polylinear map, algebra, canonical morphism}
таким образом, чтобы сгруппировать слагаемые с одинаковым набором генераторов $I_k$.
Выражение \EqRef{polylinear map, algebra, canonical morphism}
примет вид
\ShowEq{polylinear map, algebra, canonical morphism, 1}
Мы предполагаем, что индекс $s$ принимает значения, зависящие от $k_1$, ..., $k_n$.
Компоненты полилинейного отображения $f$
имеют разложение
\ShowEq{polylinear map, associative algebra, components extention}
относительно базиса $\Basis e$.
Если мы подставим \EqRef{polylinear map, associative algebra, components extention}
в \EqRef{polylinear map, algebra, canonical morphism},
мы получим
\ShowEq{polylinear map, associative algebra, standard representation, 1}
Рассмотрим выражение
\ShowEq{polylinear map, associative algebra, standard representation, 2}
В правой части подразумевается сумма тех слагаемых с индексом $s$,
для которых перестановка $\sigma_s$ совпадает. Каждая такая сумма
будет иметь уникальный индекс $t$.
Подставив в равенство
\EqRef{polylinear map, associative algebra, standard representation, 1}
выражение
\EqRef{polylinear map, associative algebra, standard representation, 2}
мы получим равенство \EqRef{polylinear map, associative algebra, standard representation}.
\end{proof}

\begin{theorem}
\label{theorem: polylinear map over field, associative algebra}
Пусть $A$ - свободная конечно мерная ассоциативная алгебра
над кольцом $D$.
Пусть $\Basis e$ - базис алгебры $A$ над кольцом $D$.
Полилинейное отображение
\EqRef{polylinear map, algebra}
можно представить в виде $D$-значной формы степени $n$
над кольцом $D$\,\footnote{Теорема доказана по аналогии
с теоремой в \citeBib{Rashevsky}, с. 107, 108}
\ShowEq{polylinear map over ring, associative algebra}
где
\ShowEq{polylinear map over ring, coordinates, associative algebra}
%и величины $f_{\gi{i_1...i_n}}$
%являются координатами $D$-значного ковариантнго тензора.
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: polylinear map of algebras}
равенство
\EqRef{polylinear map over ring, associative algebra}
следует из цепочки равенств
\ShowEq{polylinear map over ring, 1, associative algebra}
Пусть $\Basis e'$ - другой базис. Пусть
\ShowEq{polylinear map over ring, associative algebra, change basis}
преобразование, отображающее базис $\Basis e$ в
базис $\Basis e'$.
Из равенств \EqRef{polylinear map over ring, associative algebra, change basis}
и \EqRef{polylinear map over ring, coordinates, associative algebra}
следует
\ShowEq{polylinear map over ring, associative algebra, change coordinates}
%Из равенства \EqRef{polylinear map over ring, associative algebra, change coordinates}
%следует тензорный закон преобразования координат полилинейного отображения.
%Из равенства \EqRef{polylinear map over ring, associative algebra, change coordinates}
%и теоремы
%\ref{theorem: free module over ring, change basis}
%следует, что значение отображения $f\circ(\Vector a_1,...,\Vector a_n)$ не зависит от выбора
%базиса.
\end{proof}

Полилинейное отображение
\EqRef{polylinear map, algebra}
\AddIndex{симметрично}
{polylinear map symmetric, associative algebra}, если
\ShowEq{polylinear map symmetric, associative algebra, definition}
для любой перестановки $\sigma$ множества \VarSet.

\begin{theorem}
\label{theorem: polylinear map symmetric, associative algebra}
Если полилинейное отображение $f$ симметрично,
то
\ShowEq{polylinear map symmetric, associative algebra}
\end{theorem}
\begin{proof}
Равенство
\EqRef{polylinear map symmetric, associative algebra}
следует из равенства
\ShowEq{polylinear map symmetric, 1, associative algebra}
\end{proof}

Полилинейное отображение
\EqRef{polylinear map, algebra}
\AddIndex{косо симметрично}{polylinear map skew symmetric}, если
\ShowEq{polylinear map skew symmetric, associative algebra, definition}
для любой перестановки $\sigma$ множества \VarSet.
Здесь
\[
|\sigma|=
\left\{
\begin{matrix}
1&\textrm{перестановка }\sigma\textrm{ чётная}
\\
-1&\textrm{перестановка }\sigma\textrm{ нечётная}
\end{matrix}
\right.
\]

\begin{theorem}
\label{theorem: polylinear map skew symmetric, associative algebra}
Если полилинейное отображение $f$ косо симметрично,
то
\ShowEq{polylinear map skew symmetric, associative algebra}
\end{theorem}
\begin{proof}
Равенство
\EqRef{polylinear map skew symmetric, associative algebra}
следует из равенства
\ShowEq{polylinear map skew symmetric, 1, associative algebra}
\end{proof}

\begin{theorem}
\label{theorem: coordinates of polylinear map, associative algebra over ring}
Пусть $A$ - свободная конечно мерная ассоциативная алгебра
над кольцом $D$.
Пусть $\Basis I$ - базис алгебры
\EqParm{L(A;B)}{A=A,=.}
Пусть $\Basis e$ - базис алгебры $A$ над кольцом $D$.
Пусть полилинейное над кольцом $D$ отображение $f$
порождено набором отображений $(I_{k_1},...,I_{k_n})$.
Координаты отображения $f$
и его компоненты относительно базиса $\Basis e$
удовлетворяют равенству
\ShowEq{coordinates of polylinear map, associative algebra over ring}
\end{theorem}
\begin{proof}
В равенстве \EqRef{polylinear map, associative algebra, standard representation}
положим
\ShowEq{coordinates of polylinear map, 1, associative algebra over ring}
Тогда равенство \EqRef{polylinear map, associative algebra, standard representation}
примет вид
\ShowEq{polylinear map, associative algebra, standard representation, 1a}
Из равенства \EqRef{polylinear map over ring, associative algebra}
следует
\ShowEq{polylinear map over field, associative algebra, 1a}
Равенство
\EqRef{coordinates of polylinear map, associative algebra over ring}
следует из сравнения равенств
\EqRef{polylinear map, associative algebra, standard representation, 1a}
и
\EqRef{polylinear map over ring, associative algebra}.
Равенство
\EqRef{coordinates of polylinear map, associative algebra over ring, 1}
следует из сравнения равенств
\EqRef{polylinear map, associative algebra, standard representation, 1a}
и
\EqRef{polylinear map over field, associative algebra, 1a}.
\end{proof}


==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Doctor Ouch}
{
Корней Чуковский. Айболит.
\\
Детский мир, ISBN 978-5-91315-875-8, 2012
}%

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3). Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau I}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, механика,
М., Наука, 1988
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Landau III}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, том III, квантовая механика,
нерелятивистская теория,
М., Наука, 1989
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 3}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $3$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 12}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, части 1 - 2,
М., Наука, 1969
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том I, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Dubrovin Fomenko Novikov part 2}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том II, Геометрия и топология многообразий,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Kobayashi Nomizu vol 1}
{
Ш. Кобаяси, К. Номидзу,
Основы дифференциальной геометрии, Том I,
перевод с английского Л. В. Сабинина,
М., Наука, 1981
}%

\BiblioItem{Lichnerowicz}
{
Андрэ Лихнерович,
Теория связностей в целом и группы голономий,
перевод с французкого С. П. Финикова под редакцией В. В. Рыжкова,
М., Иностранная литература, 1960
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I. Gelfand, V. Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{0911.4454}
{
Vladimir Retakh,
From factorizations of noncommutative polynomials to combinatorial topology,\\
eprint \href{http://arxiv.org/abs/0911.4454}{arXiv:0911.4454} (2009)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники. ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Coppel: Number Theory}
{
W.A. Coppel,
Number Theory: An Introduction to Mathematics,\\
Springer, 2009
}%

\BiblioItem{978-0486497952}
{
Michael J. Field,
Differential Calculus and Its Applications,\\
Dover Publications, 2012; ISBN-13: 978-0486497952
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная универсальная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts{T}представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1111.6035}
{
Александр Клейн,
Базис представления универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/1111.6035}{arXiv:1111.6035} (2011)
}%

\BiblioItem{1201.4158}
{
Александр Клейн, Александер Ложье,
Ортонормированный базис в пространстве Минковского,\\
eprint \href{http://arxiv.org/abs/1201.4158}{arXiv:1201.4158} (2012)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1206.0200}
{
Александр Клейн,
Алгебра частных алгебры с сопряжением,\\
eprint \href{http://arxiv.org/abs/1206.0200}{arXiv:1206.0200} (2012)
}

\BiblioItem{1211.6965}
{
Александр Клейн,
Свободная алгебра со счётным базисом,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\BiblioItem{1302.7204}
{
Александр Клейн,
Многочлен над ассоциативной $D$-алгеброй,\\
eprint \href{http://arxiv.org/abs/1302.7204}{arXiv:1302.7204} (2013)
}%

\BiblioItem{1305.4547}
{
Александр Клейн,
Нормированная $\Omega$-группа,\\
eprint \href{http://arxiv.org/abs/1305.4547}{arXiv:1305.4547} (2013)
}%

\BiblioItem{1310.5591}
{
Александр Клейн,
Интеграл отображения в абелевую $\Omega$\Hyph группу,\\
eprint \href{http://arxiv.org/abs/1310.5591}{arXiv:1310.5591} (2013)
}%

\BiblioItem{1502.04063}
{
Александр Клейн,
Линейное отображение $D$\Hyph алгебры,\\
eprint \href{http://arxiv.org/abs/1502.04063}{arXiv:1502.04063} (2015)
}%

\BiblioItem{1505.03625}
{
Александр Клейн,
Производная отображения банаховой алгебры,\\
eprint \href{http://arxiv.org/abs/1505.03625}{arXiv:1505.03625} (2015)
}%

\BiblioItem{1601.03259}
{
Александр Клейн,
Введение в математический анализ над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1601.03259}{arXiv:1601.03259} (2016)
}%

\BiblioItem{MRepro}
{
Александр Клейн,
Теория представлений универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/MRepro}{arXiv:MRepro} (2015)
}%

\BiblioItem{Mpolym}
{
Александр Клейн,
Линейное отображение D-алгебры,\\
eprint \href{http://arxiv.org/abs/Mpolym}{arXiv:Mpolym} (2017)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{4776-3181}
{
Александр Клейн.\\
Линейная алгебра над телом: Система линейных уравнений.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1502982476
}%

\BiblioItem{4993-2400}
{
Александр Клейн.\\
Линейная алгебра над телом: Векторное пространство.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1499323948
}%

\BiblioItem{5059-9176}
{
Александр Клейн.\\
Нормированная \(\Omega\)-группа.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1505992359
}%

\BiblioItem{5114-6019}
{
Александр Клейн.\\
Представление универсальной алгебры: Полиморфизм.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1511464949
}%

\BiblioItem{5148-4632}
{
Александр Клейн.\\
Представление универсальной алгебры: Полиморфизм.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1511464949
}%

\BiblioItem{BRepro}
{
Александр Клейн,
Теория представлений универсальной алгебры,\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{CACAA.01.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{CACAA.02.097}
{
Aleks Kleyn,
Polynomial over Associative $D$-Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 2, Issue 2, pages 97 - 115, 2013
}%

\BiblioItem{CACAA.04.001}
{
Aleks Kleyn,
Integral of Map into Abelian $\Omega$-group.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 4, Issue 1, pages 1 - 68, 2013
}%

\BiblioItem{CACAA.05.001}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 5, issue 1, pages 1 - 68, 2016 
}%

\BiblioItem{GJSFRA.13.1.39}
{
Aleks Kleyn,
Reference frame and Lorentz transformation,\\
Global Journals of Science Frontier Research A,
volume 13, issue 1, pages 39 - 55, 2013 
}%

\BiblioItem{1506.05848}
{
Rida T. Farouki, Graziano Gentili, Carlotta Giannelli, Alessandra Sestini,
Caterina Stoppato,\\
Solution of a quadratic quaternion equation with mixed coefficients,\\
eprint \href{http://arxiv.org/abs/1506.05848}{arXiv:1506.05848} (2015)
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010).
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008).
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Cohn: Algebra 1}
{
Paul M. Cohn,
Algebra, Volume 1,
John Wiley \& Sons, 1982
}%

\BiblioItem
{Cohn: Algebra 3}
{
Paul M. Cohn,
Algebra, Volume 3,
John Wiley \& Sons, 1991
}%

\BiblioItem
{Cohn: Skew Fields}
{
Paul M. Cohn,
Skew Fields,
Cambridge University Press, 1995
}%

\BiblioItem
{Lam: Noncommutative Rings}
{
T. Y. Lam,
A First Course in
Noncommutative Rings,
Springer-Verlag, 1991
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem{Bourbaki: Algebra 2}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М., Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fikhtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 3}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 3,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{Basic Concepts of Differential Geometry}
{
Алексеевский Д. В., Виноградов А. М., Лычагин В. В.,
Основные понятия дифференциальной геометрии
\\
Итоги ВИНИТИ 28
\\
М. ВИНИТИ, 1988
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Convention.Russian.tex <==
%auto-ignore
\input{\FilePrefix Convention.Eq}

\section{Соглашения}

\ePrints{0812.4763,0906.0135,0908.3307,0909.0855,0912.3315,1003.1544}
\Items{1006.2597}
\ifx\Semafor\ValueOn
\begin{convention}
Функция и отображение - синонимы. Однако существует
традиция соответствие между кольцами или векторными
пространствами называть отображением, а отображение
поля действительных чисел или алгебры кватернионов называть функцией.
Я тоже следую этой традиции,
хотя встречается текст, в котором неясно, какому термину надо
отдать предпочтение.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1001.4852}
\Items{1003.1544,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
В любом выражении, где появляется индекс, я предполагаю,
что этот индекс может иметь внутреннюю структуру.
Например, при рассмотрении алгебры $A$ координаты $a\in A$
относительно базиса $\Basis e$ пронумерованы индексом $i$.
Это означает, что $a$ является вектором. Однако, если $a$
является матрицей, нам необходимо два индекса, один нумерует
строки, другой - столбцы. В том случае, когда мы уточняем структуру
индекса, мы будем начинать индекс с символа $\cdot$ в соответствующей
позиции.
Например, если я рассматриваю матрицу $a^i_j$ как элемент векторного
пространства, то я могу записать элемент матрицы в виде $a^{\cdot}{}^i_j$.
\qed
\end{convention}
\fi

\ePrints{1502.04063,5148-4632}
\ifx\Semafor\ValueOn
\begin{convention}
Мы будем пользоваться соглашением Эйнштейна о сумме,
в котором повторяющийся индекс (один вверху и один внизу)
подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av}
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1006.2597,1011.3102}
\Items{1211.6965,4910-5816,GJSFRF.Basis,1302.7204,CACAA.02.097}
\Items{4993-2400,1502.04063}
\ifx\Semafor\ValueOn
\begin{convention}
В выражении вида
\ShowEq{Sum over repeated index}
предполагается сумма по индексу $i$.
\qed
\end{convention}
\fi

\ePrints{4975-6381,1505.03625}
\ifx\Semafor\ValueOn
\begin{convention}
Если тензор
\ShowEq{a in Aoxn+1}
имеет разложение
\ShowEq{a=oxi}
то множество перестановок
\ShowEq{si in Sn}
и тензор $a$
порождают отображение
\ShowEq{ox:An->A}
определённое равенством
\ShowEq{ox circ =}
\qed
\end{convention}
\fi

\ePrints{4975-6381,1505.03625}
\ifx\Semafor\ValueOn
\begin{convention}
Пусть тензор
\ShowEq{a in Aoxn+1}.
Если
\ShowEq{x1=xn=x}
то мы положим
\ShowEq{a xn=}
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855}
\ifx\Semafor\ValueOn
\begin{convention}
Тело $D$ можно рассматривать как $D$\Hyph векторное пространство
размерности $1$. Соответственно этому, мы можем изучать не только
гомоморфизм тела $D_1$ в тело $D_2$, но и линейное отображение тел.
\qed
\end{convention}
\fi

\ePrints{0912.4061}
\ifx\Semafor\ValueOn
\begin{convention}
Для данного поля $F$, если не оговорено противное,
мы будем рассматривать конечномерную $F$\Hyph алгебру.
%без делителей нуля.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
Несмотря на некоммутативность произведения многие утверждения
сохраняются, если заменить например правое представление на
левое представление или правое векторное пространство на левое
векторное пространство.
Чтобы сохранить эту симметрию в формулировках теорем
я пользуюсь симметричными обозначениями.
Например, я рассматриваю \Ds векторное пространство
и \sD векторное пространство.
Запись \Ds векторное пространство можно прочесть
как D\Hyph star\Hyph векторное пространство либо
как левое векторное пространство.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,1211.6965,4910-5816,CACAA.01.195,GJSFRF.Basis,1302.7204}
\Items{CACAA.02.097,4993-2400,5148-4632,1502.04063}
\ifx\Semafor\ValueOn
\begin{convention}
\label{convention: we use separate color for index of element}
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,GJSFRF.Basis,1302.7204,CACAA.02.097}
\ifx\Semafor\ValueOn
\begin{convention}
%\label{convention: }
Очень трудно провести границу между модулем и алгеброй.
Тем более, иногда в процессе построения мы должны сперва
доказать, что множество $A$ является модулем,
а потом мы доказываем, что это множество является алгеброй.
Поэтому для записи координат элемента модуля
мы также будем пользоваться соглашением
\ref{convention: we use separate color for index of element}.
\qed
\end{convention}
\fi

\ePrints{1302.7204,CACAA.02.097,1310.5591,MSimplex,MBasis,1412.5425,5114-6019}
\ifx\Semafor\ValueOn
\begin{convention}
Элемент
\ePrints{1302.7204,CACAA.02.097,MSimplex,MBasis,1412.5425}
\ifx\Semafor\ValueOn
$D$\Hyph алгебры
\fi
\ePrints{5114-6019}
\ifx\Semafor\ValueOn
$\Omega$\Hyph алгебры
\fi
\ePrints{1310.5591}
\ifx\Semafor\ValueOn
$\Omega$\Hyph группы
\fi
$A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph числом, а кватернион называется $H$\Hyph числом.
\qed
\end{convention}
\fi

\ePrints{1305.4547,5059-9176,5114-6019}
\ifx\Semafor\ValueOn
\begin{convention}
Я обозначаю
\ShowEq{set of n-ary operations}
множество $n$\Hyph арных операций $\Omega$\Hyph алгебры.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,4993-2400}
\ifx\Semafor\ValueOn
\begin{convention}
Отождествление вектора и матрицы его координат
может привести к неоднозначности в равенстве
\ShowEq{Identification can lead to ambiguity, 1}
где $\Basis e$ - базис векторного пространства.
Поэтому мы будем записывать равенство
\EqRef{Identification can lead to ambiguity, 1}
в виде
\ShowEq{Identification can lead to ambiguity, 2}
чтобы видеть, где записан вектор.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,CACAA.01.195,1502.04063,5148-4632}
\ifx\Semafor\ValueOn
\begin{convention}
Если свободная конечномерная алгебра имеет единицу,
то мы будем отождествлять
вектор базиса $\Vector e_{\gi 0}$ с единицей алгебры.
\qed
\end{convention}
\fi

\ePrints{1104.5197,1105.4307}
\ifx\Semafor\ValueOn
\begin{convention}
Хотя алгебра является свободным модулем над некоторым
кольцом, мы не пользуемся векторными обозначениями
при записи элементов алгебры. В тех случаях, когда я рассматриваю
матрицу координат элемента алгебры, я буду пользоваться векторными
обозначениями для записи соответствующего элемента.
Чтобы не возникала неоднозначность при записи сопряжения,
я буду обозначать $a^*$ элемент, сопряжённый элементу $a$.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072,RepresentationE}
\ifx\Semafor\ValueOn
\begin{convention}
Так как число универсальных алгебр в башне представлений переменно,
то мы будем пользоваться векторными обозначениями для башни
представлений. Множество
$(A_1,...,A_n)$ $\Omega_i$\Hyph алгебр $A_i$, $i=1$, ..., $n$
мы будем обозначать $\Vector A$. Множество представлений
$(f_{1,2},...,f_{n-1,n})$ этих алгебр мы будем обозначать $\Vector f$.
Так как разные алгебры имеют разный тип, мы также
будем говорить о множестве $\Vector{\Omega}$\Hyph алгебр.
\ePrints{8443-0072,RepresentationE}
\ifx\Semafor\ValueOn
Символом
\else
По отношению к множеству $\Vector A$
мы также будем пользоваться матричными обозначениями, предложенными
в разделе \xRef{0701.238}{section: Concept of Generalized Index}.
Например, символом
\fi
$\Vector A_{[1]}$ мы будем обозначать
множество $\Vector{\Omega}$\Hyph алгебр $(A_2,...,A_n)$.
В соответствующем обозначении $(\VX A,\Vector f)$ башни
представлений подразумевается, что $\Vector f=(f_{2,3},...,f_{n-1,n})$.
\qed
\end{convention}

\begin{convention}
Так как мы пользуемся векторными обозначениями для элементов
башни представлений, необходимо соглашение о записи операций.
Предполагается, что операции выполняются покомпонентно. Например,
\ShowEq{vector notation in tower of representations}
\qed
\end{convention}
\fi

\ePrints{8443-0072,1111.6035,0906.0135,NewAffine,1102.5168,1305.4547,1310.5591}
\Items{1003.3714,4820-2669,MBasis,4993-2400,1412.5425,5059-9176,5114-6019}
\ifx\Semafor\ValueOn
\begin{convention}
Пусть $A$ - $\Omega_1$\Hyph алгебра.
Пусть $B$ - $\Omega_2$\Hyph алгебра.
Запись
\ShowEq{A->*B}
означает, что определено представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
\qed
\end{convention}
\fi

\ePrints{0702.561,0707.2246,0803.2620}
\ifx\Semafor\ValueOn
\begin{convention}
Я пользуюсь стрелкой $\xymatrix{\arp[r]&}$
на диаграмме для обозначения проекции расслоения.
Я пользуюсь стрелкой $\xymatrix{\ars[r]&}$
на диаграмме для обозначения сечения расслоения.
\qed
\end{convention}
\fi

\ePrints{0912.3315}
\ifx\Semafor\ValueOn
\begin{remark}
Я считаю диаграммы отображений важным инструментом. Однако временами возникает
желание увидеть диаграмму трёх мерной, что увеличило бы её выразительную
мощность. Кто знает какие сюрпризы готовит будущее.
В 1992 на конференции в Казани я рассказывал своим коллегам
какие преимущества имеет компьютерная подготовка статей.
Спустя 8 лет из письма из Казани я узнал, что теперь можно
готовить статьи с помощью LaTeX.
\qed
\end{remark}
\fi

\ePrints{1001.4852,1003.1544,1006.2597,1011.3102}
\ifx\Semafor\ValueOn
\begin{convention}
Если в некотором выражении используется несколько
операций, среди которых есть операция $\circ$, то предполагается,
что операция $\circ$ выполняется первой.
Ниже приведен пример эквивалентных выражений.
\ShowEq{list circ expressions}
\qed
\end{convention}
\fi

%\ePrints{0906.0135,NewAffine}
%\ifx\Semafor\ValueOn
%\item
%Пусть $\VX X$ - базис башни представлений $(\Vector A,\Vector f)$.
%Мы будем называть $\Omega_n$\Hyph слово
%$w_n(\Vector f,\VX X,x_n)$ координатами $x_n\in A_n$
%относительно базиса $\VX X$.
%\fi

\ePrints{1107.1139}
\ifx\Semafor\ValueOn
\begin{convention}
Для данной $D$\Hyph алгебры $A$
левый сдвиг
\ShowEq{left shift, D algebra}
определён равенством
\ShowEq{left shift 1, D algebra}
и правый сдвиг
\ShowEq{right shift, D algebra}
определён равенством
\ShowEq{right shift 1, D algebra}
\qed
\end{convention}
\fi

\ePrints{1412.5425}
\ifx\Semafor\ValueOn
\begin{convention}
Пусть $A$ ассоциативная $D$\Hyph алгебра.
Представление
\ShowEq{A2->*A}
$D$\Hyph модуля
\ShowEq{AoxA}
определено равенством
\ShowEq{a ox b c=}
и порождает множество линейных отображений.
Это представление порождает произведение $\circ$ в $D$\Hyph модуле
\ShowEq{AoxA}
согласно правилу
\ShowEq{(pq)a=p(qa)}
\qed
\end{convention}
\fi

\ePrints{MBasis}
\ifx\Semafor\ValueOn
\begin{convention}
Мы будем полагать,
что рассматриваемая мера является полной мерой.
\qed
\end{convention}
\fi

\ifx\PrintPaper\undefined
%Без сомнения, у читателя могут быть вопросы,
%замечания, возражения. Я буду признателен любому отзыву.
\fi



==> D.Algebra.Russian.tex <==
%auto-ignore

\input{D.Algebra.Eq}

\chapter{\texorpdfstring{$D$}{D}-алгебра}

\section{Алгебра над коммутативным кольцом}

\begin{definition}
\label{definition: algebra over ring}
Пусть $D$ - коммутативное кольцо.
$D$\Hyph модуль $A$ называется
\AddIndex{алгеброй над кольцом}{algebra over ring} $D$
или
\AddIndex{$D$\Hyph алгеброй}{D algebra},
если определена операция произведения\,\footnote{Я следую определению,
приведенному в
\citeBib{Richard D. Schafer}, с. 1,
\citeBib{0105.155}, с. 4. Утверждение,
верное для произвольного $D$\Hyph модуля,
верно также для $D$\Hyph алгебры.} в $A$
\DrawEq{product in D algebra}{definition}
где $C$ - билинейное отображение
\ShowEq{product in algebra, definition 1}
Если $A$ является свободным
$D$\Hyph модулем, то $A$ называется
\AddIndex{свободной алгеброй над кольцом}{free algebra over ring} $D$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: multiplication in algebra is distributive over addition}
Произведение в алгебре $A$ дистрибутивно по отношению к сложению.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочки равенств
\ShowEq{product distributive in algebra}
\end{proof}

Произведение в алгебре может быть ни коммутативным,
ни ассоциативным. Следующие определения основаны на
определениях, данным в \citeBib{Richard D. Schafer}, с. 13.

\begin{definition}
\label{definition: commutator of algebra}
\AddIndex{Коммутатор}{commutator of algebra}
\ShowEq{commutator of algebra}
служит мерой коммутативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{коммутативной}{commutative D algebra},
если
\ShowEq{commutative D algebra}
\qed
\end{definition}

\begin{definition}
\label{definition: associator of algebra}
\AddIndex{Ассоциатор}{associator of algebra}
\ShowEq{associator of algebra}
служит мерой ассоциативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной}{associative D algebra},
если
\ShowEq{associative D algebra}
\qed
\end{definition}

\begin{theorem}
Пусть $A$ - алгебра над коммутативным кольцом $D$.\,\footnote{Утверждение
теоремы опирается на равенство
\citeBib{Richard D. Schafer}-(2.4).}
\ShowEq{associator of algebra, 1}
для любых $a$, $b$, $c$, $d\in A$.
\end{theorem}
\begin{proof}
Равенство \EqRef{associator of algebra, 1}
следует из цепочки равенств
\ShowEq{associator of algebra, 2}
\end{proof}

\begin{definition}
\label{definition: nucleus of algebra}
\AddIndex{Ядро $D$\Hyph алгебры $A$}{nucleus of algebra}
- это
множество\,\footnote{Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 13}
\ShowEq{nucleus of algebra}
\qed
\end{definition}

\begin{definition}
\label{definition: center of algebra}
\AddIndex{Центр $D$\Hyph алгебры $A$}{center of algebra}
- это
множество\,\footnote{Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 14}
\ShowEq{center of algebra}
\qed
\end{definition}

\begin{theorem}
\label{theorem: unit of algebra and ring}
Пусть $D$ - коммутативное кольцо.
Если $D$\Hyph алгебра $A$ имеет единицу, то существует
изоморфизм $f$ кольца $D$ в центр алгебры $A$.
\end{theorem}
\begin{proof}
Пусть $e\in A$ - единица алгебры $A$.
Положим $f\circ a=ae$.
\end{proof}

Пусть $\Basis e$ - базис свободной алгебры $A$ над кольцом $D$.
Если алгебра $A$ имеет единицу,
положим $e_{\gi 0}$ - единица алгебры $A$.

\begin{theorem}
\label{theorem: product in algebra}
Пусть $\Basis e$ - базис свободной алгебры $A$ над кольцом $D$.
Пусть
\ShowEq{a b in basis of algebra}
Произведение $a$, $b$ можно получить согласно правилу
\ShowEq{product in algebra}
где
\ShowEq{structural constants of algebra}
- \AddIndex{структурные константы}{structural constants}
алгебры $A$ над кольцом $D$.
Произведение базисных векторов в алгебре $A$ определено согласно правилу
\ShowEq{product of basis vectors, algebra}
\end{theorem}
\begin{proof}
Равенство
\EqRef{product of basis vectors, algebra}
является следствием утверждения, что $\Basis e$
является базисом алгебры $A$.
Так как произведение в алгебре является билинейным отображением,
то произведение $a$ и $b$ можно записать в виде
\ShowEq{product in algebra, 1}
Из равенств
\EqRef{product of basis vectors, algebra},
\EqRef{product in algebra, 1},
следует
\ShowEq{product in algebra, 2}
Так как $\Basis e$ является базисом алгебры $A$, то равенство
\EqRef{product in algebra}
следует из равенства
\EqRef{product in algebra, 2}.
\end{proof}

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\begin{theorem}
Если алгебра $A$ коммутативна, то
\ShowEq{commutative product in algebra, 1}
Если алгебра $A$ ассоциативна, то
\ShowEq{associative product in algebra, 1}
\end{theorem}
\begin{proof}
Для коммутативной алгебры,
равенство
\EqRef{commutative product in algebra, 1}
следует из равенства
\ShowEq{commutative product in algebra}
Для ассоциативной алгебры,
равенство
\EqRef{associative product in algebra, 1}
следует из равенства
\ShowEq{associative product in algebra}
\end{proof}

\begin{theorem}
\label{theorem: Free Algebra over Ring}
Представление
\ShowEq{endomorphism of module from product}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
эквивалентно структуре $D$\Hyph алгебры $A$.
\end{theorem}
\begin{proof}
$\ $
\begin{itemize}
\item
Пусть в $D$\Hyph модуле $A$
определена структура $D$\Hyph алгебры $A$,
порождённая произведением
\DrawEq{product in D algebra}{}
Согласно определениям
\ref{definition: algebra over ring}
и
\ref{definition: polylinear map of modules},
\AddIndex{левый сдвиг $D$\Hyph модуля $A$}{left shift of module},
определённый равенством
\ShowEq{l(v):w->vw}
является линейным отображением.
Согласно определению
\ref{definition: linear map from A1 to A2, commutative module},
отображение \(l\circ v\)
является эндоморфизмом $D$\Hyph модуля $A$.

Равенство
\ShowEq{l(v1+v2)w}
является следствием определения
\ref{definition: polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{def sum of linear maps}
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(v1+v2)}
является следствием равенства
\EqRef{l(v1+v2)w}.
Равенство
\ShowEq{l(dv)w}
является следствием определения
\ref{definition: polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(dv)}
является следствием равенства
\EqRef{l(dv)w}.
Из равенств
\EqRef{l(v1+v2)},
\EqRef{l(dv)}
следует, что отображение
\ShowEq{v->l(v)}
является представлением $D$\Hyph модуля $A$
в $D$\Hyph модуле $A$
\ShowEq{endomorphism of module from product, 1}
\item
Рассмотрим представление
\EqRef{endomorphism of module from product}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$.
Поскольку отображение $f_{2,3}\circ v$ является эндоморфизмом $D$\Hyph модуля $A$, то
\ShowEq{endomorphism of module from product, 3}
Поскольку отображение
\EqRef{endomorphism of module from product}
является линейным отображением
\ShowEq{f23:A->L}
то,
\ShowEq{ref sum and product over scalar, linear map}
\ShowEq{endomorphism of module from product, 4}
\ShowEq{endomorphism of module from product, 7}
Из равенств
\EqRef{endomorphism of module from product, 3},
\EqRef{endomorphism of module from product, 4},
\EqRef{endomorphism of module from product, 7}
и определения
\ref{definition: polylinear map of modules},
следует, что отображение $f_{2,3}$ является билинейным отображением.
Следовательно, отображение $f_{2,3}$ определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
\end{itemize}
\end{proof}

\begin{corollary}
$D$ - коммутативное кольцо, $A$ - абелевая группа.
%Мы сперва рассматриваем вертикальное представление,
%а затем горизонтальные.
Диаграмма представлений
\EquationParm{diagram of representations of D algebra}{D= F= A=}
порождает структуру $D$\Hyph алгебры $A$.
\qed
\end{corollary}

\section{Линейный гомоморфизм}

\begin{theorem}
Пусть
\EquationParm{diagram of representations of D algebra}{D=1 F=1 A=1}
диаграмма представлений, описывающая $D_1$\Hyph алгебру $A_1$.
Пусть
\EquationParm{diagram of representations of D algebra}{D=2 F=2 A=2}
диаграмма представлений, описывающая $D_2$\Hyph алгебру $A_2$.
Морфизм $D_1$\Hyph алгебры $A_1$
в $D_2$\Hyph алгебру $A_2$
- это кортеж отображений
\ShowEq{Morphism of D algebra}
где отображение \(r_1\)
является гомоморфизмом кольца \(D_1\) в кольцо \(D_2\)
и отображение \(r_2\)
является линейным отображением
$D_1$\Hyph алгебры $A_1$ в $D_2$\Hyph алгебру $A_2$
таким, что
\ShowEq{Morphism of D algebra, 1}
\end{theorem}
\begin{proof}
Согласно равенствам
\xEqRef{0912.3315}{morphism of tower of representations, levels k k+1},
морфизм $\rR$ представления $f_{1,2}$
удовлетворяет равенству
\ShowEq{algebra, morphism of representation 12}
Следовательно, отображение $\rR$ является
линейным отображением.

Согласно равенству
\xEqRef{0912.3315}{morphism of tower of representations, levels k k+1},
морфизм $(r_2,r_2)$ представления $f_{2,3}$
удовлетворяет равенству\,\footnote{Так как в диаграммах представлений
\EqRefParm{diagram of representations of D algebra}{D=1 F=1 A=1},
\EqRefParm{diagram of representations of D algebra}{D=2 F=2 A=2},
носители $\Omega_2$\Hyph алгебры и
$\Omega_3$\Hyph алгебры совпадают, то также совпадают
морфизмы представлений на уровнях $2$ и $3$.}
\DrawEq{algebra, 23}{morphism of representation}
Из равенств
\eqRef{algebra, 23}{morphism of representation},
\EqRefParm{diagram of representations of D algebra}{D=1 F=1 A=1},
\EqRefParm{diagram of representations of D algebra}{D=2 F=2 A=2},
следует
\ShowEq{algebra, morphism of representation 23, 1}
Равенство
\EqRef{Morphism of D algebra, 1}
следует
из равенств
\EqRef{algebra, morphism of representation 23, 1},
\eqRef{product in D algebra}{definition}.
\end{proof}

\begin{definition}
\label{definition: linear homomorphism}
Морфизм представлений $D_1$\Hyph алгебры $A_1$
в $D_2$\Hyph алгебру $A_2$
называется
\AddIndex{линейным гомоморфизмом}{linear homomorphism}
$D_1$\Hyph алгебры $A_1$
в $D_2$\Hyph алгебру $A_2$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: linear homomorphism of d algebra}
Пусть $\Basis e_1$ - базис $D_1$\Hyph алгебры $A_1$.
Пусть $\Basis e_2$ - базис $D_2$\Hyph алгебры $A_2$.
Тогда линейный гомоморфизм\,\footnote{Эта теорема
аналогична теореме
\ShowEq{ref linear map of rcd vector space}
} $\rR$
$D_1$\Hyph алгебры $A_1$
в $D_2$\Hyph алгебру $A_2$ имеет представление\,\footnote{Произведение
матриц над коммутативным кольцом определено только как
\RC произведение.
Однако я предпочитаю явно указывать операцию,
так как в этом случае видно, что в выражении
участвуют матрицы. Кроме того, я планирую
рассмотреть подобную теорему в некоммутативном случае.
}
\ShowEq{algebra, morphism of representation 12, 11}
\ShowEq{algebra, morphism of representation 12, 12}
относительно заданных базисов. Здесь
\begin{itemize}
\item $a$ - координатная матрица вектора
$\Vector a$ относительно базиса $\Basis e_1$.
\item $b$ - координатная матрица вектора
\ShowEq{Vector b=r_2(a)}
относительно базиса $\Basis e_2$.
\item $r_2$ - координатная матрица множества векторов
\ShowEq{Vector r_2(e_1)}
относительно базиса $\Basis e_2$.
Мы будем называть матрицу $r_2$
\AddIndex{матрицей линейного гомоморфизма}{matrix of linear homomorphism}
относительно базисов $\Basis e_1$ и $\Basis e_2$.
\end{itemize}
\end{theorem}
\begin{proof}
Вектор $\Vector a\in A_1$ имеет разложение
\ShowEq{a in A1}
относительно базиса $\Basis e_1$.
Вектор $\Vector b\in A_2$ имеет разложение
\ShowEq{b in A2}
относительно базиса $\Basis e_2$.

Так кaк $\rR$ - линейный гомоморфизм, то на основании
\EqRef{algebra, morphism of representation 12} следует,
что
\ShowEq{linear homomorphism, 1}
где
\ShowEq{r1(a)}
\ShowEq{linear homomorphism, 1i}
также вектор $D$\Hyph модуля $A_2$ и имеет
разложение
\ShowEq{linear homomorphism, 2}
относительно базиса $\Basis e_2$.
Комбинируя \EqRef{linear homomorphism, 1}
и \EqRef{linear homomorphism, 2}, мы получаем
\EqRef{algebra, morphism of representation 12, 11}.
\EqRef{algebra, morphism of representation 12, 12}  следует
из сравнения \EqRef{b in A2}
и \EqRef{algebra, morphism of representation 12, 11} и
теоремы
\ShowEq{ref expansion relative basis, vector space}
\end{proof}

\begin{theorem}
\label{theorem: Morphism of D algebra}
Пусть $\Basis e_1$ - базис $D_1\star$\Hyph алгебры $A_1$.
Пусть $\Basis e_2$ - базис $D_2\star$\Hyph алгебры $A_2$.
Если отображение $r_1$ является инъекцией,
то матрица линейного гомоморфизма
и структурные константы связаны соотношением
\ShowEq{algebra, linear homomorphism and product}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{a, b in A1}
Из равенств
\ShowEq{algebra, linear homomorphism and product, 1}
следует
\DrawEq{algebra, homomorphism and product}{linear}
Из равенств
\EqRef{algebra, morphism of representation 12},
\eqRef{algebra, homomorphism and product}{linear},
следует
\ShowEq{algebra, linear homomorphism and product, 3}
Поскольку отображение $r_1$ является гомоморфизмом колец,
то из равенства
\EqRef{algebra, linear homomorphism and product, 3},
следует
\ShowEq{algebra, linear homomorphism and product, 4}
Из теоремы
\ref{theorem: linear homomorphism of d algebra}
и равенства
\EqRef{algebra, linear homomorphism and product, 4},
следует
\ShowEq{algebra, linear homomorphism and product, 5}

Из равенства
\EqRef{Morphism of D algebra, 1}
и теоремы
\ref{theorem: linear homomorphism of d algebra},
следует
\ShowEq{algebra, linear homomorphism and product, 6}
Из равенств
\ShowEq{algebra, linear homomorphism and product, 7}
следует
\ShowEq{algebra, linear homomorphism and product, 8}
Из равенств
\EqRef{algebra, linear homomorphism and product, 5},
\EqRef{algebra, linear homomorphism and product, 8},
следует
\ShowEq{algebra, linear homomorphism and product, 9}
Равенство
\EqRef{algebra, linear homomorphism and product}
следует из равенства
\EqRef{algebra, linear homomorphism and product, 9},
так как векторы базиса $\Basis e_2$
линейно независимы, и $a^{\gi i}$, $b^{\gi i}$ (а следовательно,
$r_1(a^{\gi i})$, $r_1(b^{\gi i})$) - произвольные величины.
\end{proof}

\section{Линейный автоморфизм алгебры кватернионов}
\label{section: Linear Automorphism of Quaternion Algebra}

Определение координат линейного автоморфизма - задача непростая.
В этом разделе мы рассмотрим пример нетривиального линейного автоморфизма
алгебры кватернионов.

\begin{theorem}
Координаты линейного автоморфизма алгебры кватернионов
удовлетворяют системе уравнений
\ShowEq{linear automorphism of quaternion algebra, 1 2 6 0}
\end{theorem}
\begin{proof}
Согласно теоремам
\xRef{1003.1544}{theorem: Quaternion over real field},
\ref{theorem: Morphism of D algebra},
линейный автоморфизм алгебры кватернионов удовлетворяет уравнениям
\ShowEq{linear automorphism of quaternion algebra}
Из равенства
\EqRef{linear automorphism of quaternion algebra}
следует
\ShowEq{linear automorphism of quaternion algebra, 1}
\ShowEq{linear automorphism of quaternion algebra, 2}
Если $\gil=\gi 0$, то из равенства
\ShowEq{linear automorphism of quaternion algebra, 1 0 1}
следует
\ShowEq{linear automorphism of quaternion algebra, 1 0 2}
Из равенства
\EqRef{linear automorphism of quaternion algebra, 1}
для $\gil=\gi 0$ и равенства
\EqRef{linear automorphism of quaternion algebra, 1 0 2},
следует
\ShowEq{linear automorphism of quaternion algebra, 1 0 3}
Если
\ShowEq{l=1,2,3}
то равенство
\EqRef{linear automorphism of quaternion algebra, 1}
можно записать в виде
\ShowEq{linear automorphism of quaternion algebra, 1 1 1}
Из равенств
\EqRef{linear automorphism of quaternion algebra, 1 1 1},
\EqRef{linear automorphism of quaternion algebra, 1 0 3}
и равенств
\ShowEq{linear automorphism of quaternion algebra, 1 1 2}
следует
\ShowEq{linear automorphism of quaternion algebra, 1 1 3}
Из равенств
\EqRef{linear automorphism of quaternion algebra, 1 1 3}
следует
\ShowEq{linear automorphism of quaternion algebra, 1 1 4}
Из равенства
\EqRef{linear automorphism of quaternion algebra, 1 1 4}
следует
\ShowEq{linear automorphism of quaternion algebra, 1 1 5}
Из равенства
\EqRef{linear automorphism of quaternion algebra, 2}
для $\gil=\gi 0$ следует
\ShowEq{linear automorphism of quaternion algebra, 1 2 1}
Из равенств
\ShowEq{linear automorphism of quaternion algebra, 1 2 2}
следует
\ShowEq{linear automorphism of quaternion algebra, 1 2 3}
Из равенств
\EqRef{linear automorphism of quaternion algebra, 1 2 3}
следует\,\footnote{Мы здесь опираемся на то, что алгебра
кватернионов определена над полем действительных чисел.
Если рассматривать алгебру кватернионов над
полем комплексных чисел, то уравнение
\EqRef{linear automorphism of quaternion algebra, 1 2 3}
определяет конус в комплексном пространстве.
Соответственно, у нас шире выбор координат линейного автоморфизма.}
\ShowEq{linear automorphism of quaternion algebra, 1 2 4}
Из равенства
\EqRef{linear automorphism of quaternion algebra, 2}
для $\gil>\gi 0$ следует
\ShowEq{linear automorphism of quaternion algebra, 1 2 7}
Равенства
\EqRef{linear automorphism of quaternion algebra, 1 2 7}
тождественно верны в силу равенств
\EqRef{linear automorphism of quaternion algebra, 1 0 3},
\EqRef{linear automorphism of quaternion algebra, 1 2 4},
\EqRef{linear automorphism of quaternion algebra, 1 1 2}.
Из равенств
\EqRef{linear automorphism of quaternion algebra, 1 2 4},
\EqRef{linear automorphism of quaternion algebra, 1 1 4},
следует
\ShowEq{linear automorphism of quaternion algebra, 1 2 6}
Равенства
\EqRef{linear automorphism of quaternion algebra, 1 2 6 0}
следуют из равенств
\EqRef{linear automorphism of quaternion algebra, 1 2 6}.
\end{proof}

\begin{example}
\label{example: linear automorphism of quaternion algebra, example}
Очевидно, координаты
\ShowEq{linear automorphism of quaternion algebra, example 1}
удовлетворяют уравнению
\EqRef{linear automorphism of quaternion algebra, 1 2 6 0}.
Мы можем убедиться непосредственной проверкой, что
координаты отображения
\ShowEq{linear automorphism of quaternion algebra, example 2}
также удовлетворяют уравнению
\EqRef{linear automorphism of quaternion algebra, 1 2 6 0}.
Матрица координат этого отображения имеет вид
\ShowEq{linear automorphism of quaternion algebra, example 2, 1}
Согласно теореме
\xRef{1003.1544}{theorem: coordinates of linear function, quaternion},
стандартные компоненты отображения $r$ имеют вид
\ShowEq{linear automorphism of quaternion algebra, example 2, 2}
Следовательно, отображение $r$ имеет вид
\ShowEq{linear automorphism of quaternion algebra, example 2, 3}
%\ShowEq{linear automorphism of quaternion algebra, example 2, 4}
\qed
\end{example}


==> D.Module.Russian.tex <==
%auto-ignore

\input{D.Module.Eq}

\chapter{\texorpdfstring{$D$}{D}-модуль}

\section{Модуль над коммутативным кольцом}

\begin{theorem}
\label{theorem: effective representation of the ring}
Пусть кольцо $D$ имеет единицу $e$.
Представление
\ShowEq{f:D->*V}
кольца $D$
в абелевой группе $A$
\AddIndex{эффективно}{effective representation of ring}
тогда и только тогда, когда
из равенства $f(a)=0$ следует $a=0$.
\end{theorem}
\begin{proof}
Сумма преобразований $f$ и $g$ абелевой группы определяется согласно
правилу
\ShowEq{(f+g)(a)=}
Поэтому, рассматривая представление кольца $D$ в
абелевой группе $A$, мы полагаем
\ShowEq{sum of transformations of Abelian group, 1}

Если $a$, $b\in R$
порождают одно и то же преобразование, то
\ShowEq{representation of ring, 1}
для любого $m\in A$.
Из равенства
\EqRef{representation of ring, 1}
следует, что $a-b$ порождает нулевое преобразование
\ShowEq{representation of ring, 2}
Элемент $e+a-b$ порождает тождественное преобразование.
Следовательно, представление $f$ эффективно тогда и только тогда,
когда $a=b$.
\end{proof}

\ShowEq{definition: module over commutative ring}

\ShowTheorem{definition of module over commutative ring}
\begin{proof}
Равенство \EqRef{distributive law, D module, 1} следует
из утверждения, что преобразование $a$ является эндоморфизмом абелевой группы.
Равенство \EqRef{distributive law, D module, 2} следует
из утверждения, что представление
\eqRef{D->*V}{module}
является гомоморфизмом аддитивной группы
кольца $D$.
Равенства \EqRef{associative law, D module} и
\EqRef{unitarity law, D module} следуют
из утверждения, что представление
\eqRef{D->*V}{module}
является
левосторонним представлением мультипликативной группы кольца $D$.
\end{proof}

\begin{theorem}
\label{theorem: set of vectors generated by the set of vectors}
Множество векторов, порождённое множеством векторов
\EqParm{vi V}{=z}
имеет вид
\ShowEq{w=sum vi}
\end{theorem}
\begin{proof}
Мы докажем теорему по индукции, опираясь на теорему
\EqParm{ref theorem: structure of subrepresentations}{=.}

Пусть $k=0$.
Согласно теореме
\EqParm{ref theorem: structure of subrepresentations}{=c}
\ShowEq{X0=v}
Для произвольного
\ShowEq{vk in v}
положим
\ShowEq{ci=dik}
Тогда
\ShowEq{vk=sum vi}
\ShowEq{vk in Jv}
следует из
\EqRef{w=sum vi},
\EqRef{vk=sum vi}.

Пусть
\ShowEq{Xk-1 in Jv}
\begin{itemize}
\item
Пусть
\ShowEq{w12 in Xk-1}
Так как $V$ является абелевой группой,
то согласно утверждению
%\ePrints{1502.04063}
%\ifx\Semafor\ValueOn
\xRefItem{0912.3315}{x1n omega in Xk+1},
%\else
%\xRefItem{8443-0072}{x1n omega in Xk+1},
%\fi
\ShowEq{w1+w2 in Xk}
Согласно утверждениям
\xEqRef{0912.3315}{structure of subrepresentations, 1},
\EqRef{w=sum vi},
существуют $D$\Hyph числа
\ShowEq{ci di}
такие, что
\ShowEq{w12=}
Так как $V$ является абелевой группой,
то из равенства
\EqRef{w12=}
следует, что
\ShowEq{w1+w2=}
Равенство
\ShowEq{w1+w2= 1}
является следствием равенств
\EqRef{distributive law, D module, 2},
\EqRef{w1+w2=}.
Из равенства
\EqRef{w1+w2= 1}
следует, что
\ShowEq{w1+w2 in Jv}
\item
Пусть
\ShowEq{w in Xk-1}
Согласно утверждению
\xRefItem{0912.3315}{ax in Xk+1},
для любого $D$\Hyph числа $a$,
\ShowEq{aw in Xk}
Согласно утверждениям
\xEqRef{0912.3315}{structure of subrepresentations, 1},
\EqRef{w=sum vi},
существуют $D$\Hyph числа
\ShowEq{ci}
такие, что
\ShowEq{w=}
Из равенства
\EqRef{w=}
следует, что
\ShowEq{aw=}
Из равенства
\EqRef{aw=}
следует, что
\ShowEq{aw in Jv}
\end{itemize}
\end{proof}

\begin{convention}
Мы будем пользоваться соглашением Эйнштейна о сумме,
в котором повторяющийся индекс (один вверху и один внизу)
подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av}
\qed
\end{convention}

\begin{definition}
\label{definition: vector linearly dependent on vectors}
{\it
Пусть
\EqParm{vi V}{=z}
- множество векторов.
Выражение
\ShowEq{linear composition of  vectors}
называется
\AddIndex{линейной комбинацией векторов}{linear composition of  vectors}
\ShowEq{vi}
Вектор
\ShowEq{w=ci vi}
называется
\AddIndex{вектором, линейно зависимым от векторов}
{vector linearly dependent on vectors}
\ShowEq{vi}
}
\qed
\end{definition}

\begin{theorem}
\label{theorem: linearly depends on rest of vectors}
Пусть $D$ - поле.
Если уравнение
\ShowEq{ci vi=0}
предполагает существования индекса $\gii=\gij$ такого, что
\ShowEq{cj ne 0}
то вектор $v_{\gij}$
линейно зависит от остальных векторов $v$.
\end{theorem}
\begin{proof}
Теорема является следствием равенства
\ShowEq{vj=sum vi}
и определения
\ref{definition: vector linearly dependent on vectors}.
\end{proof}

Очевидно, что для любого множества векторов $v_{\gii}$,
\ShowEq{0=0vi}

\begin{definition}
\label{definition: linearly independent vectors}
Векторы\,\footnote{Я следую
определению в \citeBib{Serge Lang}, с. 100.}
\ShowEq{Vector A subs row, 1}
$D$\Hyph модуля $A$
\AddIndex{линейно независимы}{linearly independent vectors},
если $c=0$ следует из уравнения
\DrawEq{ci ei=0}{}
В противном случае, векторы \ShowEq{Vector A subs row, 1}
\AddIndex{линейно зависимы}{linearly dependent vectors}.
\qed
\end{definition}

\begin{theorem}
Пусть $D$ - поле.
Множество векторов
\ShowEq{basis, module}
является
\AddIndex{базисом $D$\Hyph векторного пространства}{Basis}
$V$, если векторы $e_{\gii}$
линейно независимы и любой вектор $v\in V$
линейно зависит от векторов $e_{\gii}$.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{basis, module}
- базис $D$\Hyph векторного пространства $V$.
Согласно определению
%\ePrints{1502.04063}
%\ifx\Semafor\ValueOn
\xRef{0912.3315}{definition: basis of representation}
%\else
%\xRef{8443-0072}{definition: basis of representation}
%\fi
и теоремам
\EqParm{ref theorem: structure of subrepresentations}{=c}
\ref{theorem: set of vectors generated by the set of vectors},
произвольный вектор $v\in V$
является линейной комбинацией векторов $e_{\gii}$
\ShowEq{v=vi ei}
Из равенства
\EqRef{v=vi ei}
следует, что множество векторов $v$,
\ShowEq{Vector A subs row, 1}
не является линейно независимым.

Рассмотрим равенство
\DrawEq{ci ei=0}{basis}
Согласно теореме
\ref{theorem: linearly depends on rest of vectors},
если
\ShowEq{cj ne0}
то вектор $e_{\gij}$
линейно зависит от остальных векторов $e$.
Следовательно, множество векторов
\ShowEq{ei I-j}
порождает $D$\Hyph векторное пространство $V$.
Согласно определению
\xRef{0912.3315}{definition: basis of representation},
утверждение
\EqRef{cj ne0}
неверно.
Согласно определению
\ref{definition: linearly independent vectors},
векторы $e_{\gii}$
линейно независимы.
\end{proof}

\begin{definition}
\label{definition: free module over ring}
Множество векторов
\ShowEq{basis, module}
называется\,\footnote{Определение
\ref{definition: free module over ring}
является следствием теоремы
\xRef{0912.3315}{theorem: X is basis of representation}
и замечания
\xRef{0912.3315}{remark: X is basis of representation}.
}
\AddIndex{базисом $D$\Hyph модуля}{basis, module}
$V$, если произвольный вектор $v\in V$
является линейной комбинацией
векторов базиса и произвольный вектор базиса
нельзя представить в виде линейной комбинации
остальных векторов базиса.
$A$ - \AddIndex{свободный модуль над кольцом}{free module over ring} $D$,
если $A$ имеет базис
над кольцом $D$.\,\footnote{Я следую
определению в \citeBib{Serge Lang}, с. 103.}
\qed
\end{definition}

\ShowEq{definition: coordinates of vector}

\section{Линейное отображение \texorpdfstring{$D$}{D}-модуля}

\ShowEq{definition: linear map from A1 to A2, commutative module}

\ShowTheorem{linear map from A1 to A2, commutative module}
\begin{proof}
Из определения
\ref{definition: linear map from A1 to A2, commutative module}
и теоремы
\xRef{4993-2400}{theorem: morphism of representations of algebra, reduce}
следует, что
отображение $f$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\EqRef{linear map from A1 to A2, 1 1}).
Равенство
\EqRef{linear map from A1 to A2, 1 2}
следует из равенства
\xEqRef{4993-2400}{morphism of representations of F algebra}.
\end{proof}

\ePrints{1502.04063}
\ifx\Semafor\ValueOn
\ShowTheorem{sum of linear maps, D module}
\begin{proof}
Согласно теореме
\ref{theorem: linear map from A1 to A2, commutative module}
\DrawEq{f(v+w)=fv+fw}{sum of maps}
\DrawEq{f(dv)=dfv}{sum of maps}
\ShowEq{g(v+w)=gv+gw}
\ShowEq{g(dv)=dgv}
Равенство
\ShowEq{sum of maps, 31, D module}
является следствием равенств
\EqRef{sum of maps, D module},
\eqRef{f(v+w)=fv+fw}{sum of maps},
\EqRef{g(v+w)=gv+gw}.
Равенство
\ShowEq{sum of maps, 32, D module}
является следствием равенств
\EqRef{sum of maps, D module},
\eqRef{f(dv)=dfv}{sum of maps},
\EqRef{g(dv)=dgv}.
Из равенств
\EqRef{sum of maps, 31, D module},
\EqRef{sum of maps, 32, D module}
и теоремы
\ref{theorem: linear map from A1 to A2, commutative module}
следует, что отображение
\EqRef{sum of maps, 1, D module}
является линейным отображением $D$\Hyph модулей.

Из равенства
\EqRef{sum of maps, D module}
следует, что отображение
\ShowEq{0:A1->A2}
является нулём операции сложения
\ShowEq{0+f=f}
Из равенства
\EqRef{sum of maps, D module}
следует, что отображение
\ShowEq{-f:A1->A2}
является отображением, обратным отображению \(f\)
\ShowEq{f-f=0,v}
Из равенства
\ShowEq{sum of maps, 4, D module}
следует, что сумма отображений коммутативно.
\end{proof}

\begin{theorem}
\label{theorem: product of linear map over scalar, D module}
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,D module}
\ShowEq{product of map over scalar, 1, D module}
определённое равенством
\ShowEq{product of map over scalar, D module}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является линейным отображением.
Представление
\ShowEq{a:LA12->LA12}
кольца $D$ в абелевой группе
\EqParm{L(A;B)}{A=12,=z}
порождает структуру $D$\Hyph модуля.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: linear map from A1 to A2, commutative module}
\DrawEq{f(v+w)=fv+fw}{product of map over scalar}
\DrawEq{f(dv)=dfv}{product of map over scalar}
Равенство
\ShowEq{product of map over scalar, 31, D module}
является следствием равенств
\EqRef{product of map over scalar, D module},
\eqRef{f(v+w)=fv+fw}{product of map over scalar}.
Равенство
\ShowEq{product of map over scalar, 32, D module}
является следствием равенств
\EqRef{product of map over scalar, D module},
\eqRef{f(dv)=dfv}{product of map over scalar}.
Из равенств
\EqRef{product of map over scalar, 31, D module},
\EqRef{product of map over scalar, 32, D module}
и теоремы
\ref{theorem: linear map from A1 to A2, commutative module}
следует, что отображение
\EqRef{product of map over scalar, 1, D module}
является линейным отображением $D$\Hyph модулей.

Равенство
\DrawEq{(p+q)f=pf+qf}{D module}
является следствием равенства
\ShowEq{(a+b)f(v)=}
Равенство
\DrawEq{p(qf)=(pq)f}{D module}
является следствием равенства
\ShowEq{(ab)f=}
Из равенств
\eqRef{(p+q)f=pf+qf}{D module},
\eqRef{p(qf)=(pq)f}{D module},
следует, что отображение
\EqRef{a:LA12->LA12}
является представлением кольца $D$
в абелевой группе
\EqParm{L(A;B)}{A=12,=.}
Согласно определению
\ref{definition: module over commutative ring}
и теореме
\ref{theorem: sum of linear maps, D module},
абелевая группа
\EqParm{L(A;B)}{A=12,=z}
является $D$\Hyph модулем.
\end{proof}
\fi

\begin{theorem}
\label{theorem: linear map, 0, D algebra}
Пусть отображение
\EqParm{f:A->B}{f=f,A=12}
является линейным отображением $D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
Тогда
\ShowEq{linear map, 0, D algebra}
\end{theorem}
\begin{proof}
Следствие равенства
\ShowEq{linear map, 0, D algebra, 1}
\end{proof}

\section{Полилинейное отображение \texorpdfstring{$D$}{D}-модуля}

\begin{definition}
\label{definition: polylinear map of modules}
{\it
Пусть $D$ - коммутативное кольцо.
Приведенный полиморфизм $D$\Hyph модулей
$A_1$, ..., $A_n$ в $D$\Hyph модуль $S$
\ShowEq{polylinear map of algebras}
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль
$S$.
Обозначим
\ShowEq{set polylinear maps An}
множество $n$\hyph линейных отображений
$D$\Hyph модуля $A$ ($A_1=...=A_n=A$)
в $D$\Hyph модуль
$S$.
}
\qed
\end{definition}

\begin{theorem}
\label{theorem: polylinear map of modules}
Пусть $D$ - коммутативное кольцо.
Полилинейное отображение $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$
\ShowEq{polylinear map of algebras}
удовлетворяет равенствам
\DrawEq{f(ai+bi)=fai+fbi}{}
\DrawEq{f(pai)=pfai}{}
\ShowEq{polylinear map of algebras, 1}
\end{theorem}
\begin{proof}
Теорема является следствием определений
\ref{definition: polymorphism of representations},
\ref{definition: linear map from A1 to A2, commutative module}
и теоремы
\ref{theorem: linear map from A1 to A2, commutative module}.
\end{proof}

\ShowTheorem{sum of polylinear maps, module}
\begin{proof}
Согласно теореме
\ref{theorem: polylinear map of modules}
\DrawEq{f(ai+bi)=fai+fbi}{sum of maps}
\DrawEq{f(pai)=pfai}{sum of maps}
\ShowEq{g(ai+bi)=gai+gbi}
\ShowEq{g(pai)=pgai}
Равенство
\ShowEq{sum of maps, 31, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps},
\EqRef{g(ai+bi)=gai+gbi}.
Равенство
\ShowEq{sum of maps, 32, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(pai)=pfai}{sum of maps},
\EqRef{g(pai)=pgai}.
Из равенств
\EqRef{sum of maps, 31, polylinear},
\EqRef{sum of maps, 32, polylinear}
и теоремы
\ref{theorem: polylinear map of modules}
следует, что отображение
\EqRef{sum of maps, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Пусть
\ShowEq{module of polylinear maps, 1}
Для любого
\ShowEq{module of polylinear maps, 2}
Следовательно, сумма полилинейных отображений коммутативна и ассоциативна.

Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{0:A1n->S}
является нулём операции сложения
\ShowEq{0+f=f 1n}
Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{-f:A1n->S}
является отображением, обратным отображению \(f\)
\ShowEq{f-f=0}
так как
\ShowEq{f-f=0 1n}
Из равенства
\ShowEq{sum of maps, 4, polylinear}
следует, что сумма отображений коммутативно.
Следовательно, множество $\\$
\ShowEq{module of polylinear maps}
является абелевой группой.
\end{proof}

\ePrints{1502.04063}
\ifx\Semafor\ValueOff
\ShowEq{corollary: sum of linear maps, D module}
\fi

\begin{theorem}
\label{theorem: module of polylinear maps}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,polylinear}
\ShowEq{product of map over scalar, 1, polylinear}
определённое равенством
\ShowEq{product of map over scalar, polylinear}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является полилинейным отображением.
Представление
\ShowEq{a:LA1n->LA1n}
кольца $D$ в абелевой группе
\ShowEq{module of polylinear maps}
порождает структуру $D$\Hyph модуля.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: polylinear map of modules}
\DrawEq{f(ai+bi)=fai+fbi}{product of map over scalar}
\DrawEq{f(pai)=pfai}{product of map over scalar}
Равенство
\ShowEq{product of map over scalar, 31, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{product of map over scalar}.
Равенство
\ShowEq{product of map over scalar, 32, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(pai)=pfai}{product of map over scalar}.
Из равенств
\EqRef{product of map over scalar, 31, polylinear},
\EqRef{product of map over scalar, 32, polylinear}
и теоремы
\ref{theorem: polylinear map of modules}
следует, что отображение
\EqRef{product of map over scalar, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Равенство
\DrawEq{(p+q)f=pf+qf}{polylinear}
является следствием равенства
\ShowEq{(p+q)f=pf+qf 1}
Равенство
\DrawEq{p(qf)=(pq)f}{polylinear}
является следствием равенства
\ShowEq{p(qf)=(pq)f 1}
Из равенств
\eqRef{(p+q)f=pf+qf}{polylinear},
\eqRef{p(qf)=(pq)f}{polylinear},
следует, что отображение
\EqRef{a:LA1n->LA1n}
является представлением кольца $D$
в абелевой группе
\ShowEq{module of polylinear maps}.
Так как указанное представление эффективно,
то, согласно определению
\ref{definition: module over commutative ring}
и теореме
\ref{theorem: sum of polylinear maps, module},
абелевая группа
\EqParm{L(A;B)}{A=12,=z}
является $D$\Hyph модулем.
\end{proof}

\ePrints{1502.04063}
\ifx\Semafor\ValueOff
\begin{corollary}
\label{corollary: product of linear map over scalar, D module}
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,D module}
\ShowEq{product of map over scalar, 1, D module}
определённое равенством
\ShowEq{product of map over scalar, D module}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является линейным отображением.
Представление
\ShowEq{a:LA12->LA12}
кольца $D$ в абелевой группе
\EqParm{L(A;B)}{A=12,=z}
порождает структуру $D$\Hyph модуля.
\qed
\end{corollary}
\fi

\section{\texorpdfstring{$D$}{D}-модуль \texorpdfstring{$\mathcal L(D;A\rightarrow B)$}{L(D;A->B)}}

\begin{theorem}
\label{theorem: L(p;L(q;B))=L(p+q;B)}
\ShowEq{L(p;L(q;B))=L(p+q;B)}
\end{theorem}
\begin{proof}
\end{proof}

\begin{theorem}
\label{theorem: basis h in L(A->D)}
Пусть
\ShowEq{basis e, i in I}
базис $D$\Hyph модуля $A$.
Множество
\ShowEq{basis h in L(A->D)}
является базисом $D$\Hyph модуля
\EqParm{L(A;B)}{A=AD,=.}
\end{theorem}
\begin{proof}

\begin{lemma}
\label{lemma: maps hi are linear independent}
{\it
Отображения $h^{\gii}$ линейно независимы.
}
\end{lemma}

{\sc Доказательство.}
Пусть существуют $D$\Hyph числа $c_{\gii}$ такие, что
\ShowEq{ci hi =0}
Тогда для любого $A$\Hyph числа $e_{\gij}$
\ShowEq{cj=0}
Лемма является следствием определения
\ref{definition: linearly independent vectors}.
\hfill\(\odot\)

\begin{lemma}
\label{lemma: map f is linear composition of maps hi}
{\it
Отображение
\ShowEq{f in L(A->D)}
является линейной композицией отображений $h^{\gii}$.
}
\end{lemma}

{\sc Доказательство.}
Для любого $A$\Hyph числа $a$,
\ShowEq{a in basis e}
равенство
\ShowEq{hi a =}
является следствием равенств
\EqRef{basis h in L(A->D)},
\EqRef{a in basis e}
и теоремы
\ref{theorem: linear map from A1 to A2, commutative module}.
Равенство
\ShowEq{f(a)=}
является следствием равенства
\EqRef{hi a =}.
Равенство
\ShowEq{f=...hi}
является следствием равенств
\ShowEq{ref proof basis h in L(A->D)}
\hfill\(\odot\)

Теорема является следствием лемм
\ref{lemma: maps hi are linear independent},
\ref{lemma: map f is linear composition of maps hi}
и определения
\ref{definition: free module over ring}.
\end{proof}

\begin{theorem}
\label{theorem: basis of D-module L(xA->B)}
Пусть $D$ - коммутативное кольцо.
Пусть
\ShowEq{basis e in Ai}
базис $D$\Hyph модуля $A_i$, $i=1$, ..., $n$.
Пусть
\ShowEq{basis e in B}
базис $D$\Hyph модуля $B$.
Множество
\ShowEq{basis h, xA->B}
является базисом $D$\Hyph модуля
\EqParm{L(A;B)}{A=xAB,=.}
\end{theorem}
\begin{proof}

\begin{lemma}
\label{lemma: maps hij are linear independent}
{\it
Отображения
\EqParm{hij}{=z}
линейно независимы.
}
\end{lemma}

{\sc Доказательство.}
Пусть существуют $D$\Hyph числа
\ShowEq{cij}
такие, что
\ShowEq{cij hij =0}
Тогда для любого набора индексов
\ShowEq{cij ei=0}
Следовательно,
\ShowEq{cij=0}
Лемма является следствием определения
\ref{definition: linearly independent vectors}.
\hfill\(\odot\)

\begin{lemma}
\label{lemma: map f is linear composition of maps hij}
{\it
Отображение
\ShowEq{f in L(xA->B)}
является линейной композицией отображений
\EqParm{hij}{=.}
}
\end{lemma}

{\sc Доказательство.}
Для любого $A_1$\Hyph числа $a_1$
\ShowEq{a1 in basis e1}
...,
для любого $A_n$\Hyph числа $a_n$
\ShowEq{an in basis en}
равенство
\ShowEq{hij a =}
является следствием равенств
\EqRef{basis h, xA->B},
\EqRef{a1 in basis e1},
\EqRef{an in basis en}
и теоремы
\ref{theorem: linear map from A1 to A2, commutative module}.
Равенство
\ShowEq{f(a1n)=}
является следствием равенств
\EqRef{a1 in basis e1},
\EqRef{an in basis en}.
Так как
\ShowEq{fe1n in B}
то
\ShowEq{fe1n=}
Равенство
\ShowEq{f(a1n)= 1}
является следствием равенств
\EqRef{hij a =},
\EqRef{f(a1n)=},
\EqRef{fe1n=}.
Равенство
\ShowEq{f=...hij}
является следствием равенств
\ShowEq{ref proof basis h, xA->B}
\hfill\(\odot\)

Теорема является следствием лемм
\ref{lemma: maps hij are linear independent},
\ref{lemma: map f is linear composition of maps hij}
и определения
\ref{definition: free module over ring}.
\end{proof}

\ShowTheorem{L(An;B) is free D module}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: basis of D-module L(xA->B)}.
\end{proof}

\section{Тензорное произведение \texorpdfstring{$D$}{D}-модулей}
\label{Section: Tensor Product of Modules}

\begin{theorem}
\label{theorem: commutative ring is Abelian multiplicative Omega group}
Коммутативное кольцо $D$ является
абелевой мультипликативной $\Omega$\Hyph группой.
\end{theorem}
\begin{proof}
Мы полагаем, что произведение $\circ$ в кольце $D$
определён согласно правилу
\ShowEq{a circ b=ab}
Так как произведение в кольце дистрибутивно относительно сложения,
теорема является следствием определений
\ref{definition: multiplicative Omega group},
\ref{definition: Abelian multiplicative Omega group}.
\end{proof}

\begin{theorem}
\label{theorem: there exists tensor product of modules}
\AddIndex{Тензорное произведение}{tensor product}
\ShowEq{tensor product of modules}
$D$\Hyph модулей $A_1$, ..., $A_n$ существует.
\end{theorem}
\begin{proof}
Теорема является следствием определения
\ref{definition: module over commutative ring}
и теорем
\ref{theorem: tensor product of representations},
\ref{theorem: commutative ring is Abelian multiplicative Omega group}.
\end{proof}

\begin{theorem}
\label{theorem: Tensor product is distributive over sum}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$ - $D$\Hyph модули.
Тензорное произведение дистрибутивно относительно сложения
\ShowEq{tensors 1, tensor product}
Представление кольца $D$
в тензорном произведении определено равенством
\ShowEq{tensors 2, tensor product}
\end{theorem}
\begin{proof}
Равенство
\EqRef{tensors 1, tensor product}
является следствием равенства
\EqRef{tensors 1, representation, tensor product}.
Равенство
\EqRef{tensors 2, tensor product}
является следствием равенства
\EqRef{tensors 2, representation, tensor product}.
\end{proof}

\begin{theorem}
\label{theorem: tensor product and polylinear map}
Пусть $A_1$, ..., $A_n$ -
модули над коммутативным кольцом $D$.
Пусть
\ShowEq{map f, 1, tensor product}
полилинейное отображение,
определённое равенством
\ShowEq{map f, tensor product}
Пусть
\ShowEq{map g, tensor product}
полилинейное отображение в $D$\Hyph модуль $V$.
Существует линейное отображение
\ShowEq{map h, tensor product}
такое, что диаграмма
\ShowEq{map gh, tensor product}
коммутативна.
Отображение \(h\) определено равенством
\ShowEq{g=h, tensor product}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: tensor product and polymorphism}
и определений
\ref{definition: linear map from A1 to A2, commutative module},
\ref{definition: polylinear map of modules}.
\end{proof}

\begin{theorem}
\label{theorem: V times->V otimes}
Отображение
\ShowEq{V times->V otimes}
является полилинейным отображением.
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: B times->B otimes}
и определения
\ref{definition: polylinear map of modules}.
\end{proof}

\begin{theorem}
\label{theorem: standard component of tensor, algebra}
Тензорное произведение $\Tensor A$ свободных
конечномерных модулей
$A_1$, ..., $A_n$
над коммутативным кольцом $D$ является свободным
конечномерным модулем.

Пусть
\ShowEq{tensor product of algebras, basis i}
- базис модуля $A_i$ над кольцом $D$.
Произвольный тензор $a\in\Tensor A$ можно представить в виде
\ShowEq{standard component of tensor}
\ShowEq{tensor canonical representation, algebra}
Мы будем называть выражение
$\ShowSymbol{standard component of tensor}{}$
\AddIndex{стандартной компонентой тензора}
{standard component of tensor}.
\end{theorem}
\begin{proof}
Вектор $a_i\in A_i$ имеет разложение
\ShowEq{expansion i relative basis}
относительно базиса $\Basis e_i$.
Из равенств
\EqRef{tensors 1, tensor product},
\EqRef{tensors 2, tensor product}
следует
\ShowEq{expansion i relative basis, 1}
Так как множество тензоров $\Tensor a$
является множеством образующих модуля $\Tensor A$,
то тензор
$a\in\Tensor A$
можно записать в виде
\ShowEq{tensor canonical representation 1}
где
\ShowEq{tensor canonical representation 2}
Положим
\ShowEq{tensor canonical representation 3}
Тогда равенство \EqRef{tensor canonical representation 1}
примет вид
\EqRef{tensor canonical representation, algebra}.

Следовательно, множество тензоров $\TensorBasis i$
является множеством образующих модуля $\Tensor A$.
Так как размерность модуля $A_i$, $i=1$, ..., $n$, конечна,
то конечно множество тензоров $\TensorBasis i$.
Следовательно, множество тензоров $\TensorBasis i$
содержит базис модуля $\Tensor A$, и модуль $\Tensor A$
является свободным модулем над кольцом $D$.
\end{proof}




==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%202%*%*D вектор строка
   {$*D$\Hyph вектор строка}%
   {row *D vector}%
\Index%192%*%*D- векторное пространство
   {$*D$\Hyph векторное пространство}%
   {*D vector space}%
\Index%9%*%CR произведение
   {\CR произведение}%
   {cr-product}%
\Index%66%*%RC произведение
   {\RC произведение}%
   {rc-product}%
\SetIndexSpace%
\Index%1%1%1-форма
   {$1$\Hyph форма}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A алгебра многочленов над D алгеброй
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%818%A%A число
   {$A$\Hyph число}%
   {A number}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) map}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%575%A%Astar векторное пространство
   {$A\star$\Hyph векторное пространство}%
   {Astar vector space}%
\Index%660%A%Astar- модуль
   {$A\star$\Hyph модуль}%
   {Astar-module}%
\Index%864%A%A-представление в Omega алгебре
   {$A$\Hyph представление в $\Omega$\Hyph алгебре}%
   {A representation of algebra}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%799%B%b множество
   {$B$\Hyph множество}%
   {B set}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%304%C%crd вектор
   {\crd вектор}%
   {crd vector}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%23%D%d аффинное пространство
   {$D$\Hyph аффинное пространство}%
   {d affine space}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%92%D%D* вектор столбец
   {$D*$\Hyph вектор столбец}%
   {column D* vector}%
\Index%93%D%D* вектор строка
   {$D*$\Hyph вектор строка}%
   {row D* vector}%
\Index%87%D%D*- векторное пространство матриц
   {$D*$\hyph векторное пространство матриц}%
   {matrices vector space}%
\Index%40%D%D*-векторное пространство
   {$D*$\hyph векторное пространство}%
   {D* vector space}%
\Index%156%D%D*-модуль
   {$D*$\Hyph модуль}%
   {D*-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%38%D%dcr производная Гато отображения f D- векторного пространства V в D- векторное пространство W
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%200%D%drc вектор
   {\dcr вектор}%
   {dcr vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\Index%845%N%n-арная операция на множестве
   {$n$\Hyph арная операция на множестве}%
   {n-ary operation on set}%
\SetIndexSpace%
\Index%4%R%j i-RC квазидетерминант
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главная минорная матрица
   {\RC главная минорная матрица}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%600%R%RCcirc вырожденная матрица
   {$\RCcirc$\Hyph вырожденная матрица}%
   {RCcirc singular matrix}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица
   {$\RCcirc$\Hyph невырожденная матрица}%
   {RCcirc nonsingular matrix}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%111%R%rcd аффинный базис
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%13%R%rcd производная Гато отображения f D-векторного пространства V в D-векторное пространство W
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\Index%510%R%частная rcd производная Гато отображения fb по переменной xa
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\SetIndexSpace%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%735%S%starD аффинное пространство
   {$\star D$\Hyph аффинное пространство}%
   {starD affine space}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%185%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%823%T%T_1 пространство
   {$T_1$\Hyph пространство}%
   {T1 space}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%187%T%Tstar- представление расслоенной группы
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%830%А%абелевая мультипликативная Omega группа
   {абелевая мультипликативная $\Omega$\Hyph группа}%
   {Abelian multiplicative Omega group}%
\Index%869%А%абелевая полугруппа
   {абелевая полугруппа}%
   {Abelian semigroup}%
\Index%284%А%абсолютная величина
   {абсолютная величина}%
   {absolute value}%
\Index%859%А%автоморфизм
   {автоморфизм}%
   {automorphism}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%22%А%автоморфизм векторного пространства
   {автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%805%А%аддитивное отображение
   {аддитивное отображение}%
   {additive map}%
\Index%99%А%активное *G представление
   {активное \sT{G}представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%569%А%активное представление группы в многообразии базисов представления
   {активное представление группы $G(f)$ в многообразии базисов представления}%
   {active representation in basis manifold}%
\Index%715%А%активное преобразование многообразия базисов башни представлений
   {активное преобразование многообразия базисов башни представлений}%
   {active transformation of basis, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов представления
   {активное преобразование многообразия базисов представления}%
   {active transformation of basis, representation}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%808%А%алгебра Бореля
   {алгебра Бореля}%
   {Borel algebra}%
\Index%741%А%алгебра кватернионов
   {алгебра кватернионов}%
   {quaternion algebra}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%797%А%алгебра множеств
   {алгебра множеств}%
   {algebra of sets}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%167%А%алгебра с делением
   {алгебра с делением}%
   {division algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%907%А%альтернация полилинейного отображения
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
\Index%779%А%антилинейное отображение
   {антилинейное отображение}%
   {antilinear map}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%849%А%арность
   {арность}%
   {arity}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%89%А%ассоциативная Omega группа
   {ассоциативная $\Omega$\Hyph группа}%
   {associative Omega group}%
\Index%866%А%ассоциативная операция
   {ассоциативная операция}%
   {associative operation}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%682%А%аффинное представление группы Ли
   {аффинное представление группы Ли}%
   {affine representation of Lie group}%
\Index%758%А%аффинное преобразование
   {аффинное преобразование}%
   {affine transformation}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%734%А%аффинное пространство
   {аффинное пространство}%
   {affine space}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\Index%579%А%аффинный функционал
   {аффинный функционал}%
   {affine functional}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%203%Б%базис crd векторного пространства
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
\Index%197%Б%базис D векторного пространства
   {базис $D$\Hyph векторного пространства}%
   {basis, D vector space}%
\Index%106%Б%базис dcr векторного пространства
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
\Index%16%Б%базис drc векторного пространства
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
\Index%24%Б%базис rcd векторного пространства
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%26%Б%базис в векторном расслоении
   {базис в векторном расслоении}%
   {basis, vector bundle}%
\Index%115%Б%базис векторного пространства
   {базис векторного пространства}%
   {Basis}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%659%Б%базис модуля
   {базис модуля}%
   {basis, module}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%49%Б%базис, дуальный базису
   {базис, дуальный базису}%
   {basis dual to basis}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Vector{\Omega}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор представления
   {бесконечно малый генератор представления}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\Index%798%Б%борелевское множество
   {борелевское множество}%
   {Borel set}%
\Index%803%Б%борелевское отображение
   {борелевское отображение}%
   {Borel-measurable map}%
\SetIndexSpace%
\Index%901%В%вектор
   {вектор}%
   {vector}%
\Index%123%В%вектор Киллинга второго рода
   {вектор Киллинга второго рода}%
   {Killing vector second type}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%833%В%вектор, линейно зависимый от векторов
   {вектор, линейно зависимый от векторов}%
   {vector linearly dependent on vectors}%
\Index%727%В%векторное пространство над полем
   {векторное пространство над полем}%
   {vector space over field}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%398%В%вертикальная компонента вектора
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Index%687%В%вертикальное подпространство
   {вертикальное подпространство}%
   {vertical subspace}%
\Index%33%В%вертикальный вектор
   {вертикальный вектор}%
   {vertical vector}%
\Index%481%В%взаимно простые  A числа
   {взаимно простые  $A$\Hyph числа}%
   {relatively prime A numbers}%
\Index%908%В%внешнее произведение
   {внешнее произведение}%
   {exterior product}%
\Index%910%В%внешний дифференциал
   {внешний дифференциал}%
   {exterior differential}%
\Index%163%В%внешняя мера
   {внешняя мера}%
   {outer measure}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%231%В%всюду плотное множество
   {всюду плотное множество}%
   {everywhere dense subset}%
\Index%70%В%вторая аксиома счётности
   {вторая аксиома счётности}%
   {second axiom of countability}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%781%В%выпуклое множество
   {выпуклое множество}%
   {convex set}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\SetIndexSpace%
\Index%871%Г%геодезический эффект
   {геодезический эффект}%
   {geodetic effect}%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Index%698%Г%геометрический объект в координатном представлении, определённом в Omega_2- алгебре
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%719%Г%геометрический объект в координатном представлении, определённом в кортеже Omega- алгебр
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Index%704%Г%геометрический объект типа
   {геометрический объект типа $H$}%
   {geometric object of type H, representation g}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%700%Г%геометрический объект, определённый в Omega_2- алгбре
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%722%Г%геометрический объект, определённый в кортеже Omega- алгебр
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Index%838%Г%гиперболический косинус
   {гиперболический косинус}%
   {hyperbolic cosine}%
\Index%837%Г%гиперболический синус
   {гиперболический синус}%
   {hyperbolic sine}%
\Index%767%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%885%Г%голоморфное отображение
   {голоморфное отображение}%
   {holomorphic map}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%854%Г%гомоморфизм
   {гомоморфизм}%
   {homomorphism}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%861%Г%гомоморфный образ
   {гомоморфный образ}%
   {homomorphic image}%
\Index%73%Г%горизонтальная компонента вектора
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Index%686%Г%горизонтальное подпространство
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Index%765%Г%горизонтальный вектор
   {горизонтальный вектор}%
   {horizontal vector}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%613%Г%группа линейных преобразований
   {группа линейных преобразований}%
   {linear transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%586%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%865%Д%декартова степень
   {декартова степень}%
   {Cartesian power}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%655%Д%декартова степень систем подмножеств
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Index%390%Д%декартово произведение групп
   {декартово произведение групп}%
   {Cartesian product of groups}%
\Index%199%Д%декартово произведение мер
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%625%Д%декартово произведение систем подмножеств
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Index%825%Д%декартово произведением Omega алгебр
   {декартово произведением \(\Omega\)\Hyph алгебр}%
   {Cartesian product of Omega algebras}%
\Index%598%Д%деление без остатка
   {деление без остатка}%
   {division without remainder}%
\Index%573%Д%деление с остатком
   {деление с остатком}%
   {division with remainder}%
\Index%820%Д%делитель многочлена
   {делитель многочлена}%
   {divisor of polynomial}%
\Index%814%Д%делитель нуля
   {делитель нуля}%
   {zero divisor}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%157%Д%дифференциал отображения
   {дифференциал отображения}%
   {differential of map}%
\Index%902%Д%дифференциальная p форма
   {дифференциальная $p$\Hyph форма}%
   {differential p form}%
\Index%909%Д%дифференциальная форма степени p
   {дифференциальная форма степени $p$}%
   {differential form of degree p}%
\Index%877%Д%дифференцируемое отображение
   {дифференцируемое отображение}%
   {differentiable map}%
\Index%78%Д%долгота
   {долгота}%
   {longitude}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%796%Е%единица кольца множеств
   {единица кольца множеств}%
   {unit of ring of sets}%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\Index%44%Е%единичный интервал
   {единичный интервал}%
   {unit interval}%
\Index%875%Е%естественный гомоморфизм
   {естественный гомоморфизм}%
   {natural homomorphism}%
\SetIndexSpace%
\Index%662%З%закон ассоциативности
   {закон ассоциативности}%
   {associative law}%
\Index%672%З%закон дистрибутивности
   {закон дистрибутивности}%
   {distributive law}%
\Index%673%З%закон унитарности
   {закон унитарности}%
   {unitarity law}%
\Index%807%З%замкнутый шар
   {замкнутый шар}%
   {closed ball}%
\Index%80%З%замыкание множества
   {замыкание множества}%
   {closure of set}%
\Index%912%З%звёздное множество
   {звёздное множество}%
   {starlike set}%
\SetIndexSpace%
\Index%459%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%800%И%измеримое отображение
   {измеримое отображение}%
   {measurable map}%
\Index%164%И%измеримое по Лебегу множество
   {измеримое по Лебегу множество}%
   {Lebesgue measurable}%
\Index%855%И%изоморфизм
   {изоморфизм}%
   {isomorphism}%
\Index%31%И%изоморфизм векторных пространств
   {изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%913%И%интеграл дифференциальной 1 формы вдоль пути
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
\Index%680%И%интеграл отображения
   {интеграл отображения}%
   {integral of map}%
\Index%911%И%интегрируемая форма
   {интегрируемая форма}%
   {integrable form}%
\Index%693%И%интегрируемое отображение
   {интегрируемое отображение}%
   {integrable map}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%599%К%каноническое представление деления с остатком
   {каноническое представление деления с остатком}%
   {canonical representation of division with remainder}%
\Index%726%К%каноническое частное от деления
   {каноническое частное от деления}%
   {canonical remainder of the division}%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%177%К%категория левосторонних представлений
   {категория левосторонних представлений}%
   {category of left-side representations}%
\Index%176%К%категория левосторонних представлений Omega1 алгебры A
   {категория левосторонних представлений $\Omega$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
\Index%887%К%категория представлений
   {категория представлений}%
   {category of representations}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%842%К%квадратное уравнение
   {квадратное уравнение}%
   {quadratic equation}%
\Index%841%К%квадратный корень
   {квадратный корень}%
   {square root}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%75%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of maps}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%794%К%кольцо множеств
   {кольцо множеств}%
   {ring of sets}%
\Index%577%К%кольцо множеств, порождённое полукольцом множеств
   {кольцо множеств, порождённое полукольцом множеств}%
   {ring of sets generated by semiring}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%867%К%коммутативная операция
   {коммутативная операция}%
   {commutative operation}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%815%К%компактное множество
   {компактное множество}%
   {compact set}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%879%К%компонента производной
   {компонента производной}%
   {component of derivative}%
\Index%883%К%компонента производной второго порядка
   {компонента производной второго порядка}%
   {component of derivative of Second Order}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%873%К%конгруенция
   {конгруенция}%
   {congruence}%
\Index%170%К%конечное разложение множества
   {конечное разложение множества}%
   {finite expansion of set}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%210%К%координатное векторное расслоение
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
\Index%697%К%координатное представление в Omega_2- алгебре
   {координатное представление в $\Omega_2$\Hyph алгебре}%
   {coordinate representation, Omega_2 algebra}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%664%К%координатное представление вектора
   {координатное представление вектора}%
   {coordinate representation of vector}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%916%К%координаты
   {координаты}%
   {coordinates}%
\Index%25%К%координаты базиса
   {координаты базиса}%
   {coordinates of basis}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%676%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%701%К%координаты геометрического объекта в Omega_2- алгбре
   {координаты геометрического объекта в $\Omega_2$\Hyph алгбре $M$}%
   {coordinates of geometric object, representation g}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%221%К%координаты геометрического объекта в координатном представлении
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometric object, coordinate vector space}%
\Index%721%К%координаты геометрического объекта в координатном пространстве башни представлений
   {координаты геометрического объекта в координатном пространстве башни представлений}%
   {coordinates of geometric object, coordinate tower of representations}%
\Index%699%К%координаты геометрического объекта в координатном пространстве представления
   {координаты геометрического объекта в координатном пространстве представления}%
   {coordinates of geometric object, coordinate representation}%
\Index%723%К%координаты геометрического объекта в кортеже Omega- алгебр
   {координаты геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinates of geometric object, tower of representations g}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%737%К%координаты точки rcd аффинного пространства относительно базиса
   {координаты точки \rcd аффинного пространства относительно базиса}%
   {coordinates in rcd affine space}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%558%К%координаты элемента представления относительно множества
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%535%К%кортеж координат элемента относительно кортежа множеств
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%533%К%кортеж множеств образующих башни подпредставлений
   {кортеж множеств образующих башни подпредставлений}%
   {tuple of generating sets of tower subrepresentations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%840%К%косинус
   {косинус}%
   {cosine}%
\Index%904%К%косо симметричное полилинейное отображение
   {косо симметричное полилинейное отображение}%
   {skew symmetric polylinear map}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%821%К%коэффициент многочлена
   {коэффициент многочлена}%
   {coefficient of polynomial}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%166%Л%лебегово продолжение меры
   {лебегово продолжение меры}%
   {Lebesgue extension of measure}%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%896%Л%левое D векторное пространство
   {левое $D$\Hyph векторное пространство}%
   {left D vector space}%
\Index%585%Л%левое D векторное пространство столбцов
   {левое $D$\hyph векторное пространство столбцов}%
   {left vector space of columns}%
\Index%576%Л%левое D векторное пространство строк
   {левое $D$\hyph векторное пространство строк}%
   {left vector space of rows}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%899%Л%левостороннее A представление
   {левостороннее $A_1$\Hyph представление}%
   {left-side A representation}%
\Index%184%Л%левостороннее представление
   {левостороннее представление}%
   {left-side representation}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%892%Л%левостороннее произведение
   {левостороннее произведение}%
   {left-side product}%
\Index%665%Л%левостороннее произведение вектора на скаляр
   {левостороннее произведение вектора на скаляр}%
   {left-side product of vector over scalar}%
\Index%271%Л%левостороннее произведение отображения на скаляр
   {левостороннее произведение отображения на скаляр}%
   {left-side product of map over scalar}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%895%Л%левый D модуль
   {левый $D$\Hyph модуль}%
   {left D module}%
\Index%513%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%812%Л%левый делитель нуля
   {левый делитель нуля}%
   {left zero divisor}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль
   {левый модуль}%
   {left module}%
\Index%661%Л%левый модуль над D- алгеброй A
   {левый модуль над $D$\Hyph алгеброй $A$}%
   {left module over algebra}%
\Index%731%Л%левый сдвиг модуля
   {левый сдвиг модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {left shift, fibered group}%
\Index%88%Л%линейная комбинация векторов
   {линейная комбинация векторов}%
   {linear combination of  vectors}%
\Index%832%Л%линейная комбинация векторов
   {линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index%32%Л%линейная оболочка в векторном пространстве
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Index%98%Л%линейнное отображение, порождённое отображением
   {линейное отображение, порождённое отображением}%
   {linear map generated by map}%
\Index%688%Л%линейно зависимое множество A- модуля
   {линейно зависимое множество $A$\Hyph модуля}%
   {linear dependent vectors, module}%
\Index%20%Л%линейно зависимые векторные поля
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%21%Л%линейно зависимые векторы
   {линейно зависимые векторы}%
   {linearly dependent vectors}%
\Index%34%Л%линейно независимые векторы
   {линейно независимые векторы}%
   {linearly independent vectors}%
\Index%37%Л%линейное G* представление
   {линейное \Ts{G}представление}%
   {linear G* representation}%
\Index%35%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%608%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {linear representation of Lie group}%
\Index%740%Л%линейное преобразование rcd аффинного пространства
   {линейное преобразование \rcd аффинного пространства}%
   {linear transformation, rcd affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%769%Л%линейный гомоморфизм
   {линейный гомоморфизм}%
   {linear homomorphism}%
\Index%397%Л%линейный функционал
   {линейный функционал}%
   {linear functional}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%894%М%матрица
   {матрица}%
   {matrix}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear maps}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of maps}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%890%М%матрица Якоби отображения
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
\Index%161%М%мера
   {мера}%
   {measure}%
\Index%165%М%мера Лебега
   {мера Лебега}%
   {Lebesgue measure}%
\Index%835%М%метод последовательного дифференцирования
   {метод последовательного дифференцирования}%
   {method of successive differentiation}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%257%М%многообразие базисов \rcd аффинного пространства
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%536%М%многообразие базисов представления
   {многообразие базисов представления}%
   {basis manifold representation F algebra}%
\Index%261%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%804%М%многочлен
   {многочлен}%
   {polynomial}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%847%М%множество допускает операцию
   {множество допускает операцию}%
   {set admits operation}%
\Index%846%М%множество замкнуто относительно операции
   {множество замкнуто относительно операции}%
   {set is closed with respect to operation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%331%М%множество образующих подпредставления
   {множество образующих подпредставления}%
   {generating set of subrepresentation}%
\Index%332%М%множество образующих представления
   {множество образующих представления}%
   {generating set of representation}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%356%М%множество, плотное в множестве
   {множество, плотное в множестве}%
   {dense in set}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%860%М%может быть вложена
   {может быть вложена}%
   {can be embeded}%
\Index%856%М%мономорфизм
   {мономорфизм}%
   {monomorphism}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни представлений в башню представлений
   {морфизм из башни представлений в башню представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%828%М%мультипликативная Omega группа
   {мультипликативная $\Omega$\Hyph группа}%
   {multiplicative Omega group}%
\Index%829%М%мультипликативное отображение
   {мультипликативное отображение}%
   {multiplicative map}%
\Index%85%М%открытое множество
   {открытое множество}%
   {open set}%
\SetIndexSpace%
\Index%207%Н%наибольший общий делитель
   {наибольший общий делитель}%
   {highest common factor}%
\Index%763%Н%направление над коммутативным кольцом
   {направление над коммутативным кольцом}%
   {direction over commutative ring}%
\Index%738%Н%начало системы координат star D аффинного пространства
   {начало системы координат $\star D$\Hyph аффинного пространства}%
   {origin of coordinate system of starD affine space}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor}%
\Index%330%Н%невырожденный эндоморфизм представления
   {невырожденный эндоморфизм представления}%
   {regular endomorphism of representation}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%29%Н%независимые точки
   {независимые точки}%
   {independent points}%
\Index%870%Н%нейтральный элемент операции
   {нейтральный элемент операции}%
   {neutral element of operation}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%834%Н%неопределённый интеграл
   {неопределённый интеграл}%
   {indefinite integral}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%668%Н%непрерывный базис
   {непрерывный базис}%
   {continues basis}%
\Index%346%Н%норма в D- алгебре
   {норма в $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%460%Н%норма в D-модуле
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%675%Н%норма на Omega группе
   {норма на $\Omega$\Hyph группе}%
   {norm on Omega group}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%657%Н%норма операции
   {норма операции}%
   {norm of operation}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%801%Н%норма представления
   {норма представления}%
   {norm of representation}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%792%Н%нормированная Omega группа
   {нормированная $\Omega$\Hyph группа}%
   {normed Omega group}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%364%Н%нормированный D-модуль
   {нормированный $D$\Hyph модуль}%
   {normed D module}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\Index%852%Н%носитель Omega-алгебры
   {носитель $\Omega$\Hyph алгебры}%
   {carrier of Omega-algebra}%
\SetIndexSpace%
\Index%848%О%область операторов
   {область операторов}%
   {operator domain}%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%482%О%общий делитель
   {общий делитель}%
   {common factor}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство
   {однородное пространство}%
   {homogeneous space}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%689%О%однородный многочлен степени
   {однородный многочлен степени $n$}%
   {homogeneous polynomial of power}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%766%О%одночлен степени
   {одночлен степени $k$}%
   {monomial of power}%
\Index%844%О%операция на множестве
   {операция на множестве}%
   {operation on set}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%914%О%определённый интеграл
   {определённый интеграл}%
   {definite integral}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear map}%
\Index%893%О%орбита представления
   {орбита представления}%
   {orbit of representation}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%484%О%остаток от деления
   {остаток от деления}%
   {remainder of the division}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%793%О%открытый шар
   {открытый шар}%
   {open ball}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%886%О%отображение согласовано с операцией
   {отображение согласовано с операцией}%
   {map is compatible with operation}%
\Index%876%О%отображение сопряжения
   {отображение сопряжения}%
   {map of conjugation}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\Index%677%О%отображение, проективное над коммутативным кольцом
   {отображение, проективное над коммутативным кольцом}%
   {map projective over commutative ring}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг rcd аффинного пространства
   {параллельный сдвиг \rcd аффинного пространства}%
   {parallel shift, rcd affine space}%
\Index%587%П%парные представления
   {парные представления}%
   {twin representations}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное *G представление
   {пассивное \sT{G}представление}%
   {passive *G representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%695%П%пассивное представление группы в многообразии базисов представления
   {пассивное представление группы $G(f)$ в многообразии базисов представления}%
   {passive representation in basis manifold}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%570%П%пассивное преобразование многообразия базисов представления
   {пассивное преобразование многообразия базисов представления}%
   {passive transformation of basis, representation}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%863%П%перестановка
   {перестановка}%
   {permutation}%
\Index%853%П%подалгебра Omega-алгебры
   {подалгебра $\Omega$\Hyph алгебры}%
   {subalgebra of Omega-algebra}%
\Index%230%П%подгруппа Omega группы
   {подгруппа $\Omega$\Hyph группы}%
   {subgroup of Omega group}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%806%П%полиаддитивное отображение
   {полиаддитивное отображение}%
   {polyadditive map}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%345%П%полилинейное косо симметричное отображение
   {полилинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%764%П%полная мера
   {полная мера}%
   {complete measure}%
\Index%811%П%полная нормированная Omega группа
   {полная нормированная $\Omega$\Hyph группа}%
   {complete Omega group}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%868%П%полугруппа
   {полугруппа}%
   {semigroup}%
\Index%169%П%полукольцо множеств
   {полукольцо множеств}%
   {semiring of sets}%
\Index%186%П%пополнение нормированной Omegaгруппы
   {пополнение нормированной $\Omega$\Hyph группы}%
   {completion of normed Omega group}%
\Index%19%П%пополнение представления
   {пополнение представления}%
   {completion of representation}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%816%П%последовательность сходится
   {последовательность сходится}%
   {sequence converges}%
\Index%578%П%последовательность сходится почти всюду
   {последовательность сходится почти всюду}%
   {converges almost everywhere}%
\Index%817%П%последовательность сходится равномерно
   {последовательность сходится равномерно}%
   {sequence converges uniformly}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%898%П%правое D векторное пространство
   {правое $D$\Hyph векторное пространство}%
   {right D vector space}%
\Index%671%П%правое D векторное пространство столбцов
   {правое $D$\hyph векторное пространство столбцов}%
   {right vector space of columns}%
\Index%654%П%правое D векторное пространство строк
   {правое $D$\hyph векторное пространство строк}%
   {right vector space of rows}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%900%П%правостороннее A представление
   {правостороннее $A_1$\Hyph представление}%
   {right-side A representation}%
\Index%355%П%правостороннее представление
   {правостороннее представление}%
   {right-side representation}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%891%П%правостороннее произведение
   {правостороннее произведение}%
   {right-side product}%
\Index%674%П%правостороннее произведение вектора на скаляр
   {правостороннее произведение вектора на скаляр}%
   {right-side product of vector over scalar}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%897%П%правый D модуль
   {правый $D$\Hyph модуль}%
   {right D module}%
\Index%242%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%813%П%правый делитель нуля
   {правый делитель нуля}%
   {right zero divisor}%
\Index%42%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль
   {правый модуль}%
   {right module}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%702%П%представитель геометрического объекта в drc векторном пространстве
   {представитель геометрического объекта в \drc векторном пространстве}%
   {representative of geometric object, drc vector space}%
\Index%703%П%представитель геометрического объекта в Omega_2- алгбре
   {представитель геометрического объекта в $\Omega_2$\Hyph алгбре}%
   {representative of geometric object, representation g}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%724%П%представитель геометрического объекта в кортеже Omega- алгебр
   {представитель геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {representative of geometric object, tower of representations g}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%82%П%представление Omega1 алгебры A в Omega2 алгебре *A
   {\sT{A}представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре}%
   {*A representation of algebra}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%90%П%представление в Omega2- алгебре A*
   {\Ts{A}представление в $\Omega_2$\Hyph алгебре}%
   {A* representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%117%П%представление, сопряжённое представлению
   {представление, сопряжённое представлению}%
   {representation conjugated to representation}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%915%П%преобразование сопряжения
   {преобразование сопряжения}%
   {conjugation transformation}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%843%П%приведенное квадратное уравнение
   {приведенное квадратное уравнение}%
   {reduced quadratic equation}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%831%П%приведенный морфизм представлений
   {приведенный морфизм представлений}%
   {reduced morphism of representations}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%705%П%принцип инвариантности в \drc векторном пространстве
   {принцип инвариантности в \drc векторном пространстве}%
   {invariance principle}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%385%П%принцип инвариантности в векторном пространстве
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index%384%П%принцип инвариантности в представлении универсальной алгебры
   {принцип инвариантности в представлении универсальной алгебры}%
   {invariance principle, representation g}%
\Index%162%П%продолжение меры
   {продолжение меры}%
   {extension of measure}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%195%П%проективное отображение непрерывно по направлению над полем
   {проективное отображение непрерывно по направлению над полем}%
   {projective map is continuous in direction over field}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%663%П%произведение колец множеств
   {произведение колец множеств}%
   {product of rings of sets}%
\Index%172%П%произведение мер
   {произведение мер}%
   {product of measures}%
\Index%666%П%произведение многочленов
   {произведение многочленов}%
   {product of polynomials}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%395%П%произведением объектов в категории
   {произведением объектов в категории}%
   {product of objects in category}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%882%П%производная Гато второго порядка
   {производная второго порядка}%
   {derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%878%П%производная отображения
   {производная отображения}%
   {derivative of map}%
\Index%884%П%производная порядка n
   {производная порядка $n$}%
   {derivative of Order n}%
\Index%483%П%простое A число
   {простое $A$\Hyph число}%
   {prime A number}%
\Index%810%П%простое отображение
   {простое отображение}%
   {simple map}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит G* представления
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
\Index%684%П%пространство орбит левостороннего представления
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%412%П%прямое произведение G* представлений
   {прямое произведение \Ts{G}представлений}%
   {direct product of G* representations}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%826%П%прямое произведением Omega алгебр
   {прямое произведением \(\Omega\)\Hyph алгебр}%
   {direct product of Omega algebras}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный изоморфизм}%
   {fibered coordinate isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%782%Р%ряд сходится нормально
   {ряд сходится нормально}%
   {series converges normally}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%862%С%свободное представление
   {свободное представление}%
   {free representation}%
\Index%441%С%свободное представление группы
   {свободное представление группы}%
   {free representation of group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль над кольцом
   {свободный модуль над кольцом}%
   {free module over ring}%
\Index%517%С%связное множество
   {связное множество}%
   {connected set}%
\Index%583%С%связность в главном расслоении
   {связность в главном расслоении}%
   {connection in principal bundle}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%906%С%симметрирование полилинейного отображения
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%903%С%симметричное полилинейное отображение
   {симметричное полилинейное отображение}%
   {symmetric polylinear map}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%214%С%симплекс
   {симплекс}%
   {simplex}%
\Index%839%С%синус
   {синус}%
   {sine}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%201%С%система линейных уравнений
   {система линейных уравнений}%
   {system of linear equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%683%С%сопряжённое аффинное пространство
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Index%789%С%сопряжённое векторное пространство
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%881%С%стандартная компонента производной
   {стандартная компонента производной}%
   {standard component of derivative}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%880%С%стандартное представление производной
   {стандартное представление производной}%
   {derivative, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%822%С%старший коэффициент многочлена
   {старший коэффициент многочлена}%
   {leading coefficient of polynomial}%
\Index%171%С%степень меры
   {степень меры}%
   {power of measure}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%667%С%сумма многочленов
   {сумма многочленов}%
   {sum of polynomials}%
\Index%351%С%сумма отображений
   {сумма отображений}%
   {sum of maps}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%323%С%суперпозиция координат эндоморфизма представления и элемента
   {суперпозиция координат эндоморфизма представления $f$ и элемента $m$}%
   {superposition of coordinates, representation}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\Index%168%С%сферические координаты
   {сферические координаты}%
   {spherical coordinates}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%802%Т%тензор, обратный тензору
   {тензор, обратный тензору}%
   {inverse tensor}%
\Index%652%Т%тензорная степень
   {тензорная степень}%
   {tensor power}%
\Index%480%Т%тензорное произведение
   {тензорное произведение}%
   {tensor product}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%824%Т%точка прикосновения множества
   {точка прикосновения множества}%
   {contact point of set}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\SetIndexSpace%
\Index%851%У%универсальная алгебра
   {универсальная алгебра}%
   {universal algebra}%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%493%У%уравнение Киллинга
   {уравнение Киллинга}%
   {Killing equation}%
\Index%494%У%уравнение Киллинга второго рода
   {уравнение Киллинга второго рода}%
   {Killing equation second type}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%77%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%508%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis, division ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%511%Ч%частная dcr производная Гато отображения f^b по переменной x^a
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%888%Ч%частная производная
   {частная производная}%
   {partial derivative}%
\Index%889%Ч%частная производная второго порядка
   {частная производная второго порядка}%
   {partial derivative of second order}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%475%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\Index%827%Ч%частное от деления
   {частное от деления}%
   {quotient divided by}%
\Index%905%Ч%чётность перестановки
   {чётность перестановки}%
   {parity of permutation}%
\SetIndexSpace%
\Index%501%Ш%широта
   {широта}%
   {latitude}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%836%Э%экспонента
   {экспонента}%
   {exponent}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%858%Э%эндоморфизм
   {эндоморфизм}%
   {endomorphism}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%857%Э%эпиморфизм
   {эпиморфизм}%
   {epimorphism}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%872%Э%эффект увлечения системы отсчёта
   {эффект увлечения системы отсчёта}%
   {frame dragging effect}%
\Index%516%Э%эффективное G* представление
   {эффективное \Ts{G}представление}%
   {effective G* representation}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%500%Э%эффективное представление
   {эффективное представление}%
   {effective representation}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%874%Я%ядро гомоморфизма
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности G* представления
   {ядро неэффективности \Ts{G}представления}%
   {kernel of inefficiency of G* representation}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%
\SetIndexSpace%
\Index%809%M%mu измеримое отображение
   {$\mu$\Hyph измеримое отображение}%
   {mu measurable map}%
\SetIndexSpace%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%656%O%Omega кольцо
   {\(\Omega\)\Hyph кольцо}%
   {Omega ring}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\Index%850%O%Omega-алгебра
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
\SetIndexSpace%
\Index%658%S%sigma алгебра множеств
   {$\sigma$\Hyph алгебра множеств}%
   {sigma algebra of sets}%
\Index%795%S%sigma кольцо множеств
   {$\sigma$\Hyph кольцо множеств}%
   {sigma ring of sets}%
\Index%762%S%sigma-аддитивная мера
   {\(\sigma\)\Hyph аддитивная мера}%
   {sigma-additive measure}%

\CloseIndex


==> Polymorphism.Russian.tex <==
%auto-ignore
\input{Polymorphism.Eq}

\ePrints{1102.5168}
\ifx\Semafor\ValueOff
\chapter{Тензорное произведение представлений}
\fi

\section{Полиморфизм представлений}

\begin{definition}
\label{definition: polymorphism of representations}
Пусть
\EqParm{A1n}{=z}
- $\Omega_1$\Hyph алгебры.
Пусть
\ShowEq{B1n}
- $\Omega_2$\Hyph алгебры.
Пусть для любого \Kn
\ShowEq{representation A B k}
представление $\Omega_1$\Hyph алгебры $A_k$
в $\Omega_2$\Hyph алгебре $B_k$.
Пусть
\ShowEq{representation A B}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Отображение
\ShowEq{polymorphism of representation}
называется
\AddIndex{полиморфизмом представлений}
{polymorphism of representations}
$f_1$, ..., $f_n$ в представление $f$,
если для любого \Kn
при условии, что все переменные кроме переменных
\ShowEq{ak bk in}
имеют заданное значение, отображение $(r,R)$
является морфизмом представления $f_k$ в представление $f$.

Если $f_1=...=f_n$, то мы будем говорить, что отображение $(r,R)$
является полиморфизмом представления $f_1$ в представление $f$.

Если $f_1=...=f_n=f$, то мы будем говорить, что отображение $(r,R)$
является полиморфизмом представления $f$.
\qed
\end{definition}

\begin{theorem}
Пусть отображение $(r,R)$ является полиморфизмом
представлений $f_1$, ..., $f_n$ в представление $f$.
Отображение $(r,R)$ удовлетворяет равенству
\ShowEq{polymorphism of representation, ak}
Пусть $\omega_1\in\Omega_1(p)$.
Для любого \Kn отображение $r$ удовлетворяет равенству
\ShowEq{polymorphism of representation, omega1}
Пусть $\omega_2\in\Omega_2(p)$.
Для любого \Kn отображение $R$ удовлетворяет равенству
\ShowEq{polymorphism of representation, omega2}
\end{theorem}
\begin{proof}
Равенство
\EqRef{polymorphism of representation, ak}
следует из определения
\ref{definition: polymorphism of representations}
и равенства
\ShowEq{ref morphism of representations of F algebra, definition, 2m}
Равенство
\EqRef{polymorphism of representation, omega1}
следует из утверждения, что для любого \Kn
при условии, что все переменные кроме переменной $x_k\in A_k$
имеют заданное значение, отображение $r$
является гомоморфизмом $\Omega_1$\Hyph алгебры $A_k$ в $\Omega_1$\Hyph алгебру $A$.
Равенство
\EqRef{polymorphism of representation, omega2}
следует из утверждения, что для любого \Kn
при условии, что все переменные кроме переменной $m_k\in B_k$
имеют заданное значение, отображение $R$
является гомоморфизмом $\Omega_2$\Hyph алгебры $B_k$ в $\Omega_2$\Hyph алгебру $B$.
\end{proof}

\begin{definition}
\label{definition: reduced polymorphism of representations}
Пусть
\ShowEq{set of universal algebras 1}
- универсальные алгебры.
Пусть для любого \Kn
\ShowEq{representation A B k 1}
эффективное представление $\Omega_1$\Hyph алгебры $A_k$
в $\Omega_2$\Hyph алгебре $B_k$.
Пусть
\ShowEq{representation A B}
эффективное представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Отображение
\ShowEq{reduced polymorphism of representation}
называется
\AddIndex{приведенным полиморфизмом представлений}
{reduced polymorphism of representations}
$f_1$, ..., $f_n$ в представление $f$,
если для любого \Kn
при условии, что все переменные кроме переменной $x_k\in B_k$
имеют заданное значение, отображение $R$
является приведенным морфизмом представления $f_k$ в представление $f$.

Если $f_1=...=f_n$, то мы будем говорить, что отображение $R$
является приведенным полиморфизмом представления $f_1$ в представление $f$.

Если $f_1=...=f_n=f$, то мы будем говорить, что отображение $R$
является приведенным полиморфизмом представления $f$.
\qed
\end{definition}

\begin{theorem}
Пусть отображение $R$ является приведенным полиморфизмом
эффективных представлений $f_1$, ..., $f_n$ в эффективное представление $f$.
Для любого \Kn отображение $R$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, ak}
Пусть $\omega_2\in\Omega_2(p)$.
Для любого \Kn отображение $R$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, omega2}
\end{theorem}
\begin{proof}
Равенство
\EqRef{reduced polymorphism of representation, ak}
следует из определения
\ref{definition: reduced polymorphism of representations}
и равенства
\ShowEq{eqref morphism of representations of F algebra}
Равенство
\EqRef{reduced polymorphism of representation, omega2}
следует из утверждения, что для любого \Kn
при условии, что все переменные кроме переменной $m_k\in B_k$
имеют заданное значение, отображение $R$
является гомоморфизмом $\Omega_2$\Hyph алгебры $B_k$ в $\Omega_2$\Hyph алгебру $B$.
\end{proof}

Мы также будем говорить, что отображение $(r,R)$ является полиморфизмом
представлений в $\Omega_2$\Hyph алгебрах $B_1$, ..., $B_n$ в представление
в $\Omega_2$\Hyph алгебре $B$. Аналогично, мы будем говорить,
что отображение $R$ является приведенным полиморфизмом
представлений в $\Omega_2$\Hyph алгебрах $B_1$, ..., $B_n$ в представление
в $\Omega_2$\Hyph алгебре $B$.

\ePrints{1102.5168}
\ifx\Semafor\ValueOn
\begin{example}
Полилинейное отображение векторных пространств является приведенным
полиморфизмом векторных пространств.
\qed
\end{example}
\fi

Сравнение определений
\ref{definition: polymorphism of representations}
и
\ref{definition: reduced polymorphism of representations}
показывает, что существует разница между этими двумя
формами полиморфизма.
Особенно хорошо это различие видно при сравнении равенств
\EqRef{polymorphism of representation, ak}
и
\EqRef{reduced polymorphism of representation, ak}.
Если мы хотим иметь возможность выразить приведенный полиморфизм представлений
через полиморфизм представлений, то мы должны потребовать,
два условия:
\begin{enumerate}
\item
Представление $f$ универсальной алгебры содержит тождественное преобразование
$\delta$. Следовательно, существует $e\in A$ такой, что $f(e)=\delta$.
Не нарушая общности, мы положим, что выбор $e\in A$
не зависит от того,
какое представление $f_1$, ..., $f_n$ мы рассматриваем.
\item
Для любого \Kn
\ShowEq{polymorphism and reduced polymorphism 2}
\end{enumerate}
Тогда, при условии $a_i=e$, $i\ne k$, равенство
\EqRef{polymorphism of representation, ak}
имеет вид
\ShowEq{polymorphism of representation 1, ak}
Очевидно, что равенство
\EqRef{polymorphism of representation 1, ak}
совпадает с равенством
\EqRef{reduced polymorphism of representation, ak}.

Похожая задача появляется при анализе приведенного полиморфизма представлений.
Пользуясь равенством
\EqRef{reduced polymorphism of representation, ak},
мы можем записать выражение
\ShowEq{reduced polymorphism of representation 1, ak}
либо в виде
\ShowEq{reduced polymorphism of representation 2, ak}
либо в виде
\ShowEq{reduced polymorphism of representation 3, ak}
%Однако в равенстве
%\EqRef{reduced polymorphism of representation 3, ak}
%не очевидно, в каком порядке мы должны рассматривать суперпозицию
%отображений $f(a_k)$ и $f(a_l)$.
Отображения
\ShowEq{reduced polymorphism of representation 41, ak}
являются гомоморфизмами $\Omega_2$\Hyph алгебры $B$.
Следовательно, отображение
\ShowEq{reduced polymorphism of representation 42, ak}
является гомоморфизмом $\Omega_2$\Hyph алгебры $B$.
Однако, не всякая $\Omega_1$\Hyph алгебра $A$ имеет такой $a$
(зависящий от $a_k$ и $a_l$),
что
\ShowEq{reduced polymorphism of representation 4, ak}

Если представление $f$ однотранзитивно
и для любых $A$\Hyph чисел $a$, $b$ существует $A$\Hyph число $c$ такое, что
\ShowEq{f(c)=f(a)f(b)}
то равенство
\EqRef{f(c)=f(a)f(b)}
определяет $A$\Hyph число $c$ единственным образом.
Следовательно,
мы можем определить умножение
\DrawEq{c=ab}{}
таким образом, что
\DrawEq{f(ab)=f(a)f(b)}{representation}

\ifx\texFuture\Defined
\begin{theorem}
Пусть
\ShowEq{omega in 1}
Умножения дистрибутивно относительно операция $\omega$
\ShowEq{a omega=omega a left}
\ShowEq{a omega=omega a right}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{representation A B}
однотранзитивное представление такое, что 
\DrawEq{f(ab)=f(a)f(b)}{distributive}

Согласно равенству
\eqRef{f(ab)=f(a)f(b)}{distributive}
\ShowEq{f(a omega)}
Поскольку отображение $f$ является гомоморфизмом
$\Omega_1$\Hyph алгебра,
из равенства
\EqRef{f(a omega)}
следует, что
\ShowEq{f(a omega) 1}
\end{proof}
\fi

\begin{definition}
\label{definition: multiplicative Omega group}
{\it
Пусть произведение
\DrawEq{c=ab}{}
является операцией $\Omega_1$\Hyph алгебры $A$.
Положим
\ShowEq{Omega=...-o}
Для любой операции
\ShowEq{omega in p}
умножение дистрибутивно относительно операция $\omega$
\ShowEq{a omega=omega a left}
\ShowEq{a omega=omega a right}
$\Omega_1$\Hyph алгебра $A$ называется
\AddIndex{мультипликативной $\Omega$\Hyph группой}
{multiplicative Omega group}.\,\footnote{
Определение мультипликативной $\Omega$\Hyph группы
похоже на определение
\ShowEq{ref Omega group}
$\Omega$\Hyph группы.
Однако, $\Omega$\Hyph группа предполагает сложение
как групповую операцию. Для нас существенно,
что групповая операция мультипликативной $\Omega$\Hyph группы является произведением.
Кроме того, операция $\omega$ $\Omega$\Hyph группы
дистрибутивна относительно сложения.
В мультипликативной $\Omega$\Hyph группе,
произведение дистрибутивно относительно операции $\omega$.
}
}
\qed
\end{definition}

\begin{definition}
\label{definition: multiplicative map}
{\it
Пусть $A$, $B$ -
мультипликативные $\Omega$\Hyph группы.
Отображение
\ePrints{5148-4632,1502.04063,5114-6019}
\ifx\Semafor\ValueOff
\ShowEq{f:A->B}
\else
\EqParm{f:A->B}{f=f,A=AB}
\fi
называется
\AddIndex{мультипликативным}{multiplicative map},
если
\DrawEq{f(ab)=f(a)f(b)}{}
}
\qed
\end{definition}

\begin{theorem}
\label{theorem: multiplicative map}
Однотранзитивное представление
мультипликативной $\Omega$\Hyph группы
является мультипликативным отображением.
\end{theorem}
\begin{proof}
Утверждение является следствием равенства
\eqRef{f(ab)=f(a)f(b)}{representation}
и определения
\ref{definition: multiplicative map}.
\end{proof}

Однако утверждение теоремы
\ref{theorem: multiplicative map}
недостаточно, чтобы доказать равенство выражений
\EqRef{reduced polymorphism of representation 2, ak}
и
\EqRef{reduced polymorphism of representation 3, ak}.

\begin{definition}
\label{definition: Abelian multiplicative Omega group}
{\it
Если
\ShowEq{Abelian multiplicative Omega group}
то мультипликативная $\Omega$\Hyph группа называется
\AddIndex{абелевой}{Abelian multiplicative Omega group}.
}
\qed
\end{definition}

\begin{theorem}
Пусть
\ShowEq{f:A->M}
эффективное представление
абелевой мультипликативной $\Omega$\Hyph группы $A$.
Тогда
\ShowEq{reduced polymorphism of representation 23, ak}
\end{theorem}
\begin{proof}
Из равенств
\EqRef{reduced polymorphism of representation 2, ak},
\EqRef{reduced polymorphism of representation 3, ak},
\eqRef{f(ab)=f(a)f(b)}{representation},
\EqRef{Abelian multiplicative Omega group}
следует, что
\ShowEq{reduced polymorphism of representation 23 1, ak}
Равенство
\EqRef{reduced polymorphism of representation 23, ak}
является следствием равенства
\EqRef{reduced polymorphism of representation 23 1, ak}.
\end{proof}

\begin{theorem}
\label{theorem: reduced polymorphism of representation, ak}
Пусть $A$ - абелевая мультипликативная $\Omega$\Hyph группа.
Пусть $R$ - приведенный полиморфизм
эффективных представлений $f_1$, ..., $f_n$ в эффективное представление $f$.
Тогда для любых $k$, $l$, $k=1$, ..., $n$, $l=1$, ..., $n$,
\ShowEq{reduced polymorphism of representation 5, ak}
\end{theorem}
\begin{proof}
Равенство
\EqRef{reduced polymorphism of representation 5, ak}
непосредственно следует из равенства
\EqRef{reduced polymorphism of representation, ak}.
\end{proof}

\begin{theorem}
\label{theorem: existence of reduced polymorphism, a omega b omega}
Пусть
\ShowEq{->B 12}
эффективные представления
абелевой мультиплиткативной $\Omega_1$\Hyph группы $A$
в $\Omega_2$\Hyph алгебрах
\ShowEq{B 12}
Допустим $\Omega_2$\Hyph алгебра имеет 2 операции, а именно
\ShowEq{w1p w2q}
Необходимым условием существования приведенного полиморфизма
\ShowEq{R:B1B2->B}
является равенство 
\ShowEq{a omega b omega =}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{a in 1 b in 2}
Согласно равенству
\EqRef{reduced polymorphism of representation, omega2},
выражение
\ShowEq{R aw1 aw2}
может иметь $2$ значения
\ShowEq{R aw1 aw2 1}
\ShowEq{R aw1 aw2 2}
Из равенств
\EqRef{R aw1 aw2 1},
\EqRef{R aw1 aw2 1}
следует, что
\ShowEq{R aw1 aw2 1=2}
Следовательно, выражение
\EqRef{R aw1 aw2}
определенно корректно тогда и только тогда, когда равенство
\EqRef{R aw1 aw2 1=2}
верно.
Положим
\ShowEq{a=Rij}
Равенство
\EqRef{a omega b omega =}
является следствием равенств
\EqRef{R aw1 aw2 1=2},
\EqRef{a=Rij}.
\end{proof}

\begin{theorem}
Существует приведенный полиморфизм эффективного представления
абелевой мультиплиткативной $\Omega$\Hyph группы
в абелевой группе.
\end{theorem}
\begin{proof}
Поскольку операция сложения в абелевой группе
коммутативна и ассоциативна,
то теорема является следствием теоремы
\ref{theorem: existence of reduced polymorphism, a omega b omega}.
\end{proof}

\begin{theorem}
\label{theorem: no reduced polymorphism in ring}
Не существует приведенный полиморфизм эффективного представления
абелевой мультиплиткативной $\Omega$\Hyph группы
в кольце.
\end{theorem}
\begin{proof}
В кольце определены две операции: сложение, которое
коммутативно и ассоциативно, и произведение, которое
дистрибутивно относительно сложения.
Согласно теореме
\ref{theorem: existence of reduced polymorphism, a omega b omega},
если существует полиморфизм эффективного представления в кольцо,
то сложение и произведение должны удовлетворять равенству
\ShowEq{a * b + =}
Однако правая часть равенства
\EqRef{a * b + =}
имеет вид
\ShowEq{a+a a+a}
Следовательно, равенство
\EqRef{a * b + =}
не верно.
\end{proof}

\ePrints{1102.5168}
\ifx\Semafor\ValueOn
\begin{remark}
Возможно, что полиморфизм представлений существует
только для эффективного представления в
Абелевая группе.
Однако это утверждение пока не доказано.
\qed
\end{remark}
\else
\begin{question}
Возможно, что полиморфизм представлений существует
только для эффективного представления в
Абелевая группе.
Однако это утверждение пока не доказано.
\qed
\end{question}
\fi

%\,\footnote{Если в $\Omega_1$\Hyph алгебре
%определенно коммутативное произведение с единицей,
%а представление $f$ удовлетворяет равенству
%\[
%f(ab)=f(a)\circ f(b)
%\]
%то мы положим
%\[
%r(a_1,...,a_n)=a_1...a_n
%\]
%}

%Поэтому в дальнейшем мы будем требовать существование тождественного
%отображения в представлении $f$ и существование отображения $r$,
%удовлетворяющего равенству
%\EqRef{polymorphism and reduced polymorphism 2}.

\section{Конгруэнция}

\begin{theorem}
\label{theorem: maps and kernel equivalence}
Пусть $N$ - отношение эквивалентности
на множестве $A$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
отображения\,\footnote{Утверждение леммы аналогично утверждению 
на с. \citeBib{Serge Lang}-94.}
\ShowEq{maps category}
Мы определим морфизм $f_1\rightarrow f_2$
как отображение $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{maps category, diagram}
Отображение
\ShowEq{maps category, universal}
является универсально отталкивающим в категории $\mathcal A$.\,\footnote{Определение
универсального объекта смотри в определении
на с. \citeBib{Serge Lang}-47.}
\end{theorem}
\begin{proof}
Рассмотрим диаграмму
\ShowEq{maps category, universal, diagram}
\ShowEq{maps category, universal, ker}
Из утверждения
\EqRef{maps category, universal, ker}
и равенства
\ShowEq{maps category 1}
следует
\ShowEq{maps category 2}
Следовательно, мы можем однозначно определить отображение $h$
с помощью равенства
\ShowEq{maps category, h}
\end{proof}

\begin{theorem}
\label{theorem: morphisms representations, B B/N}
Пусть
\ShowEq{representation A B}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Пусть $N$ - такая конгруэнция\,\footnote{Смотри
определение конгруэнции на с. \citeBib{Cohn: Universal Algebra}-71.}
на $\Omega_2$\Hyph алгебре $B$, что любое преобразование
$h\in {}^*B$ согласованно с конгруэнцией $N$.
Существует представление
\ShowEq{representation B/N}
$\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $B/N$
и отображение
\ShowEq{morphisms representations, B B/N}
является приведенным морфизмом представления $f$
в представление $f_1$
\ShowEq{morphisms representations, B B/N 1}
\end{theorem}
\begin{proof}
Любой элемент множества $B/N$ мы можем представить в виде $j(a)$, $a\in B$.

Согласно теореме
\citeBib{Cohn: Universal Algebra}-II.3.5, мы можем определить
единственную структуру $\Omega_2$\Hyph алгебры на множестве $B/N$.
Если $\omega\in\Omega_2(p)$,
то мы определим операцию $\omega$ на множестве $B/N$
согласно равенству (3) на странице \citeBib{Cohn: Universal Algebra}-73
\ShowEq{omega B/N}

Также как в доказательстве теоремы
\ShowEq{ref decompositions of morphism of representations}
мы можем определить представление
\ShowEq{representation B/N}
с помощью равенства
\ShowEq{representation B/N 1}
Равенство
\EqRef{representation B/N 1}
можно представить с помощью диаграммы
\ShowEq{representation B/N 2}
Пусть $\omega\in\Omega_2(p)$.
Так как отображения $f(a)$ и $j$
являются гомоморфизмами $\Omega_2$\Hyph алгебры, то
\ShowEq{representation B/N 3}
Из равенства \EqRef{representation B/N 3}
следует, что
отображение $f_1(a)$ является гомоморфизмом $\Omega_2$\Hyph алгебры.
Из равенства
\EqRef{representation B/N 1}
и
\ShowEq{ref reduced morphism of representations}
следует, что отображение $j$ является приведенным морфизмом представления $f$
в представление $f_1$.
\end{proof}

\begin{theorem}
\label{theorem: morphism representations and kernel equivalence}
Пусть
\ShowEq{representation A B}
представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Пусть $N$ - такая конгруэнция
на $\Omega_2$\Hyph алгебре $B$, что любое преобразование
$h\in {}^*B$ согласованно с конгруэнцией $N$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
приведенные морфизмы представлений\,\footnote{Утверждение леммы аналогично утверждению 
на с. \citeBib{Serge Lang}-94.}
\ShowEq{morphisms category}
где $S_1$, $S_2$ - $\Omega_2$\Hyph алгебры и
\ShowEq{representation of algebra in S1 S2}
представления $\Omega_1$\Hyph алгебры $A$.
Мы определим морфизм $R_1\rightarrow R_2$
как приведенный морфизм представлений $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{morphisms category, diagram}
Приведенный морфизм $\mathrm{nat}\,N$ представления $f$
в представление $f_1$
(теорема \ref{theorem: morphisms representations, B B/N})
является универсально отталкивающим в категории $\mathcal A$.\,\footnote{Определение
универсального объекта смотри в определении
на с. \citeBib{Serge Lang}-47.}
\end{theorem}
\begin{proof}
Существование и единственность отображения $h$,
для которого коммутативна диаграмма
\ShowEq{morphisms category, universal, diagram}
следует из теоремы
\ref{theorem: maps and kernel equivalence}.
Следовательно, мы можем однозначно определить отображение $h$
с помощью равенства
\ShowEq{morphisms category, h}

Пусть $\omega\in\Omega_2(p)$.
Так как отображения $R$ и $j$ являются гомоморфизмами $\Omega_2$\Hyph
алгебры, то
\ShowEq{morphisms category, h 1}
Из равенства
\EqRef{morphisms category, h 1}
следует, что отображение $h$ является гомоморфизмом $\Omega_2$\Hyph алгебры.

Так как отображение $R$ является приведенным морфизмом представления $f$
в представление $g$, то верно равенство
\ShowEq{morphism representations f g}
Из равенства
\EqRef{morphisms category, h}
следует
\ShowEq{morphism representations f1 g 1}
Из равенств
\EqRef{morphism representations f g},
\EqRef{morphism representations f1 g 1}
следует
\ShowEq{morphism representations f1 g 2}
Из равенств
\EqRef{morphisms category, h},
\EqRef{morphism representations f1 g 2}
следует
\ShowEq{morphism representations f1 g 3}
Из равенств
\EqRef{representation B/N 1},
\EqRef{morphism representations f1 g 3}
следует
\ShowEq{morphism representations f1 g 4}
Из равенства
\EqRef{morphism representations f1 g 4}
следует, что отображение $h$ является приведенным морфизмом
представления $f_1$ в представление $g$.
\end{proof}

\section{Тензорное произведение представлений}

\begin{definition}
\label{definition: tensor product of representations}
Пусть $A$ является абелевой мультипликативной $\Omega_1$\Hyph группой.
Пусть
\ShowEq{set of universal algebras 2}
- $\Omega_2$\Hyph алгебры.\,\footnote{Я определяю
тензорное произведение представлений универсальной алгебры
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.
}
Пусть для любого \Kn
\ShowEq{representation A B k 1}
эффективное представление мультипликативной $\Omega_1$\Hyph группы $A$
в $\Omega_2$\Hyph алгебре $B_k$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
приведенные полиморфизмы представлений $f_1$, ..., $f_n$
\ShowEq{polymorphisms category}
где $S_1$, $S_2$ - $\Omega_2$\Hyph алгебры и
\ShowEq{representation of algebra in S1 S2}
эффективные представления мультипликативной $\Omega_1$\Hyph группы $A$.
Мы определим морфизм $R_1\rightarrow R_2$
как приведенный морфизм представлений $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{polymorphisms category, diagram}
Универсальный объект
\ShowEq{tensor product of representations}
категории $\mathcal A$ называется
\AddIndex{тензорным произведением}{tensor product}
представлений $B_1$, ..., $B_n$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: tensor product is unique}
Если тензорное произведение эффективных представлений существует,
то тензорное произведение определено однозначно
с точностью до изоморфизма представлений.
\end{theorem}
\begin{proof}
Пусть $A$ является абелевой мультипликативной $\Omega_1$\Hyph группой.
Пусть
\ShowEq{set of universal algebras 2}
- $\Omega_2$\Hyph алгебры.
Пусть для любого \Kn
\ShowEq{representation A B k 1}
эффективное представление мультипликативной $\Omega_1$\Hyph группы $A$
в $\Omega_2$\Hyph алгебре $B_k$.
Пусть эффективные представления
\ShowEq{representation of algebra in S1 S2}
являются тензорным произведением
представлений $B_1$, ..., $B_n$.
Из коммутативности диаграммы
\ShowEq{polymorphisms category, diagram 1}
следует, что
\ShowEq{R1= R2=}
Из равенств
\EqRef{R1= R2=}
следует, что морфизмы представления
\ShowEq{h1*h2}
являются тождественными отображениями.
Следовательно, морфизмы представления $h_1$, $h_2$
являются изоморфизмами.
\end{proof}

\begin{convention}
\label{convention: isomorphic representations S1=S2}
Алгебры $S_1$, $S_2$ могут быть различными множествами.
Однако они неразличимы для нас, если мы рассматриваем их
как изоморфные представления.
В этом случае мы будем писать $S_1=S_2$.
\qed
\end{convention}

\begin{definition}
\label{definition: tensor power of representation}
Тензорное произведение
\ShowEq{tensor power of representation}
называется
\AddIndex{тензорной степенью}{tensor power} представления $B$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: tensor product of representations}
Если существует полиморфизм представлений,
то тензорное произведение представлений существует.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{f:A->M}
представление $\Omega_1$\Hyph алгебры $A$, порождённое
декартовым произведением $\Times$
множеств $B_1$, ..., $B_n$.\,\footnote{Согласно теоремам
\ref{theorem: product exists in category of Omega algebras},
\ref{theorem: product of effective representations},
множество, порождённое приведенным декартовым произведением
представлений $B_1$, ..., $B_n$
совпадает с декартовым произведением $\Times$
множеств $B_1$, ..., $B_n$.
В этом месте доказательства
нас не интересует алгебраическая структра на множестве $\Times$.
}
Инъекция
\ShowEq{map i, representation, tensor product, 1}
определена по правилу\,\footnote{Равенство
\EqRef{map i, representation, tensor product}
утверждает, что мы отождествляем базис представления $M$
с множеством $\Times$.
}
\ShowEq{map i, representation, tensor product}
Пусть $N$ - отношение эквивалентности, порождённое равенствами\,\footnote{
Я рассматриваю формирование элементов представления из элементов базиса
согласно теореме
\EqParm{ref theorem: structure of subrepresentations}{=.}
Теорема
\ref{theorem: representation, tensor product}
требует выполнения условий
\EqRef{equivalence 1, representation, tensor product},
\EqRef{equivalence 2, representation, tensor product}.
}
\ShowEq{equivalence, representation, tensor product}
\ShowEq{equivalence, 1, representation, tensor product}

\begin{lemma}
\label{lemma: endomorphism coordinated with equivalence 1}
{\it
Пусть $\omega\in\Omega_2(p)$. Тогда
\ShowEq{equivalence 1 5, representation, tensor product}
}
\end{lemma}

{\sc Доказательство.}
Из равенства
\EqRef{equivalence 2, representation, tensor product}
следует
\ShowEq{equivalence 1 1, representation, tensor product}
Так как $f_i(c)$ - эндоморфизм $\Omega_2$\Hyph алгебры $B_i$, то
из равенства
\EqRef{equivalence 1 1, representation, tensor product}
следует
\ShowEq{equivalence 1 2, representation, tensor product}
Из равенств
\EqRef{equivalence 1 2, representation, tensor product},
\EqRef{equivalence 1, representation, tensor product}
следует
\ShowEq{equivalence 1 3, representation, tensor product}
Из равенств
\EqRef{equivalence 1 3, representation, tensor product},
\EqRef{equivalence 2, representation, tensor product}
следует
\ShowEq{equivalence 1 4, representation, tensor product}
Так как $f(c)$ - эндоморфизм $\Omega_2$\Hyph алгебры $B$, то
равенство
\EqRef{equivalence 1 5, representation, tensor product}
следует из равенства
\EqRef{equivalence 1 4, representation, tensor product}.
\hfill\(\odot\)

\begin{lemma}
\label{lemma: endomorphism coordinated with equivalence 2}
\ShowEq{equivalence 2 1, representation, tensor product}
\end{lemma}

{\sc Доказательство.}
Из равенства
\EqRef{equivalence 2, representation, tensor product}
следует, что
\ShowEq{equivalence 2, 1, representation, tensor product}
Равенство
\EqRef{equivalence 2 1, representation, tensor product}
следует из равенства
\EqRef{equivalence 2, 1, representation, tensor product}.
\hfill\(\odot\)

\begin{lemma}
\label{lemma: endomorphism coordinated with equivalence}
Для любого $c\in A$ эндоморфизм $f(c)$ $\Omega_2$\Hyph алгебры $M$
согласовано с эквивалентностью $N$.
\end{lemma}

{\sc Доказательство.}
Утверждение леммы следует
из лемм
\ref{lemma: endomorphism coordinated with equivalence 1},
\ref{lemma: endomorphism coordinated with equivalence 2}
и определения
\ShowEq{ref transformation coordinated with equivalence}
\hfill\(\odot\)

Из леммы
\ref{lemma: endomorphism coordinated with equivalence}
и теоремы
\ShowEq{ref transformation correlated with equivalence}
следует, что на множестве ${}^*M/N$ определена $\Omega_1$\Hyph алгебра.
Рассмотрим диаграмму
\ShowEq{endomorphism coordinated with equivalence, diagram}
Согласно лемме
\ref{lemma: endomorphism coordinated with equivalence},
из условия
\ShowEq{endomorphism coordinated with equivalence, diagram 1}
следует
\ShowEq{endomorphism coordinated with equivalence, diagram 2}
Следовательно, преобразование $F(a)$ определено корректно и
\ShowEq{endomorphism coordinated with equivalence, diagram 3}
Если $\omega\in\Omega_1(p)$, то мы положим
\ShowEq{endomorphism coordinated with equivalence, diagram 4}
Следовательно, отображение $F$ является представлением
$\Omega_1$\Hyph алгебры $A$.
Из \EqRef{endomorphism coordinated with equivalence, diagram 3}
следует, что $j$ является приведенным морфизмом представлений $f$ и $F$.

Рассмотрим коммутативную диаграмму
\ShowEq{diagram top, representation, tensor product}
Из коммутативности диаграммы
\EqRef{diagram top, representation, tensor product}
и равенства
\EqRef{map i, representation, tensor product}
следует, что
\ShowEq{g1()=j()}
Из равенств
\EqRef{map i, representation, tensor product},
\EqRef{equivalence 1, representation, tensor product},
\EqRef{equivalence 2, representation, tensor product}
следует
\ShowEq{g_1 1, representation, tensor product}
\ShowEq{g_1 2, representation, tensor product}
Из равенств \EqRef{g_1 1, representation, tensor product}
и \EqRef{g_1 2, representation, tensor product}
следует, что отображение $g_1$
является приведенным полиморфизмом представлений $f_1$, ..., $f_n$.

Поскольку $\Times$ - базис представления $M$ $\Omega_1$\Hyph алгебры $A$,
то, согласно теореме
\ShowEq{ref automorphism uniquely defined by image of basis}
для любого представления
\ShowEq{representation A V}
и любого
приведенного полиморфизма
\ShowEq{diagram bottom, 1, representation, tensor product}
существует единственный морфизм представлений $k:M\rightarrow V$,
для которого коммутативна следующая диаграмма
\ShowEq{diagram bottom, representation, tensor product}
Так как $g_2$ - приведенный полиморфизм, то
\ShowEq{ker k supseteq N}

Согласно теореме
\ref{theorem: morphism representations and kernel equivalence}
отображение $j$ универсально в категории морфизмов
представления $f$,
ядро которых содержит $N$.
Следовательно, определён морфизм представлений
\[
h:M/N\rightarrow V
\]
для которого коммутативна диаграмма
\ShowEq{diagram right, representation, tensor product}
Объединяя диаграммы
\ShowEq{diagrams, representation, tensor product}
получим коммутативную диаграмму
\ShowEq{diagram, representation, tensor product}
Так как $\mathrm{Im}\,g_1$ порождает $M/N$,
то отображение $h$ однозначно определено.
\end{proof}

Согласно доказательству теоремы
\ref{theorem: tensor product of representations}
\ShowEq{B 1n M N}
Для $d_i\in A_i$ будем записывать
\ShowEq{map j, representation, tensor product}
Из равенств
\EqRef{g1()=j()},
\EqRef{map j, representation, tensor product}
следует, что
\ShowEq{g1()=otimes}

\begin{theorem}
\label{theorem: B times->B otimes}
Отображение
\ShowEq{B times->B otimes}
является полиморфизмом.
\end{theorem}
\begin{proof}
Теорема является следствием определений
\ref{definition: reduced polymorphism of representations},
\ref{definition: tensor product of representations}.
\end{proof}

\begin{theorem}
\label{theorem: tensor product and polymorphism}
Пусть $B_1$, ..., $B_n$ -
$\Omega_2$\Hyph алгебры.
Пусть
\ShowEq{map f, 1, representation, tensor product}
приведенный полиморфизм, определённый равенством
\ShowEq{map f, representation, tensor product}
Пусть
\ShowEq{map g, representation, tensor product}
приведенный полиморфизм в $\Omega_2$\Hyph алгебру $V$.
Существует морфизм представлений
\ShowEq{map h, representation, tensor product}
такой, что диаграмма
\ShowEq{map gh, representation, tensor product}
коммутативна.
\end{theorem}
\begin{proof}
Равенство
\EqRef{map f, representation, tensor product}
следует
из равенств
\EqRef{map i, representation, tensor product} и
\EqRef{map j, representation, tensor product}.
Существование отображения $h$ следует из определения
\ref{definition: tensor product of representations}
и построений, выполненных при доказательстве теоремы
\ref{theorem: tensor product of representations}.
\end{proof}

\begin{theorem}
\label{theorem: representation, tensor product}
Пусть
\ShowEq{equivalence, 1, representation, tensor product}
Тензорное произведение дистрибутивно относительно операции $\omega$
\ShowEq{tensors 1, representation, tensor product}
Представление мультипликативной $\Omega_1$\Hyph группы $A$
в тензорном произведении определено равенством
\ShowEq{tensors 2, representation, tensor product}
\end{theorem}
\begin{proof}
Равенство
\EqRef{tensors 1, representation, tensor product}
является следствием равенства\\
\EqRef{g_1 1, representation, tensor product}
и определения
\EqRef{g1()=otimes}.
Равенство
\EqRef{tensors 2, representation, tensor product}
является следствием равенства
\EqRef{g_1 2, representation, tensor product}
и определения
\EqRef{g1()=otimes}.
\end{proof}

\ePrints{1102.5168}
\ifx\Semafor\ValueOff
\section{Ассоциативность тензорного произведения}

Пусть $A$ является мультипликативной $\Omega_1$\Hyph группой.
Пусть
\ShowEq{B1,B2,B3}
- $\Omega_2$\Hyph алгебры.
Пусть для $k=1$, $2$, $3$
\ShowEq{representation A B k 1}
эффективное представление мультипликативной $\Omega_1$\Hyph группы $A$
в $\Omega_2$\Hyph алгебре $B_k$.

\begin{lemma}
\label{lemma: ox12x3->ox123 morphism of oxB12}
{\it
Для заданного значения
\ShowEq{x3 in B3}
отображение
\ShowEq{ox12x3->ox123}
определённое равенством
\ShowEq{ox12x3->ox123=}
является приведенным морфизмом представления
\ShowEq{oxB12}
в представление
\ShowEq{oxB13}.
}
\end{lemma}
\begin{proof}
Согласно теореме
\ref{theorem: B times->B otimes},
для заданного значения
\ShowEq{x3 in B3}
отображение
\ShowEq{x123->ox123}
является полиморфизмом по переменным
\ShowEq{x in B 12}
Следовательно,
для заданного значения
\ShowEq{x3 in B3}
лемма является следствием теоремы
\ref{theorem: tensor product and polymorphism}.
\end{proof}

\begin{lemma}
\label{lemma: ox12x3->ox123 morphism of B3}
{\it
Для заданного значения
\ShowEq{x12 in B12}
отображение
$h_{12}$
является приведенным морфизмом представления
$B_3$
в представление
\ShowEq{oxB13}.
}
\end{lemma}
\begin{proof}
Согласно теореме
\ref{theorem: B times->B otimes}
и равенству
\EqRef{g1()=otimes},
для заданного значения
\ShowEq{x in B 12,}
отображение
\ShowEq{x ox12 3->ox123}
является морфизмом по переменной
\ShowEq{x in B 3}
Следовательно,
теорема является следсвием теорем
\ref{theorem: reduced polymorphism of representation, ak},
\ref{theorem: existence of reduced polymorphism, a omega b omega}.
\end{proof}

\begin{lemma}
\label{lemma: h:ox(12)3->ox123}
{\it
Существует приведенный морфизм представлений
\ShowEq{h:ox(12)3->ox123}
}
\end{lemma}
\begin{proof}
Согласно леммам
\ref{lemma: ox12x3->ox123 morphism of oxB12},
\ref{lemma: ox12x3->ox123 morphism of B3}
и определению
\ref{definition: reduced polymorphism of representations},
отображение $h_{12}$ является приведенным полиморфизмом представлений.
Утверждение леммы является следствием теоремы
\ref{theorem: tensor product and polymorphism}.
\end{proof}

\begin{lemma}
\label{lemma: g:ox123->ox(12)3}
{\it
Существует приведенный морфизм представлений
\ShowEq{g:ox123->ox(12)3}
}
\end{lemma}
\begin{proof}
Отображение
\ShowEq{x123->ox(12)3}
является полиморфизмом по переменным
\ShowEq{x in B 13}
Следовательно,
лемма является следствием теоремы
\ref{theorem: tensor product and polymorphism}.
\end{proof}

\begin{theorem}
\label{theorem: tensor product is associative}
\ShowEq{B1xB2xB3}
\end{theorem}
\begin{proof}
Согласно лемме
\ref{lemma: h:ox(12)3->ox123},
существует приведенный морфизм представлений
\ShowEq{h:ox(12)3->ox123}
Согласно лемме
\ref{lemma: g:ox123->ox(12)3},
существует приведенный морфизм представлений
\ShowEq{g:ox123->ox(12)3}
Следовательно, приведенные морфизмы представлений $h$, $g$
являются изоморфизмами, откуда следует равенство
\ShowEq{B1xB2xB3=(B1xB2)xB3}
Аналогично мы можем доказать равенство
\ShowEq{B1xB2xB3=B1x(B2xB3)}
\end{proof}

\begin{remark}
Очевидно, что структура $\Omega_2$\Hyph алгебр
\ShowEq{x(12)3 123}
слегка различна.
Мы записываем равенство
\EqRef{B1xB2xB3=(B1xB2)xB3},
опираясь на соглашение
\ref{convention: isomorphic representations S1=S2}
и это позволяет нам говорить об ассоциативности тензорного произведения представлений.
\qed
\end{remark}
\fi




==> Preface.1502.04063.English.tex <==
%auto-ignore
%\input{Preface.\BookNumber.Eq}

\chapter{Preface}

\section{Preface to Version 1}

There exist few equivalent definitions of module.
For me, the definition of module
as effective representation of commutative ring
in Abelian group is the most interesting definition.
This definition allows us to consider linear algebra
from more general point of view and to understand which construction
can be properly defined in other algebraic theories.
For instance, we may consider a linear map
as morphism of representation, i.e. a map
which preserves the structure of the representation.

The module in which the product is defined is called algebra.
Depending on the problem to be solved, we consider
different algebraic structures on algebra.
Accordingly, the map, which preserves the structure of algebra, changes.

If we do not consider the representation of ring $D$
in $D$\Hyph algebra $A$,
then the algebra $A$ is a ring. A map, preserving
the structure of algebra as a ring, is called homomorphism of
algebra.
If we do not consider the product $D$\Hyph algebra $A$,
then we consider $D$\Hyph algebra as module.
A map, preserving the
structure of algebra as module, is called a linear map of
the $D$\Hyph algebra.
Linear map is important tool
to study calculus.
A map, preserving the
structure of representation, is called a linear homomorphism.
In the section
\ref{section: Linear Automorphism of Quaternion Algebra},
I proved the existence of a nontrivial linear homomorphism.

%Какие определения и конструкции линейной алгебры
%сохраняются в общем случае?
%Какие конструции характерны для линейной алгебры?

%Текст книги разделён на две части.
%Сперва я рассматриваю декартово произведение представлений,
%полиморфизмы представлений и тензорное произведение
%эффективных представлений.

\begin{flushright}
February, 2015
\end{flushright}

\section{Preface to Version 2}

The main idea of this book is an attempt to apply
to the representation of $\Omega_1$\Hyph algebra
(which is called $\Omega_1$\Hyph algebra of transformations
of $\Omega_2$\Hyph algebra or just $\Omega_1$\Hyph algebra of transformations)
some of concepts with which we are familiar in linear algebra.
Since linear map is reduced morphism of module
when we consider module as representation of ring
in Abelian group,
then the definition of polymorphism of representations
is natural generalization of polylinear map.

Studying the linear map over non commutative
division ring $D$,
we conclude that in the equation
\[f(ax)=af(x)\]
$a$ cannot be any element of the ring $D$,
but should belong to the center of the ring $D$.
This statement makes theory of linear maps interesting and rich theory.

So, like in case of polylinear map, we request
that transformation which $\Omega_1$\Hyph algebra
generates in one factor, can be transferred
to any other factor.
In general, this requirement is not restrictive;
but compliance with this requirement allows consideration of
$\Omega_1$\Hyph algebra of transformations as Abelian multiplicative $\Omega_1$\Hyph group.

Tensor product of vector spaces is associative.
Consideration of associativity of tensor product of representation
generates new constraint on polymorphism of representations.
Any two operations of $\Omega_2$\Hyph algebra must satisfy the equation
\EqRef{a omega b omega =}.
It is possible that Abelian group is only $\Omega_2$\Hyph algebra,
such that representation in this algebra admits polymorphism of representations.
However, today, this statement has not been proved.

If we believe in a statement which we cannot prove
or disprove, then discovery of opposite statement
may lead us to interesting discoveries.
For thousands of years mathematicians tried to prove Euclid's fifth postulate.
Lobachevsky and Bolyai proved that there exists geometry
which does not hold this postulate.
Mathematicians tried to find solution of algebraic equation using radicals.
However Galois proved this is imposible to do when the power of equation is greater than $4$.

For long time, I believed that existence of reduced morphism of representation
imply existence of reduced polymorphism of representation.
The theorem
\ref{theorem: no reduced polymorphism in ring}
was a surprise to me.

I believe that text about polymorphism and tensor product of representations is important.

\begin{itemize}
\item
After writing of few papers dedicated to calculus over Banach algebra,
I believed that one day I will be able to write
similar paper about calculus
in a representation.
I was confused by the need to refuse addition as estimate how small is distance
between maps. Of course, I may state that morphism of representation
is in neighborhood of a considered map.
However addition is an essential component of the construction.
Absence of reduced polymorphism deprive me of the opportunity
to define derivatives of second order.
\item
We can consider linear and polylinear maps of effective representation
in Abelian $\Omega_2$\Hyph group
like we consider linear and polylinear maps of $D$\Hyph algebra.
The structure of linear map of effective representation
in Abelian $\Omega_2$\Hyph group is more complicated than the structure of linear map
of $D$\Hyph algebra. However this problem is interesting for me and I hope
to return to this problem in the future.
\end{itemize}

\begin{flushright}
May, 2015
\end{flushright}


==> Preface.1502.04063.Russian.tex <==
%auto-ignore
%\input{Preface.\BookNumber.Eq}

\chapter{Предисловие}

\section{Предисловие к изданию 1}

Существует несколько эквивалентных определений модуля.
Для меня наиболее интересно определение модуля
как эффективное представление коммутативного кольца
в абелевой группе.
Это позволяет рассмотреть конструкции линейной алгебры
с более общей точки зрения и понять какие конструкции
верны в других алгебраических теориях.
Например, мы можем рассматривать линейное отображение
как морфизм представления, т. е. отображение,
которое сохраняет структуру представления.

Модуль, в котором определено произведение, называется алгеброй.
В зависимости от решаемой задачи, мы можем рассматривать
различные алгебраические структуры на алгебре.
Соответственно меняются отображения, сохраняющие структуру алгебры.

Если нас не интересует представление кольца $D$
в $D$\Hyph алгебре $A$,
то алгебра $A$ является кольцом. Отображение, сохраняющее
структуру алгебры как кольца, называется гомоморфизмом
алгебры.
Если нас не интересует произведение в $D$\Hyph алгебре $A$,
то мы рассматриваем $D$\Hyph алгебру как модуль.
Отображение, сохраняющее
структуру алгебры как модуля, называется линейным отображением
$D$\Hyph алгебры.
Линейные отображения являются важным инструментом
при изучении математического анализа.
Отображение, сохраняющее
структуру представления, называется линейным гомоморфизмом.
В разделе
\ref{section: Linear Automorphism of Quaternion Algebra}
я показал существование нетривиального линейного гомоморфизма.

%Какие определения и конструкции линейной алгебры
%сохраняются в общем случае?
%Какие конструции характерны для линейной алгебры?

%Текст книги разделён на две части.
%Сперва я рассматриваю декартово произведение представлений,
%полиморфизмы представлений и тензорное произведение
%эффективных представлений.

\begin{flushright}
Февраль, 2015
\end{flushright}

\section{Предисловие к изданию 2}

Основной замысел этой книги - попытка перенести
в представление $\Omega_1$\Hyph алгебры
(которую мы будем называть $\Omega_1$\Hyph алгеброй преобразований
$\Omega_2$\Hyph алгебры или просто $\Omega_1$\Hyph алгеброй преобразований)
некоторые понятия, с которыми мы хорошо знакомы в линейной алгебре.
Поскольку линейное отображение - это приведенный морфизм модуля,
если мы рассматриваем модуль как представление кольца
в абелевой группе,
то определение полиморфизма представлений
является естественным обобщением полилинейного отображения.

Изучая линейное отображение над некоммутативным
кольцом с делением $D$,
мы приходим к выводу что в равенстве
\[f(ax)=af(x)\]
$a$ не может быть произвольным элементом кольца $D$,
но должно принадлежать центру кольца $D$.
Это позволяет сделать теорию линейных отображений интересной и богатой.

Поэтому, также как в случае полилинейного отображения, мы требуем,
чтобы преобразование, которое $\Omega_1$\Hyph алгебра
порождает в одном сомножителе, можно было бы перенести
на любой другой сомножитель.
Вообще говоря, это требование не представляется жёстким,
но выполнение этого требования позволяет рассматривать
$\Omega_1$\Hyph алгебру преобразований как абелевую мультипликативную $\Omega_1$\Hyph группу.

Тензорное произведение векторных пространств ассоциативно.
Рассмотрение ассоциативности тензорного произведения представлений
порождает новое ограничение на полиморфизм представлений.
Любые две операции $\Omega_2$\Hyph алгебры должны удовлетворять равенству
\EqRef{a omega b omega =}.
Возможно, что абелевая группа является единственной $\Omega_2$\Hyph алгеброй,
представление в которой допускает полиморфизм представлений.
Однако сегодня это утверждение не доказано.

Если мы верим в некоторое утверждение, которое мы не можем доказать
или опровергнуть, то открытие противоположного утверждения
может привести к интересным открытиям.
На протяжении тысячелетий математики пытались доказать пятый постулат Евклида.
Лобачевский и Больяй доказали, что существует геометрия,
где этот постулат неверен.
Математики пытались найти решение алгебраического уравнения, используя радикалы.
Однако Галуа доказал, что это невозможно сделать, если степень уравнения выше $4$.

Я долгое время полагал, что из существования приведенного морфизма представления
следует существование приведенного полиморфизма представления.
Теорема
\ref{theorem: no reduced polymorphism in ring}
оказалась для меня полной неожиданностью.

Я полагаю, что текст о полиморфизме и тензорном произведении представлений важен.

\begin{itemize}
\item
Написав серию статей, посвящённых математическому анализу над банаховыми алгебрами,
я полагал, что однажды я смогу написать
подобную статью о математическом анализе
в произвольном представлении.
Меня смущала необходимость отказаться от сложения как оценки как мало расстояние
между отображениями. Конечно, я могу утверждать, что морфизм представления
находится в окрестности рассматриваемого отображения.
Однако сложение является существенной компонентой построения.
Отсутствие приведенного полиморфизма лишает меня возможности
определить производные второго порядка.
\item
Аналогично тому, как мы рассматриваем линейное отображение $D$\Hyph алгебры,
мы можем рассматривать линейное отображение эффективного представления
в абелевой $\Omega_2$\Hyph группе.
Структура линейного отображения эффективного представления
в абелевой $\Omega_2$\Hyph группе сложнее чем структура линейного отображения
$D$\Hyph алгебры. Однако это задача интересна для меня, и я надеюсь
вернуться к ней в будущем.
\end{itemize}

\begin{flushright}
Май, 2015
\end{flushright}


==> Representation.Product.Russian.tex <==
%auto-ignore

\input{Representation.Product.Eq}

\chapter{Произведение представлений}

\section{Декартово произведение универсальных алгебр}

\begin{definition}
\label{definition: product of objects in category}
Пусть $\mathcal A$ - категория.
Пусть $\{B_i,\Ii\}$ - множество объектов из $\mathcal A$.
Объект
\ShowEq{product of objects in category}
и множество морфизмов
\[
\{\xymatrix{f_i:P\ar[r]&B_i},\Ii\}
\]
называется
\AddIndex{произведением объектов $\{B_i,\Ii\}$ в категории $\mathcal A$}
{product of objects in category}\,\footnote{Определение
дано согласно \citeBib{Serge Lang},
страница 45.}, если для любого объекта $R$ и множество морфизмов
\[
\{\xymatrix{g_i:R\ar[r]&B_i},\Ii\}
\]
существует единственный морфизм
\[
\xymatrix{h:R\ar[r]&P}
\]
такой, что диаграмма
\ShowEq{product of objects in category diagram}
коммутативна для всех $\Ii$.

Если $|I|=n$, то для произведения объектов
$\{B_i,\Ii\}$ в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{product of objects in category, 1 n}
\qed
\end{definition}

\begin{example}
Пусть \(\mathcal S\) - категория множеств.\,\footnote{Смотри
также пример в
\citeBib{Serge Lang},
страница 45.
}
Согласно определению
\ref{definition: product of objects in category},
декартово произведение
\ShowEq{Cartesian product of sets}
семейства множеств
\ShowEq{Ai iI}
и семейство проекций на \(i\)\Hyph й множитель
\ShowEq{projection on i factor}
являются произведением в категории \(\mathcal S\).
\qed
\end{example}

\begin{theorem}
\label{theorem: product exists in category of Omega algebras}
Произведение существует в категории \(\mathcal A\) \(\Omega\)\Hyph алгебр.
Пусть \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\).
%семейства \(\Omega\)\Hyph алгебр
Тогда
\StartLabelItem
\begin{enumerate}
\item
Множество \(A\) является декартовым произведением
семейства множеств
\ShowEq{Ai iI}
\item
Гомоморфизм \(\Omega\)\Hyph алгебры
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
\item
Любое \(A\)\Hyph число $a$ может быть однозначно представлено
в виде кортежа
\ShowEq{tuple represent A number}
\(A_i\)\Hyph чисел.
\LabelItem{tuple represent A number}
\item
Пусть
\ShowEq{omega in Omega}
- n\Hyph арная операция.
Тогда операция $\omega$ определена покомпонентно
\ShowEq{operation is defined componentwise}
где
\ShowEq{a=ai 1n}.
\LabelItem{operation is defined componentwise}
\end{enumerate}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{Cartesian product of sets}
декартово произведение
семейства множеств
\ShowEq{Ai iI}
и, для каждого \iI, отображение 
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
Рассмотрим диаграмму морфизмов в категории множеств $\mathcal S$
\ShowEq{operation is defined componentwise, diagram}
где отображение $g_i$ определено равенством
\ShowEq{gi()=}
Согласно определению
\ref{definition: product of objects in category},
отображение $\omega$ определено однозначно из множества диаграмм
\EqRef{operation is defined componentwise, diagram}
\ShowEq{omega(ai)=(omega ai)}
Равенство
\EqRef{operation is defined componentwise}
является следствием равенства
\EqRef{omega(ai)=(omega ai)}.
\ifx\texFuture\Defined

\begin{lemma}
\label{lemma: tuple represent A number}
{\it
Пусть \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{projection on i factor}
является произведением в категории \(\mathcal A\).
Любое \(A\)\Hyph число $a$ может быть однозначно представлено
в виде кортежа
\ShowEq{tuple represent A number}
\(A_i\)\Hyph чисел.
}
\end{lemma}

{\sc Доказательство.}
Пусть
\ShowEq{a ne b}
- такие \(A\)\Hyph числа, что для любого \iI
\ShowEq{p(a)=p(b)}
Если предположить, что неравные \(A\)\Hyph числа
имеют равные разложения в виде кортежа,
то мы можем определить отношение эквивалентности,
фактор по которому скорее кандидат на произведение.
\hfill\(\odot\)

Из равенства
\ShowEq{pj(a)=aj}
следует, что отображение \(p_j\) является проекцией.
\fi
\end{proof}

\begin{definition}
Если \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\),
то \(\Omega\)\Hyph алгебра \(A\) называется
\AddIndex{прямым}{direct product of Omega algebras}
или
\AddIndex{декартовым произведением \(\Omega\)\Hyph алгебр}
{Cartesian product of Omega algebras}
\ShowEq{Ai iI}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: map from product into product}
Пусть множество \(A\) является
декартовым произведением множеств
\ShowEq{Ai iI}
и множество \(B\) является
декартовым произведением множеств
\ShowEq{Bi iI}.
Для каждого \iI, пусть
\ShowEq{f:A->B i}
является отображением множества $A_i$ в множество $B_i$.
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras diagram}
где отображения
\ShowEq{pi p'i}
являются проекцией на \(i\)\Hyph й множитель.
Множество коммутативных диаграмм
\EqRef{homomorphism of Cartesian product of Omega algebras diagram}
однозначно определяет отображение
\EqParm{f:A->B}{f=f,A=12}
\DrawEq{f:A->B=}{}
\end{theorem}
\begin{proof}
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras}
Пусть \(a\in A\).
Согласно утверждению
\RefItem{tuple represent A number},
\(A\)\Hyph число \(a\)
может быть представлено в виде кортежа \(A_i\)\Hyph чисел
\ShowEq{a=p(a)i}
Пусть
\ShowEq{b=f(a)}
Согласно утверждению
\RefItem{tuple represent A number},
\(B\)\Hyph число \(b\)
может быть представлено в виде кортежа \(B_i\)\Hyph чисел
\ShowEq{b=p(b)i}
Из коммутативности диаграммы $(1)$
и из равенств
\EqRef{b=f(a)},
\EqRef{b=p(b)i}
следует, что
\ShowEq{b=g(a)i}
Из коммутативности диаграммы $(2)$
и из равенства
\EqRef{a=p(a)i}
следует, что
\ShowEq{b=f(a)i}
\end{proof}

\begin{theorem}
\label{theorem: homomorphism of Cartesian product of Omega algebras}
Пусть \(\Omega\)\Hyph алгебра \(A\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Ai iI}
и \(\Omega\)\Hyph алгебра \(B\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Bi iI}.
Для каждого \iI,
пусть отображение
\ShowEq{f:A->B i}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
Тогда отображение
\EqParm{f:A->B}{f=f,A=12}
определённое равенством
\DrawEq{f:A->B=}{homomorphism}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{omega in Omega}
- n\Hyph арная операция.
Пусть
\ShowEq{a=ai 1n} и
\ShowEq{b=bi 1n}.
Из равенств
\EqRef{operation is defined componentwise},
\eqRef{f:A->B=}{homomorphism}
следует, что
\ShowEq{f:A->B omega}
\end{proof}

\section{Декартово произведение представлений}

\begin{lemma}
\label{lemma: product of *algebras is *algebra}
Пусть
\ShowEq{Cartesian product of sets}
декартово произведение семейства \(\Omega_1\)\Hyph алгебр
\ShowEq{Ai iI}.
Для каждого \iI, пусть множество ${}^*A_i$
является \(\Omega_2\)\Hyph алгеброй.
Тогда множество
\ShowEq{f in *A =}
является декартовым произведением \(\Omega_2\)\Hyph алгебр ${}^*A_i$.
\end{lemma}
\begin{proof}
Согласно определению
\EqRef{f in *A =},
мы можем представить отображение
\ShowEq{f in *A}
в виде кортежа
\ShowEq{f=(fi)}
отображений
\ShowEq{fi in *Ai}
Согласно определению
\EqRef{f in *A =},
\ShowEq{(fi)(ai)=}
Пусть
\ShowEq{omega in 2}
- n\Hyph арная операция.
Мы определим операцию $\omega$
на множестве
\ShowEq{circ A}
равенством
\ShowEq{circ A omega}
\end{proof}

\begin{definition}
%\label{definition: category of representations of F algebra from category}
Пусть $\mathcal A_1$ - категория $\Omega_1$\Hyph алгебр.
Пусть $\mathcal A_2$ - категория $\Omega_2$\Hyph алгебр.
Мы определим \AddIndex{категорию
\ShowEq{(mA1*)mA2 symb}
$\ $ левосторонних представлений}
{category of left-side representations}.
Объектами этой категории являются левосторонние представления
$\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре.
Морфизмами этой категории являются морфизмы соответствующих представлений.
\qed
\end{definition}

\begin{theorem}
\label{theorem: product of single transitive representations}
В категории
\ShowEq{(mA1*)mA2}
существует произведение
однотранзитивных левосторонних представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре.
\end{theorem}
\begin{proof}
Для
\ShowEq{j=12}
пусть
\EqParm{P=xBi}{P=P}
произведение семейства $\Omega_j$\Hyph алгебр
\EqParm{Bi}{P=P}
и для любого $\Ii$ отображение
\EqParm{ti:P->Bi}{P=P}
является проекцией на множитель $i$.
Для каждого $\Ii$, пусть
\EqParm{F:P->*P}{P=B}
однотранзитивное \Ts{B_{1i}}представление в \(\Omega_2\)\Hyph алгебре $B_{2i}$.

Пусть
\(b_1\in P_1\).
Согласно утверждению
\RefItem{tuple represent A number},
\(P_1\)\Hyph число \(b_1\)
может быть представлено в виде кортежа \(B_{1i}\)\Hyph чисел
\ShowEq{b=t(b)1i}
Пусть
\(b_2\in P_2\).
Согласно утверждению
\RefItem{tuple represent A number},
\(P_2\)\Hyph число \(b_2\)
может быть представлено в виде кортежа \(B_{2i}\)\Hyph чисел
\ShowEq{b=t(b)2i}

\begin{lemma}
Для каждого $\Ii$, рассмотрим диаграмму отображений
\ShowEq{define product of single transitive representations}
Пусть отображение
\EqParm{g:P1->*P2}{P=P}
определено равенством
\ShowEq{g(b1)(b2)=}
Тогда отображение \(g\) является
однотранзитивным \Ts{P_1}представлением в \(\Omega_2\)\Hyph алгебре $P_2$
\EqParm{F:P->*P}{P=P}
Отображение
\ShowEq{ti12}
является морфизмом представления \(g\) в представление \(h_i\).
\end{lemma}

{\sc Доказательство.}
\StartLabelItem
\begin{enumerate}
\item
Согласно определениям
\ShowEq{ref transformation of universal algebra}
отображение $h_i(b_{1i})$ является гомоморфизмом
\(\Omega_2\)\Hyph алгебры $B_{2i}$.
Согласно теореме
\ref{theorem: homomorphism of Cartesian product of Omega algebras},
из коммутативности диаграммы $(1)$ для каждого \iI,
следует, что отображение
\EqParm{g(b):P->P}{P=P}
определённое равенством
\EqRef{g(b1)(b2)=}
является гомоморфизмом
\(\Omega_2\)\Hyph алгебры $P_2$.
\LabelItem{g(b) is homomorphism of Omega2 algebra P2}
\item
Согласно определению
\ShowEq{ref representation of algebra}
множество
\EqParm{*B2i}{P=P}
является $\Omega_1$\Hyph алгеброй.
Согласно лемме
\ref{lemma: product of *algebras is *algebra},
множество
\EqParm{*P2}{P=P}
является $\Omega_1$\Hyph алгеброй.
\item
Согласно определению
\ShowEq{ref representation of algebra}
отображение
\ShowEq{h:B1->*B2 i}
является гомоморфизмом
\(\Omega_1\)\Hyph алгебры.
Согласно теореме
\ref{theorem: homomorphism of Cartesian product of Omega algebras},
отображение
\EqParm{g:P1->*P2}{P=P}
определённое равенством
\ShowEq{g(b1)=}
является гомоморфизмом
\(\Omega_1\)\Hyph алгебры.
\LabelItem{g is homomorphism of Omega1 algebra P1->*P2}
\end{enumerate}

Согласно утверждениям
\RefItem{g(b) is homomorphism of Omega2 algebra P2},
\RefItem{g is homomorphism of Omega1 algebra P1->*P2}
и определению
\ShowEq{ref representation of algebra}
отображение $g$ является \Ts{P_1}представлением
в $\Omega_2$\Hyph алгебре $P_2$.

Пусть
\EqParm{b2 12 in P2}{P=P}
Согласно утверждению
\RefItem{tuple represent A number},
\(P_2\)\Hyph числа
\ShowEq{b2 12}
могут быть представлены в виде кортежей \(B_{2i}\)\Hyph чисел
\ShowEq{b=t(b)2i 12}
Согласно теореме
\ShowEq{ref Representation is single transitive iff}
поскольку представление $h_i$ однотранзитивно,
то существует единственное \(B_{1i}\)\Hyph число $b_{1i}$ такое, что
\ShowEq{b22=h(b1)b21}
Согласно определениям
\EqRef{b=t(b)1i},
\EqRef{g(b1)(b2)=},
\EqRef{b=t(b)2i 12},
существует единственное \(P_1\)\Hyph число $b_1$ такое, что
\ShowEq{b22=g(b1)b21}
Согласно теореме
\ShowEq{ref Representation is single transitive iff}
представление $g$ однотранзитивно.

Из коммутативности диаграммы $(1)$ и определения
\ShowEq{ref morphism of representations of universal algebra}
следует, что отображение
\ShowEq{ti12}
является морфизмом представления \(g\) в представление \(h_i\).
\hfill\(\odot\)

Пусть
\DrawEq{d=g(b)(b)}{regular}
Из равенств
\EqRef{g(b1)(b2)=},
\eqRef{d=g(b)(b)}{regular}
следует, что
\ShowEq{d=h(b)(b)}

Для
\ShowEq{j=12}
пусть $R_j$ - другой объект категории $\mathcal A_j$. Для любого $\Ii$, пусть отображение
\EqParm{ti:P->Bi}{P=R1}
является морфизмом из $\Omega_1$\Hyph алгебра $R_1$ в
$\Omega_1$\Hyph алгебру $B_{1i}$.
Согласно определению
\ref{definition: product of objects in category},
существует единственный морфизм $\Omega_1$\Hyph алгебры
\ShowEq{s:R->P,1}
такой, что коммутативна диаграмма
\ShowEq{t*s=r1}
Пусть
\ShowEq{a in R1}
Пусть
\ShowEq{b=s(a)1}
Из коммутативности диаграммы
\EqRef{t*s=r1}
и утверждений
\EqRef{b=s(a)1},
\EqRef{b=t(b)1i}
следует, что
\ShowEq{b=r(a)1i}

Пусть
\EqParm{F:P->*P}{P=R}
однотранзитивное \Ts{R_1}представление в \(\Omega_2\)\Hyph алгебре $R_2$.
Согласно теореме
\ShowEq{ref unique morphism of representations of universal algebra}
морфизм $\Omega_2$\Hyph алгебры
\EqParm{ti:P->Bi}{P=R2}
такой, что отображение
\ShowEq{(r12)}
является морфизмом
представлений из $f$ в $h_i$,
определён однозначно
с точностью до выбора образа $R_2$\Hyph числа $a_2$.
Согласно замечанию
\ShowEq{ref remark morphism of representations of universal algebra}
в диаграмме отображений
\ShowEq{r12 product of single transitive representations}
диаграмма $(2)$ коммутативна. 
Согласно определению
\ref{definition: product of objects in category},
существует единственный морфизм $\Omega_2$\Hyph алгебры
\ShowEq{s:R->P,2}
такой, что коммутативна диаграмма
\ShowEq{t*s=r2}
Пусть
\ShowEq{a in R2}
Пусть
\ShowEq{b=s(a)2}
Из коммутативности диаграммы
\EqRef{t*s=r2}
и утверждений
\EqRef{b=s(a)2},
\EqRef{b=t(b)2i}
следует, что
\ShowEq{b=r(a)2i}
Пусть
\DrawEq{c=f(a)a}{regular}
Из коммутативности диаграммы $(2)$ и равенств
\EqRef{d=h(b)(b)},
\EqRef{b=r(a)2i},
\eqRef{c=f(a)a}{regular}
следует, что
\ShowEq{d=r(c)2i}
Из равенств
\EqRef{d=h(b)(b)},
\EqRef{d=r(c)2i}
следует, что
\ShowEq{d=s(c)2}
что согласуется с коммутативносью диаграммы
\EqRef{t*s=r2}.

Для каждого $\Ii$, мы объединим диаграммы отображений
\EqRef{define product of single transitive representations},
\EqRef{t*s=r1},
\EqRef{t*s=r2},
\EqRef{r12 product of single transitive representations}
\ShowEq{product of single transitive representations}
Из равенств
\eqRef{d=g(b)(b)}{regular}
\EqRef{b=s(a)2}
и из равенств
\eqRef{c=f(a)a}{regular},
\EqRef{d=s(c)2},
следует коммутативность диаграммы $(3)$.
Следовательно, отображение
\ShowEq{(s12)}
является морфизмом
представлений из $f$ в $g$.,
Согласно теореме
\ShowEq{ref unique morphism of representations of universal algebra}
морфизм
\ShowEq{(s12)}
определён однозначно,
так как мы требуем
\EqRef{d=s(c)2}.

Согласно определению
\ref{definition: product of objects in category},
представление $g$
и семейство морфизмов представления
\ShowEq{ti12, family}
является произведением в категории
\ShowEq{(mA1*)mA2}.
\end{proof}

\section{Приведенное декартово произведение представлений}

\begin{definition}
%\label{definition: category of representations of F algebra from category}
Пусть $A_1$ - $\Omega_1$\Hyph алгебра.
Пусть $\mathcal A_2$ - категория $\Omega_2$\Hyph алгебр.
Мы определим \AddIndex{категорию
\ShowEq{(A1*)mA2 symb}
$\ $ левосторонних представлений}
{category of left-side representations}.
Объектами этой категории являются левосторонние представления
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре.
Морфизмами этой категории являются приведенные морфизмы соответствующих представлений.
\qed
\end{definition}

\begin{theorem}
\label{theorem: product of effective representations}
В категории
\ShowEq{(A1*)mA2}
существует произведение
эффективных левосторонних представлений $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре
и это произведение является
эффективным левосторонним представлением $\Omega_1$\Hyph алгебры $A_1$.
\end{theorem}
\begin{proof}
Пусть
\EqParm{P=xBi}{P=A}
произведение семейства $\Omega_2$\Hyph алгебр
\EqParm{Bi}{P=A}
и для любого $\Ii$ отображение
\EqParm{ti:P->Bi}{P=A}
является проекцией на множитель $i$.
Для каждого $\Ii$, пусть
\EqParm{F:A->*P}{P=A}
эффективное \Ts{A_1}представление в \(\Omega_2\)\Hyph алгебре $A_{2i}$.

Пусть
\(b_1\in A_1\).
Пусть
\(b_2\in A_2\).
Согласно утверждению
\RefItem{tuple represent A number},
\(A_2\)\Hyph число \(b_2\)
может быть представлено в виде кортежа \(A_{2i}\)\Hyph чисел
\ShowEq{b=t(b)i}

\begin{lemma}
Для каждого $\Ii$, рассмотрим диаграмму отображений
\ShowEq{define product of single transitive representations, reduced}
Пусть отображение
\EqParm{g:P1->*P2}{P=A}
определено равенством
\ShowEq{g(b1)(b2)=, reduced}
Тогда отображение \(g\) является
эффективным \Ts{A_1}представлением в \(\Omega_2\)\Hyph алгебре $A_2$
\EqParm{F:P->*P}{P=A}
Отображение
\(t_i\)
является приведенным морфизмом представления \(g\) в представление \(h_i\).
\end{lemma}

{\sc Доказательство.}
\StartLabelItem
\begin{enumerate}
\item
Согласно определениям
\ShowEq{ref transformation of universal algebra}
отображение $h_i(b_1)$ является гомоморфизмом
\(\Omega_2\)\Hyph алгебры $A_{2i}$.
Согласно теореме
\ref{theorem: homomorphism of Cartesian product of Omega algebras},
из коммутативности диаграммы $(1)$ для каждого \iI,
следует, что отображение
\EqParm{g(b):P->P}{P=A}
определённое равенством
\EqRef{g(b1)(b2)=, reduced}
является гомоморфизмом
\(\Omega_2\)\Hyph алгебры $A_2$.
\LabelItem{g(b) is homomorphism of Omega2 algebra A2}
\item
Согласно определению
\ShowEq{ref representation of algebra}
множество
\EqParm{*B2i}{P=A}
является $\Omega_1$\Hyph алгеброй.
Согласно лемме
\ref{lemma: product of *algebras is *algebra},
множество
\EqParm{*P2}{P=A}
является $\Omega_1$\Hyph алгеброй.
\item
Согласно определению
\ShowEq{ref representation of algebra}
отображение
\ShowEq{h:A1->*A2i}
является гомоморфизмом
\(\Omega_1\)\Hyph алгебры.
Согласно теореме
\ref{theorem: homomorphism of Cartesian product of Omega algebras},
отображение
\EqParm{g:P1->*P2}{P=A}
определённое равенством
\ShowEq{g(b1)=,}
является гомоморфизмом
\(\Omega_1\)\Hyph алгебры.
\LabelItem{g is homomorphism of Omega1 algebra A1->*A2}
\end{enumerate}

Согласно утверждениям
\RefItem{g(b) is homomorphism of Omega2 algebra A2},
\RefItem{g is homomorphism of Omega1 algebra A1->*A2}
и определению
\ShowEq{ref representation of algebra}
отображение $g$ является \Ts{A_1}представлением
в $\Omega_2$\Hyph алгебре $A_2$.

Для любого $\Ii$,
согласно определению
\ShowEq{ref effective representation of algebra}
$A_1$\Hyph число $a_1$ порождает единственное преобразование
\ShowEq{b22=a1*b21 i}
Пусть
\EqParm{b2 12 in P2}{P=A}
Согласно утверждению
\RefItem{tuple represent A number},
\(A_2\)\Hyph числа
\ShowEq{b2 12}
могут быть представлены в виде кортежей \(A_{2i}\)\Hyph чисел
\ShowEq{b=t(b)i 12}
Согласно определению
\EqRef{g(b1)(b2)=, reduced}
представления $g$,
из равенств
\EqRef{b22=a1*b21 i},
\EqRef{b=t(b)i 12}
следует, что
$A_1$\Hyph число $a_1$ порождает единственное преобразование
\ShowEq{b22=a1*b21}
Согласно определению
\ShowEq{ref effective representation of algebra}
представление $g$ эффективно.

Из коммутативности диаграммы $(1)$ и определения
\ShowEq{ref morphism of representations of universal algebra}
следует, что отображение
$t_i$
является приведенным морфизмом представления \(g\) в представление \(h_i\).
\hfill\(\odot\)

Пусть
\DrawEq{d=g(b)(b)}{reduced}
Из равенств
\EqRef{g(b1)(b2)=, reduced},
\eqRef{d=g(b)(b)}{reduced}
следует, что
\ShowEq{d=h(b)(b),}

Пусть $R_2$ - другой объект категории $\mathcal A_2$.
Пусть
\ShowEq{f:A->*R}
эффективное \Ts{A_1}представление в \(\Omega_2\)\Hyph алгебре $R_2$.
Для любого $\Ii$,
пусть существует морфизм
\EqParm{ti:P->Bi}{P=A2}
представлений из $f$ в $h_i$.
Согласно замечанию
\ShowEq{ref remark morphism of representations of universal algebra}
в диаграмме отображений
\ShowEq{r12 product of effective representations}
диаграмма $(2)$ коммутативна. 
Согласно определению
\ref{definition: product of objects in category},
существует единственный морфизм $\Omega_2$\Hyph алгебры
\ShowEq{s:R->A}
такой, что коммутативна диаграмма
\ShowEq{t*s=r}
Пусть
\ShowEq{a in R2}
Пусть
\ShowEq{b=s(a)}
Из коммутативности диаграммы
\EqRef{t*s=r}
и утверждений
\EqRef{b=s(a)},
\EqRef{b=t(b)i}
следует, что
\ShowEq{b=r(a)i}
Пусть
\DrawEq{c=f(a)a}{reduced}
Из коммутативности диаграммы $(2)$ и равенств
\EqRef{d=h(b)(b),},
\EqRef{b=r(a)i},
\eqRef{c=f(a)a}{reduced}
следует, что
\ShowEq{d=r(c)i}
Из равенств
\EqRef{d=h(b)(b),},
\EqRef{d=r(c)i}
следует, что
\ShowEq{d=s(c)}
что согласуется с коммутативносью диаграммы
\EqRef{t*s=r}.

Для каждого $\Ii$, мы объединим диаграммы отображений
\EqRef{define product of single transitive representations, reduced},
\EqRef{t*s=r},
\EqRef{r12 product of effective representations}
\ShowEq{product of effective representations}
Из равенств
\eqRef{d=g(b)(b)}{reduced},
\EqRef{b=s(a)}
и из равенств
\eqRef{c=f(a)a}{reduced},
\EqRef{d=s(c)},
следует коммутативность диаграммы $(3)$.
Следовательно, отображение
\(s\)
является приведенным морфизмом
представлений из $f$ в $g$.
Согласно замечанию
\ShowEq{ref reduced morphism of representations}
отображение $s$ является гомоморфизмом $\Omega_2$ алгебры.
Согласно теореме
\ref{theorem: product exists in category of Omega algebras}
и определению
\ref{definition: product of objects in category},
приведенный морфизм
$s$
определён однозначно.

Согласно определению
\ref{definition: product of objects in category},
представление $g$
и семейство морфизмов представления
\ShowEq{ti, family}
является произведением в категории
\ShowEq{(A1*)mA2}.
\end{proof}



==> Stmt.Module.Russian.tex <==
%auto-ignore
\input{Stmt.Module.Eq}

\DefEq
{
\begin{definition}
\label{definition: module over ring}
Пусть коммутативное кольцо $D$ имеет единицу $1$.
Эффективное представление
\DrawEq{D->*V}{def}
кольца $D$
в абелевой группе $V$
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
Эффективное представление
\eqRef{D->*V}{def}
поля $D$ в абелевой группе $V$
называется
\AddIndex{векторным пространством над полем}{vector space over field} $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\qed
\end{definition}
}
{... definition: module over ring}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: tensor product of D-algebras is D-algebra}
Пусть
\ShowEq{A1...n}
- $D$\Hyph алгебры.
Тензорное произведение
$\Tensor A$
$D$\Hyph модулей
\ShowEq{A1...n}
является $D$\Hyph алгеброй,
если мы определим произведение согласно правилу
\ShowEq{xA1n*xA1n->oxA1n=}
\end{theorem}
}
{theorem: tensor product of D-algebras is D-algebra}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: representation of algebra A2 in LA}
Пусть $A$ является $D$\Hyph алгеброй.
Пусть произведение в алгебре $A\otimes A$
определено согласно правилу
\DrawEq{product in algebra AA}{}
Представление
\ShowEq{h:AoxA->L(A)}
$D$\Hyph алгебры
\ShowEq{AoxA}
в модуле $\mathcal L(D;A;A)$,
определённое равенством
\ShowEq{representation AA in LA}
позволяет отождествить тензор
\ShowEq{d in AxoA}
с линейным отображением
\ShowEq{product in algebra AA 2},
где
\ShowEq{product in algebra AA 3}
- тождественное отображение.
Линейное отображение, порождённое тензором
\ShowEq{a ox b},
имеет вид
\ShowEq{a ox b c=}
\end{theorem}
}
{theorem: representation of algebra A2 in LA}
%\DefEq

\DefEq
{
\begin{definition}
\label{definition: module over commutative ring}
Эффективное представление коммутативного кольца $D$
в абелевой группе $V$
\DrawEq{D->*V}{module}
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
\qed
\end{definition}
}
{definition: module over commutative ring}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: definition of module over commutative ring}
Элементы $D$\Hyph модуля $V$ удовлетворяют соотношениям
\begin{itemize}
\item 
\AddIndex{закону ассоциативности}{associative law}
\ShowEq{associative law, D module}
\item 
\AddIndex{закону дистрибутивности}{distributive law}
\ShowEq{distributive law, D module}
\item 
\AddIndex{закону унитарности}{unitarity law}
\ShowEq{unitarity law, D module}
\end{itemize}
для любых
\ShowEq{a,b in D, m,n in V}
\end{theorem}
}
{theorem: definition of module over commutative ring}
%\DefEq

\DefEq
{
\begin{definition}
\label{definition: \SideWS module over ring}
Пусть кольцо $D$ имеет единицу $1$.
Эффективное \SideRu востороннее представление
\DrawEq{\SideWS D->*V}{def}
кольца $D$
в абелевой группе $V$
называется
\AddIndex{\SideRu вым модулем}{\SideWS module} над кольцом $D$
или
\AddIndex{\SideRu вым $D$\Hyph модулем}{\SideWS D module}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
Эффективное \SideRu востороннее представление
\DrawEq{\SideWS D->*V}{}
кольца с делением $D$ в абелевой группе $V$
называется
\AddIndex{\SideRu вым векторным пространством}{\SideWS vector space} над кольцом с делением $D$
или
\AddIndex{\SideRu вым $D$\Hyph векторным пространством}{\SideWS D vector space}.
\qed
\end{definition}
}
{definition: module over ring}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: definition of \SideWS D module}
Элементы \SideRu вого $D$\Hyph модуля $V$ удовлетворяют соотношениям
\begin{itemize}
\item 
\AddIndex{закону ассоциативности}{associative law}
\ShowEq{associative law, \SideWS D module}
\item 
\AddIndex{закону дистрибутивности}{distributive law}
\ShowEq{distributive law, \SideWS D module}
\item 
\AddIndex{закону унитарности}{unitarity law}
\ShowEq{unitarity law, \SideWS D module}
\end{itemize}
для любых
\ShowEq{a,b in D, m,n in V}
\end{theorem}
}
{theorem: definition of D module}
%\DefEq

\DefEq
{
\begin{definition}
\label{definition: vector linearly dependent on vectors, \SideWS module}
{\it
Пусть
\EqParm{vi V}{=z}
- множество векторов.
Выражение
\ShowEq{linear composition of \SideWS vectors}
называется
\AddIndex{линейной комбинацией векторов}{linear composition of  vectors}
\ShowEq{vi}
Вектор
\ShowEq{w=ci vi \SideNS}
называется
\AddIndex{вектором, линейно зависимым от векторов}
{vector linearly dependent on vectors}
\ShowEq{vi}
}
\qed
\end{definition}
}
{definition: vector linearly dependent on vectors}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: set of vectors generated by set of vectors, \SideWS module}
Множество векторов, порождённое множеством векторов
\EqParm{vi V}{=c}
имеет вид
\ShowEq{w=sum vi, \SideNS}
\end{theorem}
}
{theorem: set of vectors generated by set of vectors}
%\DefEq

\DefEq
{
Представим множество $D$\Hyph чисел
\ShowEq{ci}
в виде матрицы
\ShowEq{c=ci}
Представим множество векторов
\ShowEq{set vi}
в виде матрицы
\ShowEq{v=vi}
Тогда мы можем записать линейную комбинацию векторов
\ShowEq{w=ci vi \SideNS}
в виде
\ShowEq{w=c cr v \SideNS}
}
{remark: scalars and vectors as matrix}
%\DefEq

\DefEq
{
\begin{definition}
\label{definition: linearly independent vectors, \SideWS module}
Векторы\,\footnote{Я следую
определению в \citeBib{Serge Lang}, страница 100.}
\ShowEq{Vector A subs row, 1}
$D$\Hyph модуля $A$
\AddIndex{линейно независимы}{linearly independent vectors},
если $c=0$ следует из уравнения
\DrawEq{ci ei=0 \SideNS}{}
В противном случае, векторы \ShowEq{Vector A subs row, 1}
\AddIndex{линейно зависимы}{linearly dependent vectors}.
\qed
\end{definition}
}
{definition: linearly independent vectors}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: basis of \SideWS vector space}
Пусть $D$ - кольцо с делением.
Множество векторов\newline
\ShowEq{basis, module}
является
\AddIndex{базисом \SideRu вого $D$\Hyph векторного пространства}{Basis}
$V$, если векторы $e_{\gii}$
линейно независимы и любой вектор $v\in V$
линейно зависит от векторов $e_{\gii}$.
\end{theorem}
}
{theorem: basis of vector space}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: basis of module, \SideWS module}
Множество векторов
\ShowEq{basis, module}
является
\AddIndex{базисом \SideRu вого $D$\Hyph модуля}{basis, module}
$V$, если произвольный вектор
\ShowEq{vv in V}
является линейной комбинацией
векторов базиса
\ShowEq{vv=ve \SideNS}
и произвольный вектор базиса
нельзя представить в виде линейной комбинации
остальных векторов базиса.
Матрица $D$\Hyph чисел
\ShowEq{coordinate matrix of vector}
называется
\AddIndex{координатной матрицей вектора}{coordinate matrix of vector}
$\Vector v$ в базисе $\Basis e$
и её элементы
\AddIndex{координатами вектора}{coordinates of vector}
$\Vector v$ относительно базиса $\Basis e$.
\end{theorem}
}
{theorem: basis of module}
%\DefEq

\DefEq
{
\begin{definition}
\label{definition: free \SideWS module over ring}
Модуль $V$ - \AddIndex{свободный \SideRu вый модуль над кольцом}{free module over ring} $D$,
если векторы базиса \SideRu вого $D$\Hyph модуля $V$ линейно независимы.\,\footnote{
Я следую определению на странице \citeBib{Serge Lang}\Hyph 103.}
\qed
\end{definition}
}
{definition: free module over ring}
%\DefEq

\DefEq
{
\begin{convention}
\label{convention: we use separate color for index of element}
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
\qed
\end{convention}
}
{convention: we use separate color for index of element}
%\DefEq

\DefEq
{
\begin{convention}
Пусть $\Basis e$ - базис свободной алгебры $A$ над кольцом $D$.
Если алгебра $A$ имеет единицу,
положим $e_{\gi 0}$ - единица алгебры $A$.
\qed
\end{convention}
}
{convention: unit of algebra in basis}
%\DefEq

\DefEq
{
\begin{definition}
\label{definition: linear map from A1 to A2, commutative module}
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Морфизм представлений
\EqParm{f:A->B}{f=f,A=12}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
$D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
Обозначим
\ShowEq{set linear maps, module}
множество линейных отображений
$D$\Hyph модуля $A_1$ в $D$\Hyph модуль $A_2$.
\qed
\end{definition}
}
{definition: linear map from A1 to A2, commutative module}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: linear map from A1 to A2, commutative module}
Линейное отображение
\EqParm{f:A->B}{f=f,A=12}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
удовлетворяет равенствам\,\footnote{В некоторых книгах
(например, \citeBib{Serge Lang}, с. 94) теорема \ref{theorem: linear map from A1 to A2, commutative module}
рассматривается как определение.}
\ShowEq{linear map from A1 to A2, 1}
\end{theorem}
}
{theorem: linear map from A1 to A2, commutative module}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: set of A->B is D module}
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - банаховый $D$\Hyph модуль с нормой $|y|_B$.
\StartLabelItem
\begin{enumerate}
\item
Множество
$B^A$
отображений
\EqParm{f:A->B}{f=f,A=AB}
является $D$\Hyph модулем.
\LabelItem{set of A->B is D module}
\item
Отображение
\ShowEq{f in BA->|f|}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
является нормой в $D$\Hyph модуле $B^A$
и величина
\ShowEq{show|f|}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
\LabelItem{norm of map}
\end{enumerate}
\end{theorem}
}
{theorem: set of A->B is D module}
%\DefEq

\DefEq
{
\begin{definition}
\label{definition: coordinates of vector}
{\it
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$,
и $A$\Hyph число $a$ имеет разложение
\[a=a^ie_i\]
относительно базиса $\Basis e$.
$D$\Hyph числа $a^i$ называются
\AddIndex{координатами}{coordinates}
$A$\Hyph числа $a$ относительно базиса $\Basis e$.
}
\qed
\end{definition}
}
{definition: coordinates of vector}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: standard representation of map A1 A2, associative algebra}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A_2$.
Пусть $\Basis I$
- базис левого \BoxB{A_2}модуля
\EqParm{L(A;B)}{A=12,=.}\,\footnote{
Если $D$\Hyph модуль $A_1$ или $D$\Hyph модуль $A_2$
не является свободным $D$\Hyph модулем,
то мы будем рассматривать множество
\ShowEq{Ik 1n}
линейно независимых линейных отображений. Теорема верна для любого линейного отображения
\EqParm{f:A->B}{f=f,A=12}
порождённого множеством линейных отображений $\Basis I$.
}
\StartLabelItem
\begin{enumerate}
\item
Отображение
\EqParm{f:A->B}{f=f,A=12}
имеет следующее разложение
\LabelItem{map f generated by basis I}
\DrawEq{map f generated by basis I}{expansion}
where
\ShowEq{fk= in A2xA2}
\item
Отображение $f$ имеет стандартное представление
\LabelItem{standard representation of map A1 A2, associative algebra}
\ShowEq{standard representation of map A1 A2, associative algebra}
\end{enumerate}
\end{theorem}
}
{theorem: standard representation of map A1 A2, associative algebra}
%\DefEq

\DefEq
{
\begin{proof}
Поскольку $\Basis I$ является базисом левого \BoxB{A_2}модуля
\EqParm{L(A;B)}{A=12,=c}
то согласно определению
\ShowEq{ref definition: basis of representation}
и теореме
\ref{theorem: set of vectors generated by the set of vectors},
существует разложение
\ShowEq{expansion of linear map with respect to basis}
линейного отображения $f$ относительно базиса $\Basis I$.
Согласно определению
\EqRef{map j, representation, tensor product},
\ShowEq{f=fkxfk}
Равенство
\eqRef{map f generated by basis I}{expansion}
является следствием равенств
\EqRef{expansion of linear map with respect to basis},
\EqRef{f=fkxfk}.
Согласно теореме
\ref{theorem: standard component of tensor, algebra},
стандартное представление тензора $f^k$ имеет вид
\ShowEq{standard representation of map A1 A2, 3, associative algebra}
Равенство
\EqRef{standard representation of map A1 A2, associative algebra}
следует из равенств
\eqRef{map f generated by basis I}{expansion},
\EqRef{standard representation of map A1 A2, 3, associative algebra}.
\end{proof}
}
{proof: standard representation of map A1 A2, associative algebra}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: conjugation transformation}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis I$ - базис левого \BoxB{A_2}модуля
\EqParm{L(A;B)}{A=12,=.}
Для любого отображения
\ShowEq{Ik in I}
существует множество линейных отображений
\ShowEq{conjugation transformation}
\ShowEq{conjugation transformation:}
$D$\Hyph модуля
$A_1\otimes A_1$
в $D$\Hyph модуль
$A_2\otimes A_2$
таких, что
\ShowEq{conjugation transformation =}
Отображение
\ShowEq{show conjugation transformation}
называется
\AddIndex{преобразованием сопряжения}{conjugation transformation}.
\end{theorem}
}
{theorem: conjugation transformation}
%\DefEq

\DefEq
{
\begin{proof}
Согласно теореме
\ref{theorem: product of linear map, algebra},
для произвольного тензора
$a\in A_1\otimes A_1$,
отображение
\ShowEq{x->Ik a x}
является линейным.
Согласно утверждению
\RefItem{map f generated by basis I},
существует разложение
\ShowEq{expansion Ik a x}
Положим
\ShowEq{b=Ikl a}
Равенство
\EqRef{conjugation transformation =}
является следствием равенств
\EqRef{expansion Ik a x},
\EqRef{b=Ikl a}.
Из равенств
\ShowEq{Ikl a1+a2}
\ShowEq{Ikl d a}
следует, что отображение $I_k^l$ является линейным.
\end{proof}
}
{proof: conjugation transformation}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: representation of composition of linear maps}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$, $A_3$ - свободные ассоциативные $D$\Hyph алгебры.
Пусть $\Basis I$ - базис левого \BoxB{A_2}модуля
\EqParm{L(A;B)}{A=12,=.}
Пусть $\Basis J$ - базис левого \BoxB{A_3}модуля
\EqParm{L(A;B)}{A=23,=.}
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\LabelItem{basis of composition of linear maps}
\DrawEq{JlIk}{linear map}
является базисом левого \BoxB{A_3}модуля
\EqParm{L(A;B)}{A=123,=.}
\item
Пусть линейное отображение
\EqParm{f:A->B}{f=f,A=12}
имеет разложение
\ShowEq{expansion of f with respect to basis I}
относительно базиса $\Basis I$.
Пусть линейное отображение
\EqParm{f:A->B}{f=g,A=23}
имеет разложение
\ShowEq{expansion of g with respect to basis J}
относительно базиса $\Basis J$.
Тогда линейное отображение
\DrawEq{h=g o f}{123}
имеет разложение
\LabelItem{hlk=glfk}
\ShowEq{expansion of h with respect to basis K}
относительно базиса $\Basis K$, где
\ShowEq{hlk=glfk}
\end{enumerate}
\end{theorem}
}
{theorem: representation of composition of linear maps}
%\DefEq

\DefEq
{
\begin{proof}
Равенство
\ShowEq{h(a)1}
является следствием равенств
\EqRef{expansion of f with respect to basis I},
\EqRef{expansion of g with respect to basis J},
\eqRef{h=g o f}{123}.
Равенство
\ShowEq{h(a)2}
является следствием равенств
\eqRef{JlIk}{linear map},
\EqRef{h(a)1}
и теоремы
\ref{theorem: conjugation transformation}.
Из равенства
\EqRef{h(a)2}
следует, что множество отображений $\Basis K$ порождает
левый \BoxB{A_3}модуля\newline
\EqParm{L(A;B)}{A=123,=.}
Из равенства
\ShowEq{aK=aJI}
следует, что
\ShowEq{aJ=0}
и, следовательно, $a^{lk}=0$.
Следовательно, множество $\Basis K$ является базисом
левого \BoxB{A_3}модуля
\EqParm{L(A;B)}{A=123,=.}
\end{proof}
}
{proof: representation of composition of linear maps}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: representation of composition of linear maps A->A}
Пусть $A$ - свободная ассоциативная $D$\Hyph алгеба.
Пусть левый \BoxB{A}модуль
\EqParm{L(A;B)}{A=A,=z}
порождён тождественным отображением $I_0=\delta$.
Пусть линейное отображение
\EqParm{f:A->B}{f=f,A=A}
имеет разложение
\ShowEq{expansion of f A->A}
Пусть линейное отображение
\EqParm{f:A->B}{f=g,A=A}
имеет разложение
\ShowEq{expansion of g A->A}
Тогда линейное отображение
\DrawEq{h=g o f}{A}
имеет разложение
\ShowEq{expansion of h A->A}
где
\ShowEq{hlk=glfk 01}
\end{theorem}
}
{theorem: representation of composition of linear maps A->A}
%\DefEq

\DefEq
{
\begin{proof}
Равенство
\ShowEq{h(a)}
является следствием равенств
\EqRef{expansion of f A->A},
\EqRef{expansion of g A->A},
\eqRef{h=g o f}{A}.
Равенство
\EqRef{hlk=glfk 01}
является следствием равенства
\EqRef{h(a)}.
\end{proof}
}
{proof: representation of composition of linear maps A->A}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: linear map in L(A,A), associative algebra}
Пусть $A_1$ - $D$\Hyph алгебра.
Пусть $A_2$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A_2$.
Левый \BoxB{A_2}модуль
\EqParm{L(A;B)}{A=12,=z}
имеет конечный
\AddIndex{базис}{basis of algebra L(A,A)} $\Basis I$.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\EqParm{f in L(A->B)}{A=12}
имеет вид
\LabelItem{f in L(A,A), 1, associative algebra}
\ShowEq{f in L(A,A), 1, associative algebra}
\item
Его стандартное представление имеет вид
\LabelItem{f in L(A,A), 2, associative algebra}
\ShowEq{f in L(A,A), 2, associative algebra}
\end{enumerate}
\end{theorem}
}
{theorem: linear map in L(A,A), associative algebra}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: h generated by f, associative algebra}
Рассмотрим $D$\Hyph алгебру $A_1$
и ассоциативную $D$\Hyph алгебру $A_2$.
Рассмотрим представление алгебры $\ATwo$
в модуле $\mathcal L(D;A_1;A_2)$.
Отображение
\ShowEq{h:A1->A2}
порождённое отображением
\EqParm{f:A->B}{f=f,A=12}
имеет вид
\ShowEq{h generated by f, associative algebra}
\end{theorem}
}
{theorem: h generated by f, associative algebra}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: coordinates of map A1 A2, algebra}
Пусть $\Basis e_1$ - базис свободного конечно мерного
$D$\Hyph модуля $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A_2$.
Пусть $\Basis I$ - базис
левого \BoxB{A_2}модуля
\EqParm{L(A;B)}{A=12,=z}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $I_k$ относительно базисов $\Basis e_1$ и $\Basis e_2$.
Координаты
\ShowEq{Coordinates of map f}
отображения
\EqParm{f in L(A->B)}{A=12}
и его стандартные компоненты
\ShowEq{standard components of map f}
связаны равенством
\ShowEq{coordinates of map A1 A2, 2, associative algebra}
\end{theorem}
}
{theorem: coordinates of map A1 A2, algebra}
%\DefEq

\DefEq
{
\begin{proof}
Относительно базисов
$\Basis e_1$ и $\Basis e_2$, линейные отображения $f$ и $I_k$ имеют вид
\ShowEq{coordinates of map f, associative algebra}
\ShowEq{coordinates of map Ik, associative algebra}
Равенство
\ShowEq{coordinates of map A1 A2, 3, associative algebra}
является следствием равенств
\EqRef{standard representation of map A1 A2, associative algebra},
\EqRef{coordinates of map f, associative algebra},
\EqRef{coordinates of map Ik, associative algebra}.
Так как векторы $\Vector e_{2\cdot\gik}$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\EqRef{coordinates of map A1 A2, 2, associative algebra}
следует из равенства
\EqRef{coordinates of map A1 A2, 3, associative algebra}.
\end{proof}
}
{proof: coordinates of map A1 A2, algebra}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: sum of linear maps, D module}
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
\end{theorem}
}
{theorem: sum of linear maps, D module}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: sum of polylinear maps, module}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,polylinear}
\ShowEq{sum of maps, 1, polylinear}
определённое равенством
\ShowEq{sum of  maps, polylinear}
называется
\AddIndex{суммой полилинейных отображений}{sum of maps}
$f$ и $g$
и является полилинейным отображением.
Множество
\ShowEq{module of polylinear maps}
является абелевой группой
относительно суммы отображений.
\end{theorem}
}
{theorem: sum of polylinear maps, module}
%\DefEq

\DefEq
{
\begin{corollary}
\label{corollary: sum of linear maps, D module}
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
\qed
\end{corollary}
}
{corollary: sum of linear maps, D module}
%\DefEq

\DefTheorem{L(An;B) is free D module}
{
Пусть $A_1$, ..., $A_n$, $B$ - свободные модули над коммутативным кольцом $D$.
$D$\Hyph модуль
\EqParm{L(A;B)}{A=xAB,=z}
является свободным $D$\Hyph модулем.
}

\DefEq
{
\begin{definition}
\label{definition: linear map from A1 to A2, module}
Приведенный морфизм представлений
\EqParm{f:A->B}{f=f,A=12}
\SideRu вого $D$\Hyph модуля $A_1$
в \SideRu вый $D$\Hyph модуль $A_2$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu вого $D$\Hyph модуля $A_1$ в \SideRu вый $D$\Hyph модуль $A_2$.

Обозначим
\ShowEq{set linear maps, module}
множество линейных отображений
\SideRu вого $D$\Hyph модуля $A_1$ в \SideRu вый $D$\Hyph модуль $A_2$.
\qed
\end{definition}
}
{definition: linear map from A1 to A2, module}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: linear map of \SideWS \DFDT module}
Линейное отображение
\ShowEq{\MF r2:A1->A2}
\SideRu вого $\DF$\Hyph модуля $A_1$
в \SideRu вый $\DT$\Hyph модуль $A_2$
удовлетворяет равенствам\,\footnote{
В некоторых книгах
(например, на странице \citeBib{Serge Lang}\Hyph 94) теорема
\ref{theorem: linear map of \SideWS \DFDT module}
рассматривается как определение.}
\ShowEq{\DFDT linear map eq}
\end{theorem}
}
{theorem: linear map of module}
%\DefEq

\DefEq
{
\begin{theorem}
\label{theorem: linear map of \SideWS \DFDT module, coordinates}
Пусть
\ShowEq{basis, module V1}
базис в свободном \SideRu вом $\DF$\Hyph модуле $A_1$
и
\ShowEq{basis, module V2}
базис в свободном \SideRu вом $\DT$\Hyph модуле $A_2$.
Тогда линейное отображение
\ShowEq{\MF r2:A1->A2}
имеет представление
\ShowEq{r2:A1->A2, \SideWS \DFDT module}
относительно заданных базисов. Здесь
\begin{itemize}
\item $a$ - координатная матрица вектора
$\Vector a$ относительно базиса $\Basis e_1$
\DrawEq{va=ae1 \SideNS}{\DFDT}
\def\Temp{D1 D2 }
\ifx\DFDT\Temp
\item
\ShowEq{r1(a)=...}
- матрица $D_2$\Hyph чисел
\fi
\item $b$ - координатная матрица вектора
\ShowEq{vb=r2(va)}
относительно базиса $\Basis e_2$
\DrawEq{vb=be2 \SideNS}{\DFDT}
\item $r_2$ - координатная матрица множества векторов
\ShowEq{Vector r2(e1)}
относительно базиса $\Basis e_2$.
Мы будем называть матрицу $r_2$
\AddIndex{матрицей линейного отображения}{matrix of linear map}
относительно базисов $\Basis e_1$ и $\Basis e_2$.
\end{itemize}
\end{theorem}
}
{theorem: linear map of module, coordinates}
%\DefEq

\DefEq
{
\begin{definition}
\label{definition: algebra over ring}
Пусть $D$ - коммутативное кольцо.
$D$\Hyph модуль $A$ называется
\AddIndex{алгеброй над кольцом}{algebra over ring} $D$
или
\AddIndex{$D$\Hyph алгеброй}{D algebra},
если определена операция произведения\,\footnote{
Я следую определению,
приведенному в
\citeBib{Richard D. Schafer}, страница 1,
\citeBib{0105.155}, страница 4. Утверждение,
верное для произвольного $D$\Hyph модуля,
верно также для $D$\Hyph алгебры.} в $A$
\DrawEq{product in D algebra}{definition}
где $C$ - билинейное отображение
\ShowEq{product in algebra, definition 1}
Если $A$ является свободным
$D$\Hyph модулем, то $A$ называется
\AddIndex{свободной алгеброй над кольцом}{free algebra over ring} $D$.
\qed
\end{definition}
}
{definition: algebra over ring}
%\DefEq

\DefEq
{
\begin{definition}
\label{definition: commutator of algebra}
\AddIndex{Коммутатор}{commutator of algebra}
\ShowEq{commutator of algebra}
служит мерой коммутативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{коммутативной}{commutative D algebra},
если
\ShowEq{commutative D algebra}
\qed
\end{definition}
}
{definition: commutator of algebra}
%\DefEq

\DefEq
{
\begin{definition}
\label{definition: nucleus of algebra}
\AddIndex{Ядро $D$\Hyph алгебры $A$}{nucleus of algebra}
- это
множество\,\footnote{
Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 13}
\ShowEq{nucleus of algebra}
\qed
\end{definition}
}
{definition: nucleus of algebra}
%\DefEq

\DefEq
{
\begin{definition}
\label{definition: associator of algebra}
\AddIndex{Ассоциатор}{associator of algebra}
\ShowEq{associator of algebra}
служит мерой ассоциативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной}{associative D algebra},
если
\ShowEq{associative D algebra}
\qed
\end{definition}
}
{definition: associator of algebra}
%\DefEq

\DefEq
{
\begin{definition}
\label{definition: center of algebra}
\AddIndex{Центр $D$\Hyph алгебры $A$}{center of algebra}
- это
множество\,\footnote{
Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, страница 14}
\ShowEq{center of algebra}
\qed
\end{definition}
}
{definition: center of algebra}
%\DefEq

\DefEq
{
\begin{definition}
\label{definition: otimes -}
Билинейное отображение
\ShowEq{otimes -}
определено равенством
\ShowEq{otimes -, 1}
\qed
\end{definition}
}
{definition: otimes -}
%\DefEq

\DefEq
{
\begin{theorem}[принцип двойственности для модуля над кольцом]
\label{theorem: duality principle, module over ring}
Любое утверждение, справедливое для
левого $D$\Hyph модуля $V$,
будет справедливо для правого $D$\Hyph модуля $V$, если
\begin{itemize}
\item
мы будем пользоваться правосторонним произведением на $D$\Hyph число $a$ вместо
левостороннего произведения на $D$\Hyph число $a$;
\item
мы будем пользоваться правым сдвигом $R(a)$ кольца $D$
вместо левого сдвига $L(a)$.
\end{itemize}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: duality principle, algebra representation}.
\end{proof}
}
{theorem: duality principle, module over ring}
%\DefEq


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%0%0
\Symb%
   {единичный интервал}%
   {unit interval}%
   {0}{0}%

\SetIndexSpace%A%0
\Symb%
   {минорная матрица}%
   {A from b a}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {A from columns T}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {A from rows S}%
   {A}{0}%
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {A without column a}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {A without columns T}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {A without row b}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {A without rows S}%
   {A}{0}%
\Symb%
   {активное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
   {A}{0}%
\Symb%
   {активное представление группы $G(\Vector  f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {active representation in basis manifold, tower of representations}%
   {A}{0}%
\Symb%
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
   {A}{0}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
   {A}{0}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
   {A}{0}%
\Symb%
   {аффинное пространство}%
   {An}%
   {A}{0}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
   {A}{0}%
\Symb%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
   {A}{0}%
\Symb%
   {категория левосторонних представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
   {A}{0}%
\Symb%
   {категория представлений}%
   {category of representations}%
   {A}{0}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
   {A}{0}%
\Symb%
   {компонента линейного отображения}%
   {component of linear map, vector}%
   {A}{0}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
   {A}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map, vector}%
   {A}{0}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
   {A}{0}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
   {A}{0}%
\Symb%
   {\crd вектор}%
   {crd vector}%
   {A}{0}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
   {A}{0}%
\Symb%
   {\CR произведение}%
   {cr-product}%
   {A}{0}%
\Symb%
   {\dcr вектор}%
   {dcr vector}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
   {A}{0}%
\Symb%
   {\drc вектор}%
   {drc vector}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
   {A}{0}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
   {A}{0}%
\Symb%
   {тензор, обратный тензору $a$}%
   {inverse tensor}%
   {A}{0}%
\Symb%
   {изоморфны}%
   {isomorphic}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {левая дробь}%
   {left fraction}%
   {A}{0}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
   {A}{0}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
   {A}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {A}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
   {A}{0}%
\Symb%
   {$A$\Hyph модуль однородных многочленов над $D$\Hyph алгеброй $A$}%
   {module of homogeneous polynomials over algebra}%
   {A}{0}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
   {A}{0}%
\Symb%
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
   {A}{0}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
   {A}{0}%
\Symb%
   {орбита эффективного левостороннего представления}%
   {orbit of effective left-side representation}%
   {A}{0}%
\Symb%
   {орбита эффективного правостороннего представления}%
   {orbit of effective right-side representation}%
   {A}{0}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear map}%
   {A}{0}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
   {A}{0}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
   {A}{0}%
\Symb%
   {главный идеал}%
   {principal ideal}%
   {A}{0}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
   {A}{0}%
\Symb%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
   {A}{0}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
   {A}{0}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
   {A}{0}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
   {A}{0}%
\Symb%
   {\RC произведение}%
   {rc-product}%
   {A}{0}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
   {A}{0}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
   {A}{0}%
\Symb%
   {множество аддитивных отображений}%
   {set additive maps}%
   {A}{0}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
   {A}{0}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
   {A}{0}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
   {A}{0}%
\Symb%
   {симплекс}%
   {simplex}%
   {A}{0}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
   {A}{0}%
\Symb%
   {пространство орбит эффективного левостороннего представления}%
   {space of orbits of effective left-side representation}%
   {A}{0}%
\Symb%
   {пространство орбит эффективного правостороннего представления}%
   {space of orbits of effective right-side representation}%
   {A}{0}%
\Symb%
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
   {A}{0}%
\Symb%
   {квадратный корень}%
   {square root}%
   {A}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {A}{0}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
   {A}{0}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
   {A}{0}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
   {A}{0}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
   {A}{0}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов \rcd векторного пространства $\Vector V$}%
   {basis manifold of rcd vector space}%
   {B}{0}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
   {B}{0}%
\Symb%
   {многообразие базисов представления $f$}%
   {basis manifold representation F algebra}%
   {B}{0}%
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
   {B}{0}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
   {B}{0}%
\Symb%
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
   {B}{0}%
\Symb%
   {алгебра Бореля}%
   {Borel algebra}%
   {B}{0}%
\Symb%
   {каноническое частное от деления}%
   {canonical remainder of the division}%
   {B}{0}%
\Symb%
   {декартова степень}%
   {Cartesian power}%
   {B}{0}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
   {B}{0}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
   {B}{0}%
\Symb%
   {замкнутый шар}%
   {closed ball}%
   {B}{0}%
\Symb%
   {замыкание множества}%
   {closure of set}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
   {B}{0}%
\Symb%
   {структура всех подпредставлений представления $f$}%
   {lattice of subrepresentations}%
   {B}{0}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
   {B}{0}%
\Symb%
   {открытый шар}%
   {open ball}%
   {B}{0}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, 1 n}%
   {B}{0}%
\Symb%
   {правая дробь}%
   {right fraction}%
   {B}{0}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
   {B}{0}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph алгебра измеримых относительно меры $\mu$ множеств}%
   {algebra of sets measurable with respect to measure}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
   {C}{0}%
\Symb%
   {класс непрерывности}%
   {class Cn}%
   {C}{0}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
   {C}{0}%
\Symb%
   {косинус}%
   {cosine}%
   {C}{0}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
   {C}{0}%
\Symb%
   {гиперболический косинус}%
   {hyperbolic cosine}%
   {C}{0}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
   {C}{0}%
\Symb%
   {структурные константы}%
   {structural constants}%
   {C}{0}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
   {D}{0}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
   {D}{0}%
\Symb%
   {компонента производной отображения $f(x)$}%
   {component of derivative}%
   {D}{0}%
\Symb%
   {компонента производной второго порядка отображения $f(x)$}%
   {component of derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
   {D}{0}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
   {D}{0}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
   {D}{0}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
   {D}{0}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
   {D}{0}%
\Symb%
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map inline}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n inline}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order inline}%
   {D}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
   {D}{0}%
\Symb%
   {дифференциал отображения $f$}%
   {differential of map}%
   {D}{0}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
   {D}{0}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
   {D}{0}%
\Symb%
   {внешний дифференциал}%
   {exterior differential}%
   {D}{0}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
   {D}{0}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
   {D}{0}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
   {D}{0}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
   {D}{0}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
   {D}{0}%
\Symb%
   {производная Картана}%
   {overbrace D}%
   {D}{0}%
\Symb%
   {производная}%
   {overline D}%
   {D}{0}%
\Symb%
   {частная производная}%
   {partial derivative}%
   {D}{0}%
\Symb%
   {частная производная второго порядка}%
   {partial derivative of second order}%
   {D}{0}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
   {D}{0}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
   {D}{0}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
   {D}{0}%
\Symb%
   {стандартная компонента производной}%
   {standard component of derivative}%
   {D}{0}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%
   {D}{0}%

\SetIndexSpace%E%0
\Symb%
   {матрица Якоби левого сдвига}%
   {aE, quaternion, Jacobian matrix}%
   {E}{0}%
\Symb%
   {аффинный базис}%
   {Affine Basis}%
   {E}{0}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
   {E}{0}%
\Symb%
   {базис модуля}%
   {basis for module}%
   {E}{0}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
   {E}{0}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
   {E}{0}%
\Symb%
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
   {E}{0}%
\Symb%
   {базис $D$\Hyph векторного пространства}%
   {basis, D vector space}%
   {E}{0}%
\Symb%
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
   {E}{0}%
\Symb%
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
   {E}{0}%
\Symb%
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
   {E}{0}%
\Symb%
   {базис в векторного расслоения}%
   {basis, vector bundle}%
   {E}{0}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
   {E}{0}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
   {E}{0}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
   {E}{0}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
   {E}{0}%
\Symb%
   {экспонента}%
   {exponent}%
   {E}{0}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
   {E}{0}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
   {E}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
   {E}{0}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
   {E}{0}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
   {E}{0}%
\Symb%
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
   {E}{0}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
   {E}{0}%
\Symb%
   {множество эндоморфизмов}%
   {set of endomorphisms}%
   {E}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {множество преобразований универсальной алгебры}%
   {set of transformations}%
   {E}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
   {E}{0}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
   {E}{0}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
   {E}{0}%
\Symb%
   {вектор базиса}%
   {vector of basis}%
   {E}{0}%

\SetIndexSpace%F%0
\Symb%
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
   {F}{0}%
\Symb%
   {центро-аффинный}%
   {Central Affine Basis, division ring}%
   {F}{0}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
   {F}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
   {F}{0}%
\Symb%
   {внешнее произведение}%
   {exterior product}%
   {F}{0}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
   {F}{0}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
   {F}{0}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
   {F}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
   {F}{0}%
\Symb%
   {норма функционала}%
   {norm of functional}%
   {F}{0}%
\Symb%
   {норма отображения}%
   {norm of map}%
   {F}{0}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
   {F}{0}%
\Symb%
   {норма представления}%
   {norm of representation}%
   {F}{0}%
\Symb%
   {орбита представления}%
   {orbit of representation}%
   {F}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
   {F}{0}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
   {F}{0}%
\Symb%
   {система отсчёта}%
   {reference frame}%
   {F}{0}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
   {F}{0}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
   {F}{0}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
   {F}{0}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
   {F}{0}%
\Symb%
   {сумма отображений}%
   {sum of maps}%
   {F}{0}%
\Symb%
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
   {F}{0}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, 1 n}%
   {G}{0}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
   {G}{0}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
   {G}{0}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
   {G}{0}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
   {G}{0}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
   {G}{0}%
\Symb%
   {неопределённый интеграл}%
   {indefinite integral}%
   {G}{0}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {алгебра Ли группы Ли}%
   {Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {группа линейных преобразований}%
   {linear transformation group}%
   {G}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {G}{0}%
\Symb%
   {орбита эффективного	\Ts представления группы}%
   {orbit of effective starT representation of fibered group}%
   {G}{0}%
\Symb%
   {орбита эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar representation of fibered group}%
   {G}{0}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
   {G}{0}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
   {G}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {G}{0}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
   {H}{0}%
\Symb%
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
   {H}{0}%
\Symb%
   {горизонтальное подпространство}%
   {horizontal subspace}%
   {H}{0}%
\Symb%
   {алгебра кватернионов}%
   {quaternion algebra}%
   {H}{0}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
   {H}{0}%
\Symb%
   {множество гомоморфизмов}%
   {set of homomorphisms}%
   {H}{0}%

\SetIndexSpace%I%0
\Symb%
   {преобразование сопряжения}%
   {conjugation transformation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
   {I}{0}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
   {I}{0}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%
   {I}{0}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
   {J}{0}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
   {J}{0}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
   {J}{0}%
\Symb%
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
   {J}{0}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
   {J}{0}%

\SetIndexSpace%K%0
\Symb%
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
   {K}{0}%
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%
   {K}{0}%

\SetIndexSpace%L%0
\Symb%
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
   {L}{0}%
\Symb%
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
   {L}{0}%
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
   {L}{0}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
   {L}{0}%
\Symb%
   {левый сдвиг}%
   {left shift}%
   {L}{0}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
   {L}{0}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
   {L}{0}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
   {L}{0}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
   {L}{0}%
\Symb%
   {модуль косо симметричных полилинейных отображений}%
   {module of skew symmetric polylinear maps}%
   {L}{0}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
   {L}{0}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
   {L}{0}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
   {L}{0}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
   {L}{0}%
\Symb%
   {множество линейных отображений}%
   {set linear maps}%
   {L}{0}%
\Symb%
   {множество левосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of left-side nonsingular transformations}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
   {L}{0}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
   {L}{0}%

\SetIndexSpace%M%0
\Symb%
   {множество левосторонних преобразований универсальной алгебры $M$}%
   {set of left-side transformations}%
   {M}{0}%
\Symb%
   {множество отображений в $\Omega$\Hyph группу $A$}%
   {set of maps to Omega group}%
   {M}{0}%
\Symb%
   {множество правосторонних преобразований универсальной алгебры $M$}%
   {set of right-side transformations}%
   {M}{0}%
\Symb%
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
   {M}{0}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
   {N}{0}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
   {N}{0}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
   {O}{0}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
   {O}{0}%
\Symb%
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
   {O}{0}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
   {O}{0}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
   {O}{0}%
\Symb%
   {орбита \Ts{G}представления группы}%
   {orbit of representation of group}%
   {O}{0}%
\Symb%
   {тензорное произведение}%
   {tensor product}%
   {O}{0}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
   {P}{0}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
   {P}{0}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
   {P}{0}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
   {P}{0}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {пассивное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {passive representation in basis manifold}%
   {P}{0}%
\Symb%
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {passive representation in basis manifold, tower of representations}%
   {P}{0}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
   {P}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%
   {P}{0}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
   {R}{0}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
   {R}{0}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
   {R}{0}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
   {R}{0}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
   {R}{0}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
   {R}{0}%
\Symb%
   {произведение колец множеств}%
   {product of rings of sets}%
   {R}{0}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
   {R}{0}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
   {R}{0}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
   {R}{0}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
   {R}{0}%
\Symb%
   {правый сдвиг}%
   {right shift}%
   {R}{0}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
   {R}{0}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
   {R}{0}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
   {R}{0}%
\Symb%
   {множество правосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of right-side nonsingular transformations}%
   {R}{0}%
\Symb%
   {сферические координаты}%
   {spherical coordinates}%
   {R}{0}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
   {S}{0}%
\Symb%
   {гиперболический синус}%
   {hyperbolic sine}%
   {S}{0}%
\Symb%
   {интеграл отображения \(f\)}%
   {integral of map}%
   {S}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
   {S}{0}%
\Symb%
   {образ базиса $X$ при пассивном преобразовании $S$}%
   {passive transformation of basis, representation}%
   {S}{0}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of permutations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of transpositions}%
   {S}{0}%
\Symb%
   {синус}%
   {sine}%
   {S}{0}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%
   {S}{0}%

\SetIndexSpace%T%0
\Symb%
   {категория левосторонних представлений}%
   {category of left-side representations}%
   {T}{0}%
\Symb%
   {касательная плоскость к группе Ли $G$}%
   {tangent plane to Lie group}%
   {T}{0}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%
   {T}{0}%

\SetIndexSpace%V%0
\Symb%
   {аффинное пространство}%
   {affine space}%
   {V}{0}%
\Symb%
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
   {V}{0}%
\Symb%
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
   {V}{0}%
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
   {V}{0}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
   {V}{0}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
   {V}{0}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
   {V}{0}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
   {V}{0}%
\Symb%
   {линейная комбинация векторов}%
   {linear composition of vectors}%
   {V}{0}%
\Symb%
   {векторное пространство}%
   {V}%
   {V}{0}%
\Symb%
   {вертикальная компонента вектора}%
   {vertical component of vector}%
   {V}{0}%
\Symb%
   {вертикальное подпространство}%
   {vertical subspace}%
   {V}{0}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
   {W}{0}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to generating set, representation}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
   {W}{0}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
   {W}{0}%
\Symb%
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
   {W}{0}%
\Symb%
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
   {W}{0}%
\Symb%
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
   {W}{0}%
\Symb%
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
   {W}{0}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
   {W}{0}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
   {W}{0}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
   {W}{0}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
   {W}{0}%
\Symb%
   {суперпозиция координат эндоморфизма представления $f$ и точки $m$}%
   {superposition of coordinates, representation}%
   {W}{0}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
   {W}{0}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
   {W}{0}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%
   {W}{0}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
   {X}{0}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
   {X}{0}%
\Symb%
   {неголономная координата}%
   {x(k)}%
   {X}{0}%

\SetIndexSpace%Z%0
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
   {Z}{0}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%
   {Z}{0}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
   {Delta}{1}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
   {Delta}{1}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
   {Delta}{1}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%
   {Delta}{1}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
   {Gamma}{1}%
\Symb%
   {связность}%
   {conection overline}%
   {Gamma}{1}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
   {Gamma}{1}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
   {Gamma}{1}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
   {Gamma}{1}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
   {Gamma}{1}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%
   {Gamma}{1}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
   {Lambda}{1}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%
   {Lambda}{1}%

\SetIndexSpace%Mu%1
\Symb%
   {декартово произведение мер}%
   {Cartesian product of measures}%
   {Mu}{1}%
\Symb%
   {степень меры}%
   {power of measure}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures, otimes}%
   {Mu}{1}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%
   {Omega}{1}%
\Symb%
   {определённый интеграл}%
   {definite integral}%
   {Omega}{1}%
\Symb%
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
   {Omega}{1}%
\Symb%
   {норма операции}%
   {norm of operation}%
   {Omega}{1}%
\Symb%
   {область операторов}%
   {operator domain}%
   {Omega}{1}%
\Symb%
   {множество дифференциальных $p$\Hyph форм}%
   {set of differential p forms}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операций $\Omega$\Hyph алгебры}%
   {set of n-ary operations}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операторов}%
   {set of n-ary operators}%
   {Omega}{1}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%
   {Psi}{1}%

\SetIndexSpace%Sigma%1
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
   {Sigma}{1}%
\Symb%
   {чётность перестановки}%
   {parity of permutation}%
   {Sigma}{1}%
\Symb%
   {подрасслоение}%
   {subbundle}%
   {Sigma}{1}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
   {Nabla}{2}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%
   {Nabla}{2}%

\SetIndexSpace%Phi%1
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%
   {Phi}{1}%
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
   {Phi}{1}%

\SetIndexSpace%Pi%1
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_i$, $i\in I$}%
   {Cartesian product of groups}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, i 1 n}%
   {Pi}{1}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
   {Pi}{1}%
\Symb%
   {произведением объектов $\{B_i,i\in I\}$ в категории $\mathcal A$}%
   {product of objects in category}%
   {Pi}{1}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, i 1 n}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%
   {Pi}{1}%

\CloseIndex

